Offline Reinforcement Learning and Sequence Modeling for Downlink Link Adaptation

Link adaptation (LA) is an essential function in modern wireless communication systems that dynamically adjusts the transmission rate of a communication link to match time- and frequency-varying radio link conditions. However, factors such as user mobility, fast fading, imperfect channel quality information, and aging of measurements make the modeling of LA challenging. To bypass the need for explicit modeling, recent research has introduced online reinforcement learning (RL) approaches as an alternative to the more commonly used rule-based algorithms. Yet, RL-based approaches face deployment challenges, as training in live networks can potentially degrade real-time performance. To address this challenge, this paper considers offline RL as a candidate to learn LA policies with minimal effects on the network operation. We propose three LA designs based on batch-constrained deep Q-learning, conservative Q-learning, and decision transformer. Our results show that offline RL algorithms can match the performance of state-of-the-art online RL methods when data is collected with a proper behavioral policy.

==> img.tex <==
% \begin{figure*}[ht]
%     \centering
%     \begin{minipage}{0.33\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{Figures/PL1-throughput-legend-inside.pdf}
%         \label{fig:PL1-Throughput}
%     \end{minipage}
%     \begin{minipage}{0.33\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{Figures/PL1-bler-legend-inside.pdf}
%         \label{fig:PL1-bler}
%     \end{minipage}
%     \begin{minipage}{0.33\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{Figures/PL1-se-legend-inside.pdf}
%         \label{fig:PL1-se}
%     \end{minipage}

%     \begin{minipage}{0.33\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{Figures/PL2-throughput-legend-inside.pdf}
%         \label{fig:PL2-throughput}
%     \end{minipage}
%     \begin{minipage}{0.33\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{Figures/PL2-bler-legend-inside.pdf}
%         \label{fig:PL2-bler}
%     \end{minipage}
%     \begin{minipage}{0.33\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{Figures/PL2-se-legend-inside.pdf}
%         \label{fig:PL2-se}
%     \end{minipage}
% \end{figure*}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.4\textwidth]{Figures/PL1-throughput-legend-inside.pdf}
%     \caption{Comparison of throughput values of the considered offline RL algorithms.}
%     \label{fig:PL1-Throughput}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.4\textwidth]{Figures/PL1-bler-legend-inside.pdf}
%     \caption{Comparison of BLER values of the considered offline RL algorithms.}
%     \label{fig:PL1-bler}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.4\textwidth]{Figures/PL1-se-legend-inside.pdf}
%     \caption{Comparison of SE values of the considered offline RL algorithms.}
%     \label{fig:PL1-se}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.4\textwidth]{Figures/PL2-throughput-legend-inside.pdf}
%     \caption{Comparison of throughput values of the considered offline RL algorithms (trained on suboptimal data).}
%     \label{fig:PL2-throughput}
% \end{figure}
% %
% \begin{figure}
%     \centering
%     \includegraphics[width=0.4\textwidth]{Figures/PL2-bler-legend-inside.pdf}
%     \caption{Comparison of BLER values of the considered offline RL algorithms (trained on suboptimal data).}
%     \label{fig:PL2-bler}
% \end{figure}
% %
% \begin{figure}
%     \centering
%     \includegraphics[width=0.4\textwidth]{Figures/PL2-se-legend-inside.pdf}
%     \caption{Comparison of SE values of the considered offline RL algorithms (trained on suboptimal data).}
%     \label{fig:PL2-se}
% \end{figure}




\begin{table}[t!]
\centering
\setlength{\tabcolsep}{8pt} % Adjust the column spacing
\begin{tabular}{lccc}
\hline
\toprule\toprule
    \ac{LA} algorithm & Throughput & \ac{SE} & \ac{BLER} \\
\toprule
    BC            & 16.10 Mbps   & 7.53 bps/Hz   & 0.30     \\
    BCQ           & 16.11 Mbps   & 7.53 bps/Hz   & 0.30     \\
    CQL           & 16.10 Mbps   & 7.52 bps/Hz   & 0.30     \\
    DT            & 16.07 Mbps   & 7.46 bps/Hz   & 0.31     \\
    DQN$_{opt}$   & 16.02 Mbps   & 7.50 bps/Hz   & 0.32     \\
    OLLA ($10\%$) & 14.76 Mbps   & 6.21 bps/Hz   & 0.13     \\
    OLLA ($30\%$) & 15.51 Mbps   & 6.87 bps/Hz   & 0.30     \\
    OLLA ($50\%$) & 15.16 Mbps   & 6.92 bps/Hz   & 0.49     \\
    OLLA ($70\%$) & 14.77 Mbps   & 6.81 bps/Hz   & 0.66     \\
    OLLA ($90\%$) & 14.71 Mbps   & 6.84 bps/Hz   & 0.83     \\
\bottomrule\bottomrule
\hline
\end{tabular}
\vspace{0.25cm} % Adjust vertical space between table and caption
\caption{Comparison of the offline RL methods trained on $\mathcal D_\text{opt}$. \\ OLLA (x\%) refers to OLLA with a fixed BLER target of x\%.}
\label{table: opt table}
\end{table}

\begin{table}[t!]
\centering
\setlength{\tabcolsep}{8pt} % Adjust the column spacing
\begin{tabular}{lccc}
\hline
\toprule\toprule
    \ac{LA} algorithm & Throughput & \ac{SE} & \ac{BLER} \\
\toprule
    BC            & 16.00 Mbps   & 7.50 bps/Hz   & 0.31     \\
    BCQ           & 16.00 Mbps   & 7.60 bps/Hz   & 0.34     \\
    CQL           & 16.05 Mbps   & 7.59 bps/Hz   & 0.33     \\
    DT            & 15.67 Mbps   & 7.25 bps/Hz   & 0.36     \\
    DQN$_{s-opt}$ & 15.89 Mbps   & 7.45 bps/Hz   & 0.33     \\
    OLLA ($10\%$) & 14.76 Mbps   & 6.21 bps/Hz   & 0.13     \\
    OLLA ($30\%$) & 15.51 Mbps   & 6.87 bps/Hz   & 0.30     \\
    OLLA ($50\%$) & 15.16 Mbps   & 6.92 bps/Hz   & 0.49     \\
    OLLA ($70\%$) & 14.77 Mbps   & 6.81 bps/Hz   & 0.66     \\
    OLLA ($90\%$) & 14.71 Mbps   & 6.84 bps/Hz   & 0.83     \\
\bottomrule\bottomrule
\hline
\end{tabular}
\vspace{0.25cm} % Adjust vertical space between table and caption
\caption{Comparison of the offline RL methods trained on $\mathcal D_\text{s-opt}$. \\ OLLA (x\%) refers to OLLA with a fixed BLER target of x\%.}
\label{table: s-opt table}
\end{table}


==> old_versions/backup_2024_11_17/1_introduction_2024_1118.tex <==
\section{Introduction}\label{sec:introduction}
\begin{comment}
The increasing complexity of \ac{RRM} functionalities across successive generations of mobile broadband systems, coupled with the expanding variety of deployment scenarios \cite{calabrese_learning_2018}, has driven research efforts focused on leveraging the vast amount of data available within the network from measurements and system observations \cite{calabrese_learning_2018, generalization_2024}. 

\Ac{ML} methods and, in particular, \ac{RL} have recently gained attention as a solution to address the complex control problems involved in \ac{RRM} for \acp{RAN} where time- and frequency-varying channel conditions often make rule-based algorithms suboptimal. Due to their ability to learn directly from experienced behavior and to adapt to changing environment conditions, \ac{RL} methods are being considered to replace traditional rule-based \ac{RAN} functionalities with models learned from data \cite{gronland2024constrained,mollerstedt2024model}. However, training \ac{RL} agents in a live network requires algorithms to explore the state-action space in order to learn an optimal policy, at the cost of taking actions that may be suboptimal \cite{lattimore2020bandit,russo2024model}.

In this paper, we focus on the problem of \ac{LA}, a fundamental functionality of \ac{RRM} dynamically adjusting the transmission rate of a communication link based on the channel conditions reported by the \ac{UE}. We will consider the downlink communication between a base station and the \ac{UE}, but similar findings are reusable for the uplink case. In a data-rich environment such as the \ac{RAN} one, the recent advancements in ML and, at the same time, hardware, present an opportunity to tackle the problem of link adaptation with a strongly data-driven approach \cite{calabrese_learning_2018}. A data-driven approach directly acting on the link adaptation parameters could address the shortcomings associated with current solutions to \ac{LA} that frame it as a control problem and, as shown in multiple works such as \cite{geiser_drlla_2022}, improve performance.

With the goal of overcoming the challenges associated with the training phase of \ac{RL} agents mentioned above, we consider a family of \ac{RL} algorithms referred to as \textbf{offline \ac{RL}}. Offline \ac{RL} algorithms aim at learning policies from fixed datasets of transitions previously collected by a, possibly unknown, behavioral policy. This approach is attractive for critical applications, like \acp{RAN} operations, where online learning methods could be costly to implement or negatively affect system performance, especially during training. 

The main contributions of this work include: \textbf{(1)} a thorough evaluation and comparison of the performance of the various offline \ac{RL} algorithms designed for \ac{LA} using an event-driven system-level simulator compliant with the \ac{3GPP} \ac{5G} NG-RAN system; \textbf{(2)} a new sequence modeling framework necessary to solve \ac{LA} using the \ac{DT} architecture; \textbf{(3)} the design of an offline \ac{RL} algorithm based on \ac{DT}, including a new positional encoding definition; \textbf{(4)} the definition of a new objective function for the \ac{LA} problem allowing multiple, alternative ways of conditioning the inference with \ac{DT}.

The choice of considering \ac{DT} is driven by the capability to well-generalize over different tasks and data distributions which appears evident with transformer for, especially, \ac{NLP}. Similarly, we hope \ac{DT} to be able to adapt to different types of network traffic, facilitating the deployment of a same model over different network sites.

\begin{itemize}
    \item Highlight contributions, including how to construct the sequence in training and inference
    \item Add comment on choice of baseline for comparison (e.g., why we do not relate to prior published papers)
\end{itemize}

\end{comment}
%----


Modern radio access and wireless networks -- such as the \ac{5G} \ac{NR} systems -- employ model-based \ac{LA} algorithms to adapt the \ac{MCS} to time-- and frequency-varying channel conditions to maintain high spectral efficiency\iffalse while adhering to \ac{BLER} targets\fi ~\cite{duran_self-optimization_2015, blanquez-casado_eolla_2016, Blanquez-Casado:19, Ramireddy:22, Nicolini:23}. Both in \ac{TDD} and \ac{FDD} systems, \ac{LA} in the \ac{DL} relies on \ac{CSI} reports provided by the \ac{UE} that include the \ac{CQI}, a rank indicator, and a precoder matrix indicator~\cite{3rd_generation_partnership_project_3gpp_technical_2024}.

As \ac{CSI} reports may be inaccurate and rapidly age due to variations in channel and interference conditions, an \ac{OLLA} scheme is typically adopted to adjust \ac{SINR} estimates inferred from inaccurate or aged~\acp{CQI} to adhere to \ac{BLER} targets based on the \ac{HARQ} feedback~\cite{duran_self-optimization_2015}. Nonetheless, user mobility, fast fading, limited receiver-side information at the transmitter, as well as the heterogeneity of \acp{UE} population, e.g., in terms of receiver and hardware capabilities, render \ac{RRM} problems in \acp{RAN}, like \ac{LA}, complex control tasks to model~\cite{Chen:23, generalization_2024}.

Recognizing the challenges faced by model-based approaches, \ac{ML} methods, such as \ac{RL}, have recently gained attention to address the complex control problems in \acp{RAN} \cite{calabrese_learning_2018}, where time- and frequency-varying channel conditions often make rule-based algorithms suboptimal. The ability of \ac{RL} to learn directly from experienced behavior and to adapt to changes in the environment makes it appealing to replace traditional rule-based \ac{RAN} functionalities with models learned from data~\cite{generalization_2024}. Several works have applied this approach to \ac{LA}, starting with tabular~\cite{Bruno:14} and bandit~\cite{saxena_reinforcement_2021} approaches, adaptations of \ac{OLLA} based on Q-learning~\cite{Chen:23}, and \ac{DQN}-based designs intended to replace \ac{OLLA}~\cite{generalization_2024}.
%
However, training \ac{RL} agents in live networks requires algorithms to explore the state-action space to learn~an optimal policy, at the cost of taking suboptimal actions that may temporarily affect the network performance~\cite{generalization_2024, russo2024model}.

To address this adverse effect of \ac{RL}, recent works have proposed offline \ac{RL}, which aims at learning an optimal policy from a \emph{static dataset} of transitions produced by a behavioral policy, thus avoiding direct interactions with the environment while training~\cite{levine_offline_2020-1, janner2021offline, schweighofer2022dataset, Kumar:23, lyu2022mildly}. The inability to improve the training dataset during the training phase 
binds the quality and the behavior of the learned policy to the quality and state-action coverage of the available data. As such, distribution shift and out-of-distribution behavior, that is, a mismatch between the training and testing trajectory distributions, can render the learned policy ineffective.
%As the training dataset is not augmented during training, the quality and the behavior of the learned policy is constrained by the quality and state-action coverage of the available data. As such, distribution shift and out-of-distribution behavior, that is, a mismatch between the training and testing trajectories, can render the learned policy ineffective. %Thus employing offline \ac{RL} in complex real-time control problems, such as \ac{LA}, is non-trivial.
%\gf{\it GF: One paragraph about offline RL and the out-of-distribution and distribution shift problems and the concept 
%of transformers, as well as maybe other main concepts that must not come out of the blue later (maybe attention mechanisms ?).}
%
Thus, employing offline \ac{RL} to replace complex real-time \ac{RRM} control functions in \acp{RAN}, such as \ac{LA}, is non-trivial and presents two main challenges: firstly, the ability of an offline \ac{RL} design to achieve, when trained with proper data, optimal performance, e.g., comparable with an policy learned online; secondly, the design of a non-invasive behavioral policy to collect rich data in live networks without affecting performance.
\begin{comment}
    To capitalize the advantages of \ac{RL} over rule-based approaches while reducing the potentially negative impact of active exploration on the \acp{RAN} operation, this paper considers offline RL to design LA in 5G networks. We propose three LA designs  based on \ac{BCQ}~\cite{fujimoto_off-policy_2019}, \ac{CQL}~\cite{kumar_conservative_2020}, and \ac{DT}~\cite{chen_decision_2021}. While for \ac{BCQ} and \ac{CQL} we model the \ac{LA} problem as a partially observable \ac{MDP}, for \ac{DT} we consider a sequence modeling approach, where an \ac{LA} action for a packet transmission (or retransmission) is inferred based on a sequence of historical states, actions and rewards. Our results show that offline \ac{RL} algorithms can achieve performance of state-of-the-art online \ac{RL} when data is collected with a proper behavioral policy.
\end{comment}

This paper focuses on the first challenge considering offline \ac{RL} for \ac{LA} in \ac{5G} networks. We present three \ac{LA} designs based on \ac{BCQ}~\cite{fujimoto2019off}, \ac{CQL}~\cite{kumar_conservative_2020}, and \ac{DT}~\cite{chen_decision_2021}, with  a trained \ac{DQN} model \cite{mnih_playing_2013} acting as a behavioral policy for data collection. While for \ac{BCQ} and \ac{CQL} we model the \ac{LA} problem as a partially observable \ac{MDP}, \ac{DT} requires a sequence modeling approach, where a \ac{LA} action is inferred using a sequence of historical states, actions and rewards, allowing to optimize long-term rewards, e.g.,~average throughput or spectral efficiency. Our results show that offline \ac{RL} can achieve the performance of online \ac{RL} and outperform practical state-of-the-art \ac{LA} based on \ac{OLLA}  when data is collected with a proper behavioral policy.



%% REMOVED 4 ARXIV %%
{\color{black}The rest of the paper is organized as follows. Section~\ref{sec:background}~introduces preliminary concepts, Section~\ref{sec:problem formulation} formally describes the problem of \ac{LA} while Section~\ref{sec:problem} presents the \ac{BCQ} and \ac{CQL} design for \ac{LA}. Section~\ref{sec:method} frames \ac{LA} as a sequence modeling problem, presenting a \ac{DT}-based design. Section~\ref{sec:experiments} discusses numerical results, while Section~\ref{sec:conclusion} concludes the paper.}

\begin{comment}
to employ \ac{BCQ}  and \ac{CQL} 
for \ac{LA} in 5G networks, which are
value-based algorithms for offline \ac{RL} \cite{fujimoto_off-policy_2019}, \cite{kumar_conservative_2020}.  
In its discrete variant, \ac{BCQ} tackles the distributional shift issue by restricting the support 
of action selection to a subset of actions whose probability is at least $\tau>0$ times the probability 
of the action most likely selected by the behavioral policy, \gf{where $\tau$ is ... }  \cite{fujimoto_benchmarking_2019}. 
In contrast, \ac{CQL} modifies the training objective to minimize -- alongside the Bellman error \cite{Sutton:14} -- 
the estimates of the Q-values to learn lower-bounded estimates that are not overly optimistic \cite{kumar_conservative_2020}.
%which is a known issue in offline \ac{RL}  \cite{kumar_conservative_2020}.
\gf{\it GF: Need $\sim 2$ more sentences on (1) why using BCQ and CQL is challenging to employ specifically for LA and (2) how we address these challenges (at a very high level), "the punch line". 
This is just a teaser that motivates the reviewer/reader to read further.}    

\sam{SAM: mention reason for data collection with dqn maybe}

\gf{\it GF: 1. Check the consistency across the title, abstract, index terms and intro. 2. The intro should not exceed 1 page.}

\textbf{Possible ways to present contributions}
\begin{itemize}
    \item focus more broadly on offline RL
    \item offline RL modelling for link adaptation using CQL, BCQ and DT. More effort needed to design DT.
    \item evelautaion with industrial simulator
    \item be open about data collection policy
    \item show that we can replicate performance of DQN, and discuss remaining problems
    \item future work...
\end{itemize}

\end{comment}






==> old_versions/backup_2024_11_17/2_background_20241118.tex <==
\section{Preliminaries}\label{sec:background}
This section reviews some of the key concepts and introduces notation that will be useful in the sequel.

\subsection{Elements of \ac{RL}}

\ac{RL} frames the interaction between an agent and the environment as a \ac{MDP} \cite{Sutton:14,puterman2014markov}, defined by the tuple: $(\mathcal{S, A, P}, r)$. Here, $\mathcal{S}$ is the state-space, $\mathcal{A}$ is the action-space, $\mathcal{P}$ is the transition probability function (also known as transition dynamics), $r:\mathcal{S}\times\mathcal{A}\times\mathcal{S}\to\mathbb{R}$ is the reward function.
In an online setting, at each time-step $t$ the agent chooses an action $a_t$ according to some Markovian policy $\pi:{\cal S}\to {\cal A}$, which is function of the current state $s_t$ of the MDP, and observes the next state $s_{t+1}$, distributed according to $P(\cdot|s_t,a_t)$, and a reward $r_t$. 
For episodic MDPs, with a finite terminal state, the goal of the agent is to find a policy $\pi$ maximizing the expected collected reward $\mathbb{E}^\pi[G_t|s_0\sim \mu]$ for some initial state distribution $\mu$, where
$
    G_t = \sum_{k=0}^T r_{t+k},
$
and $T$ indicates the terminal step. In the context of \textit{continuing task}, where $T$ is not naturally defined, or may be infinite, the goal is to maximize the collected discounted reward, defined with a  discount factor $\gamma\in (0,1)$ as $
    \mathbb{E}^\pi[\sum_{k=0}^\infty \gamma^k r_{t+k+1}|s_0\sim \mu]
$.
\begin{comment}
In settings where $T$ is not naturally defined, we introduce the notion of \textit{continuing task} and re-define the return to include the discount factor $\gamma$: $
    G_t = \sum_{k+0}^\infty \gamma^k r_{t+k+1}.
$
\end{comment}

\subsection{Offline RL}
Differently from the online RL setting, in offline RL \cite{levine_offline_2020} the agent learns a policy from a previously collected dataset of experiences $\mathcal{D} = \{( s_t^i, a_t^i, r_{t}^i,s_{t+1}^i)_i\}$ (collected using a behavioral policy $\pi_\beta$).
As a consequence, the amount of data, and its quality, play a crucial role in offline RL, since the agent is not able to interact with the environment in an online fashion to collect new data. 
%While the goal of offline \ac{RL} remains the maximization of returns, in this framework agents no longer interact with the environment during training to collect new transitions using a behavioral policy $\pi_\beta$. 
%Instead, the learning algorithm shall derive a sufficient understanding of the \ac{MDP} dynamics exclusively from transitions available in a static \textit{training dataset} $\mathcal{D} = \{( s_t^i, a_t^i, s_{t+1}^i, r_{t+1}^i)_i\}$ collected by a behavioral policy $\pi_\beta$ prior to training. 
The inability to explore the state-action space during training may result in a distributional shift between the distribution under which the policy $\pi$ is trained and the one on which it will be evaluated \cite{levine_offline_2020}.

To address this issue, some approaches constraint how much the learned policy $\pi$ differs from the behavioral policy $\pi_\beta$, while other methods penalize the learned $Q$-values. For example, with discrete action spaces, \ac{BCQ} tackles the distributional shift issue by restricting the support  of action selection to a subset of actions whose probability exceeds the probability  of the action most likely selected by the behavioral policy by a minimum threshold~\cite{fujimoto_benchmarking_2019}.
%
In contrast, \ac{CQL} \cite{kumar_conservative_2020} uses a \emph{pessimism} principle: it modifies the training objective to minimize -- alongside the Bellman error \cite{Sutton:14} -- the estimates of the Q-values to learn lower-bounded estimates that are not overly optimistic. A comprehensive survey can be found in~\cite{levine_offline_2020}.


 


\begin{comment}
    While the goal is still the maximization of returns, in the offline \ac{RL} framework agents no longer have the ability to interact with the environment and collect additional transitions using the behavioral policy. This limits the possibility of exploring the state-action space to the transitions included in a static \textit{training dataset} $\mathcal{D} = \{( s_t^i, a_t^i, s_{t+1}^i, r_{t+1}^i)_i\}$, forcing the learning algorithm to derive a sufficient understanding of the \ac{MDP} dynamics exclusively from the available transitions. The challenge addressed by offline \ac{RL} is the distributional shift between the distribution under which the function approximator (policy, value function, or model) is trained and the one on which it will be evaluated. The simplest solution consists in bounding the distributional shift by constraining how much the learned policy $\pi$ differs from the behavioral policy $\pi_\beta$, with different algorithms employing slightly different approaches. A comprehensive review can be found in~\cite{levine_offline_2020}.
\end{comment}

%\\

% \textcolor{blue}{This work is going to consider \ac{BCQ} \cite{fujimoto_off-policy_2019} and \ac{CQL} \cite{kumar_conservative_2020}, two of the main value-based algorithms for offline \ac{RL}. In its discrete variant, \ac{BCQ} \cite{fujimoto_benchmarking_2019} tackles the distributional shift issue by restricting the support of action selection to a subset of actions whose probability is at least $\tau$ times the probability of the action most likely to be selected by the behavioral policy. On the other hand, \ac{CQL} \cite{kumar_conservative_2020} modifies the training objective to minimize, alongside the Bellman error, the estimates of the Q-values to learn lower-bounded estimates that are not overly optimistic, which is a known issue in offline \ac{RL} }


%     \begin{figure*}
%     \centering
%     \begin{minipage}{.49\textwidth}
%     \includegraphics[width=\textwidth]{Figures/olla_v1.2.png}
%     \caption{Visual description of the functioning of Link Adaptation.}
%     \label{fig:olla schema}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{.49\textwidth}
%     \includegraphics[width=\textwidth]{Figures/sequence_1.png}
%     \caption{Episodes in our MDP formulation for LA. Each box represents a TTI, and acknowledgements use the same color as the transmission they respond to. Between TTI 5 and 7 two packets are active, with episodes 1 and 2 overlapping. \textcolor{red}{TODO: make picture more narrow}}
%     \label{fig:sequence_1}
%     \end{minipage}
% \end{figure*}

\subsection{Sequence Modeling and Decision Transformer} 
Sequence modeling involves training auto-regressive models (such as the \ac{DT} \cite{chen_decision_2021}) on sequential data to capture patterns and make future predictions. Since the goal in \ac{RL}~is~to produce a sequence of actions leading to high cumulative rewards, one can re-frame the RL problem in terms of sequence modeling.

The \ac{DT} is a particular auto-regressive architecture used in sequence modeling that exploits the capabilities of GPT2~\cite{radford_language_2019} to perform sequential decision making. For each time step $t$ of a trajectory, \ac{DT}  uses sequences of $3$ embedded tokens: the state $s_t$, the action $a_t$, and the \ac{RTG} $\hat R_t = \sum_{t'=t}^T r_{t'}$. 
At inference time the \ac{RTG} allows to condition the output of the network to generate optimal actions by specifying \textit{future target} returns.
% Note that it is of particular importance  the \ac{RTG}: at inference time it allows to condition the output of the network by specifying \textit{future target} returns.
The model is trained by predicting the action $a_t$ at each time-step of the sequence. Overall, this architecture allows to bypass the need for bootstrapping to propagate returns, one of the key destabilizing elements in offline \ac{RL}.






==> old_versions/backup_2024_11_17/3_problem_20241118..tex <==
\section{Problem Formulation}\label{sec:problem formulation}
We consider the problem of \ac{LA} in the downlink of multi-cellular \acp{RAN}. The aim of LA is to dynamically adapt the transmission rate of individual packet transmissions to time- and frequency-varying channel conditions and radio interference. In \ac{5G} systems, this is achieved by selecting a set of \ac{MCS} parameters encoded by an integer taking value in the range~$\{0,31\}$,  known as the \ac{MCS} index~\cite{3rd_generation_partnership_project_3gpp_technical_2024}. Each \ac{MCS} index corresponds to a modulation order, code rate, and spectral efficiency to be used for transmitting a data packet to the \ac{UE}.

State-of-the-art \ac{LA} algorithms used in real-time \acp{RAN} combine two control loops executed on a sub-millisecond~timescale: an \ac{ILLA} converts the latest \ac{CQI} reported by the \ac{UE} into an initial \ac{SINR} estimate; an \ac{OLLA} scheme adjusts such an estimate (e.g., to compensate inaccuracies or aging of the \ac{CQI}) based on the \ac{HARQ} feedback (i.e., either positive or negative acknowledgments) received from the \ac{UE} for previous packet transmissions. The goal of the \ac{OLLA} is to maximize the link spectral efficiency while adhering to a desired \ac{BLER} target. As variants of this approach are widely adopted in today's communication systems, we consider it as reference for performance comparison in Section~\ref{sec:experiments}. 



%In this section, we first present \ac{LA} as framed for solving it as a control problem and then provide a formulation as a \ac{MDP}: we are going to consider this alternative formulation for training and evaluation of value-based offline \ac{RL} methods as well as data collection.


    
%\subsection{Pure Control Formulation}\label{olla}
%Traditional \ac{LA} algorithms rely on the combination of an inner- and \ac{OLLA} to reconstruct an estimate of the \ac{UE} \ac{SINR}: the \ac{ILLA} converts a \ac{CQI} to an initial estimate according to some pre-defined, link level curves while \ac{OLLA} adjusts such an estimate to take into account uncertainties in the \ac{CQI} transmission by means of a feedback loop acting on the received \ac{HARQ} signals (i.e., either positive or negative acknowledgments). \Ac{OLLA} algorithms circumvent the inherent complexity in modeling link adaptation by fixing a target \ac{BLER} value, defined as the experienced frequency of packet retransmissions. %\textcolor{red}{However, while several transmissions are required for OLLA to converge to the \ac{SINR} adjustments meeting the desired \ac{BLER}, traffic for most \acp{UE} consists of short bursts of transmissions. Furthermore, most implementations require to specify a fixed \ac{BLER}, which is not optimal for all channel conditions. Figure \ref{fig:olla schema} provides a visual description of the \ac{LA} process, highlighting the different stages of the above-described solution. THIS MAY BE REMOVED AND STAY ONLY IN THE INTRO?}

==> old_versions/backup_2024_11_17/4_LA_as_offline_RL_20241118..tex <==
\section{Link Adaptation as an Offline RL Problem}\label{sec:problem}
This section explores how \ac{LA} can be solved with offline \ac{RL}. \sam{We propose a \ac{MDP} formulation enabling agents to learn from experiences generated by any \ac{UE} within the network, collected in static datasets in the form of $(s_t,a_t,r_{t+1},s_{t+1})$ tuples. Being particularly well-suited both for online and offline \ac{RL} approaches, we consider such a formulation not only for training \ac{BCQ} and \ac{CQL} agents but also for collecting data using a behavioral \ac{DQN} policy, trained online.}


% We begin by presenting our \ac{MDP} formulation of LA and then discuss how offline \ac{RL} methods, like \ac{BCQ} and \ac{CQL}, can be applied to solve this \ac{MDP} formulation.

%     \begin{figure}
%     \centering

%     \includegraphics[width=0.5\textwidth]{tikz_imgs}
%     \caption{Episodes in our MDP formulation for LA. Each box represents a TTI, and acknowledgements use the same color as the transmission they respond to. Between TTI 5 and 7 two packets are active, with episodes 1 and 2 overlapping. \textcolor{red}{TODO: make picture more narrow}}
%     \label{fig:sequence_1}
% \end{figure}

\begin{figure}
    \centering
    % Resize the combined TikZ images to fit within the column width
    \resizebox{\linewidth}{!}{%
    \input{tikz_imgs/img_harq_example}
    }
    \caption{Episodes in our \ac{MDP} formulation for LA. Each box represents a \ac{TTI}, and acknowledgments use the same color as the transmission they respond to. Note that episodes 1 and 2 overlap between \ac{TTI} 5 and 12.}
    \label{fig:sequence_1}
\end{figure}
\subsection{\ac{MDP} Formulation}  

We model \ac{LA} as an episodic \ac{MDP} in which an episode (or trajectory) $\tau=(s_0,a_0,r_0,\dots, s_T,a_T,r_T)$  corresponds to the lifespan of a \ac{UE}'s data packet from its first transmission to, alternatively, a successful reception or the packet being dropped after four retransmissions (as illustrated in~\cref{fig:sequence_1}). As such, the episode's length $T$ is bounded to five steps (each corresponding to a transmission of the packet).
\begin{itemize}
    \item The state $s_t \in \mathbb{R}^n$ is a  vector of semi-static and dynamic information characterizing the serving cell, the \ac{UE} design, as well as radio measurements, channel state information, \ac{HARQ} feedback, and more\footnote{The exact list of states cannot be disclosed as it is based on Ericsson's internal research work.}.
    \item The action $a_t\in \{0,\dots,27\}$ takes an integer, representing one of 28 \ac{MCS} indices for data transmissions, as defined by the \ac{5G} specifications~\cite{3rd_generation_partnership_project_3gpp_technical_2024}. When dealing with a re-transmission, that is $t\geq 1$,  the simulator maps the agent's action to a reserved \ac{MCS} index in the interval $\{28,\dots,31\}$, as per \ac{5G} specifications.
    \item  The reward signal $r_t=r(s_t,a_t)$ is function of the \ac{SE} of the packet transmission. 
\end{itemize}

Additionally, as the \ac{UE}'s \ac{HARQ} process supports multiple active packets at any given time, multiple \ac{UE}'s episodes may overlap in time (as in the example in~\cref{fig:sequence_1}). 

% \subsection{Solving LA with Offline \ac{RL}}
% The proposed \ac{MDP} modeling enables an \ac{RL} agent to learn from experiences generated by any \ac{UE} within the network. Hence, it is particularly well-suited both for online and offline \ac{RL} approaches thanks to the large amounts of data collected in the network. 

% We consider this formulation to train a \ac{DQN} policy  to serve as behavioral policy for data collection as well as performance reference for offline \ac{RL}. As training data samples for offline \ac{RL} consist of state-action-reward tuples $(s_t,a_t,r_t)$, we can consider the evaluation and training of value-based and actor-critic methods~\cite{Sutton:14}.  

% We propose two offline \ac{RL} algorithms for \ac{LA} based on \ac{BCQ}~\cite{fujimoto2019off}, and \ac{CQL}~\cite{kumar_conservative_2020}, respectively. 

% {\color{red}[@Alessio, @Samuele]: could we add a couple of sentences to indicate in what way you designed these algorithms for LA? It does not need to long}

%Training data samples for offline \ac{RL} are represented by state-action-reward tuples $(s_t,a_t,r_t)$, which allows for the evaluation and training of value-based and actor-critic methods \cite{Sutton:14}. Consequently, this formulation is particularly well-suited for use with offline \ac{RL}, as it can exploit the large amounts of data collected in the network to train a policy using a fixed dataset \cite{levine_offline_2020}.

%{\color{blue} [PS]: I would add here a description of the LA design based on BCQ and CQL and move the sequence modeling paragraph to the beginning of Sec IV}
\begin{comment}
  \paragraph{Sequence modeling}
However, there are some shortcomings with this modeling of LA. Firstly, such formulation optimizes only over one packet at the time, without considering sequences of multiple packets. Secondly, since packet arrivals are unknown and channel conditions are time-varying, the overall stochastic process we aim to control can be more generally framed as a \emph{contextual} \ac{MDP} \cite{hallak2015contextual}. A contextual \ac{MDP} is a specific type of \ac{MDP} that includes an underlying time-varying hidden parameter (context) affecting the transition dynamics—such as packet arrivals and channel conditions. Managing such a process is generally more complex than controlling a classical \ac{MDP} \cite{kaelbling1998planning}. To address these complexities, we propose a sequence modeling approach \cite{janner2021offline,emmons_rvs_2021}, a method to efficiently handle sequences of data.  
\end{comment}
    



==> old_versions/backup_2024_11_17/5_sequence_modelling_for_LA_20241118..tex <==
\section{Sequence Modeling for Link Adaptation}\label{sec:method}

The previous \ac{MDP} formulation of \ac{LA}, and thereby the related offline \ac{RL} designs,  present some shortcomings. Firstly, such formulation optimizes the return for individual packets. Thus, it may not capitalize that sequences of packets can experience correlated channel conditions that would allow to optimize longer-term metrics (e.g., \ac{UE} throughput). Secondly, since packet arrivals are unknown and channel conditions are time-varying, the overall stochastic process we aim to control can be more generally framed as a \emph{contextual} \ac{MDP} \cite{hallak2015contextual}. A contextual \ac{MDP} is a specific type of \ac{MDP} that includes an underlying time-varying hidden parameter (context) affecting the transition dynamics—such as packet arrivals and channel conditions. Managing such a process is generally more complex than controlling a classical \ac{MDP} \cite{kaelbling1998planning}. 

To address these complexities, this section reformulate \ac{LA} using a sequence modeling approach \cite{janner2021offline,emmons_rvs_2021}, a method to efficiently handle sequences of data. We then outline our contributions in adapting the original \ac{DT} design \cite{chen_decision_2021} to the \ac{LA} problem.

\subsection{RL via Supervised Learning (RvS)}
%Sequence modeling involves training auto-regressive models on sequential data to capture patterns and make future predictions. Since the main goal in \ac{RL} is to produce a sequence of actions leading to high cumulative rewards, we can re-frame the RL problem in terms of sequence modeling.

By framing RL as a sequence modeling problem, we can better capture the time-varying interactions in the underlying process. This approach simplifies various design decisions and leverages the strengths of sequence models in handling temporal dependencies.

We consider the \ac{RvS} learning approach for offline RL considered in \cite{emmons_rvs_2021}. This approach takes as input a dataset ${\cal D}=\{\tau\}$ of trajectories of experience and outputs an \emph{outcome-conditioned} policy $\pi_\theta(a_t\mid s_t,\omega)$ that optimizes
\begin{equation}
    \max_\theta \mathbb{E}_{\tau \sim {\cal D}}\left[\sum_{t=0}^{|\tau|-1} \mathbb{E}_{\omega \sim f(\omega\mid \tau_t)}\left[ \ln \pi_\theta(a_t\mid s_t,\omega)\right]\right],
\end{equation}
where $\tau_t=\{s_t,a_t,r_t,s_{t+1},\dots\}$ denotes the trajectory starting at time $t$, $|\tau|$ denotes the trajectory length, and $f(\omega|\tau)$  denotes the distribution over outcomes $\omega$ that occur in a trajectory. These outcomes are user-chosen, and can be, for example:
\begin{itemize}
    \item \emph{Goal-oriented}: $\omega=\{s_{h}=s\}$, that is, $f(\omega|\tau)$ indicates the likelihood of visiting state $s$ at step $h$.
    \item \emph{Reward-oriented}: $\omega=\sum_{n\geq t}\gamma^{n-t} r_n$, and $f(\omega|\tau)$ indicates the likelihood of achieving a certain total discounted  reward starting from $t$. Such conditioning is also referred to as \emph{return-to-go} (RTG).
\end{itemize}
At inference-time, then, the user can choose to condition the policy according to the desired objective.

\subsection{RvS Learning for LA}
To formulate  \ac{LA}  in terms of the \ac{RvS} learning framework, we introduce a trajectory definition that extends beyond the lifespan of a single packet, departing from the previous \ac{MDP} formulation.  After that, we introduce different ways to condition the policy $\pi_\theta$.
 %After that, we introduce our proposed reward-oriented conditioning, as well as  a particular type of ci
%This extension allows us to leverage a \ac{DT} approach for \ac{LA}, benefiting from the transformer's ability to perform long-term credit assignment by considering long sequences spanning multiple packet transmissions.


\subsubsection{Trajectory definition} \label{trajectory definition} We consider fixed-horizon trajectories $\tau=\{s_0,a_0,r_0,\dots, s_H,a_H,r_H\}$, which include  transmissions of packets belonging to a specific \ac{UE}.

%. Letting $3K$ denote the transformer's context size, each sequence can include tokens corresponding to up to $K$ transmissions, with extra positions filled using padding tokens.
We consider two alternative approaches to construct $\tau$:

\begin{enumerate}[label=\alph*)]
    \item \emph{Recent transmissions}:  $\tau$ consists of the most recent $K$ transmissions of the \ac{UE} considered (hence $H=K$).
    \item \emph{Consecutive packets}: $\tau$ includes only up to  $n_p$ of a \ac{UE}'s most recent consecutive packets. Since the maximum number of retransmissions is $5$, we have that $H\in\{n_p,\dots, 5n_p\}$.
\end{enumerate}
At training time, we sample trajectories of data from the dataset ${\cal D}$ using one of these two approaches, and, if needed, extra positions in  $\tau$ are filled using padding tokens.

% To formulate the \ac{LA} functionality as a sequence modeling problem, we introduce a trajectory definition that departs from the previous \ac{MDP} formulation and extends the episode horizon beyond the lifespan of a packet. This allows us to leverage a \ac{DT} approach for \ac{LA} and benefit from the transformer's ability in performing long-term credit assignment by considering long sequences of tokens that span across transmissions for multiple packets. Specifically, we define a trajectory to include all the transmissions of packets belonging to a certain \ac{UE} in a simulation. Letting $3K$ denote the context size of the transformer, tokens relative to up to $K$ transmissions can be included in each sequence, with extra positions being filled with padding tokens. We consider two alternative approaches: (1) a sequence consisting of the most recent $K$ transmissions relative to a certain \ac{UE}; (2) a sequence including transmissions relative to $n_p$ of a \ac{UE}'s most recent consecutive packets. Considering~$5$ as the maximum number of retransmission, each sequence will include a number of transmissions in $[n_p, 5n_p]$. 



% \subsection{DT design modifications}
% \label{DT modifications}
% \ac{LA} has some fundamental differences when compared to standard \ac{RL} baselines such as those considered in the original \ac{DT} paper \cite{chen_decision_2021}. In this section, we present the main modifications to its design that we found necessary for our use case.


\subsubsection{Outcome conditioning}\label{subsec:conditioning} We propose the following three ways to condition the policy $\pi_\theta$:
\begin{enumerate}[label=\alph*)]
    \item {\bf VANILLA}: This is a simple conditioning that consists in fixing a target \ac{RTG} value $\omega$ for each packet $p$. At training time, the \ac{RTG} at the $k$-th step of a packet is computed as  $\omega=\sum_{t=k}^{T(p)} \gamma^{t-k} r_k(p)$, where $r_k(p)$ indicates the reward associated to the $k$-th transmission for packet $p$, $\gamma \in(0,1]$, and  $T(p)$ is a random variable indicating the termination step for the transmission of packet $p$. At inference time, the \ac{RTG} is fixed to a pre-defined value at the first transmission and adjusted in case of retransmissions (we expand on this in~\cref{sec:experiments}).

    \item {\bf DAVG}: The VANILLA approach has the same shortcomings of the MDP formulation proposed in \cref{sec:problem}. An alternative is to condition according to a discounted average of  future rewards. Letting $n$ denote the $n$-th step in a sequence of continuous transmissions from a UE, at training time we condition according to:
    \[
           \omega=(1-\gamma)\sum_{t=n}^\infty \gamma^{t-n}r_t,
    \]
    with $\gamma \in(0,1)$.   At inference time, as for the VANILLA case, we condition according to some pre-defined value.
    \item {\bf 3GPP}: Lastly, we propose a novel conditioning method based on the observation that the reward signal, as mentioned in \cref{sec:problem}, is directly related to the spectral efficiency of the channel. Therefore, we condition the policy $\pi_\theta$ according to a nominal spectral efficiency value given the channel quality. Specifically, at each first packet transmission, depending on the \ac{CQI} value reported by the \ac{UE} in the state $s$, we use the corresponding nominal spectral efficiency from the \ac{CQI} Table 5.2.2.1\text{-}3 of the \ac{3GPP} specification~\cite{3rd_generation_partnership_project_3gpp_technical_2024} as the target \ac{RTG} value.
\end{enumerate}






% When shifting to a trajectory definition including all of a \ac{UE}'s transmissions it becomes unfeasible to compute \acp{RTG} on an infinite horizon. Furthermore, in radio communications, packets’ transmissions that are distant in time are roughly independent and the knowledge about future rewards is unlikely to be useful for generating optimal actions for earlier packets. Taking inspiration from the framework described by Emmons et al. in \cite{emmons_rvs_2021}, we propose the following expression as a new objective definition for \ac{LA}:

% \begin{itemize}
%     \item VANILLA: 
%         \begin{equation}
%             V(p)=\mathbb{E}\left[\sum_{k=0}^{T(p)} r_k(p)\right].
%         \end{equation}
%     \item AVG
%         \begin{equation}
%             RTG(i_0)=\mathbb E_{\tau \sim \mathcal{D}} \left[\sum_{i=i_0}^{|\tau|-1} \gamma_0^{i-i_0}r_i\right], 
%         \end{equation}
% \end{itemize}

% \begin{equation}
% \label{equation:final objective definition}
%     \mathbb E_{\Upsilon \sim \rho} \left[\sum_{n=n_0}^\infty \gamma_0^{t_n-t_{n_0}}V(p_n)\right], 
% \end{equation}
% where with $V(p)$ we refer to the value of a packet, defined as:
% \begin{equation}
%     V(p)=\mathbb{E}\left[\sum_{k=0}^{T(p)}\gamma_1^k r_k(p)\right].
% \end{equation}

% In such a formulation, $\Upsilon$ denotes a sequence of packets transmitted at random times, where $\rho$ is the distribution over packets and time. $\gamma_0$ and $\gamma_1$ are discount factors respectively affecting the sum of the values of successive packets and successive retransmissions for a single packet. $t_n$ is the time of transmission of packet $n$, with $t_{n_0}$ being the time of transmission of the first packet of the sequence. $T(p)$ is a random variable indicating the termination step for the transmission of packet $p$. Finally, $r_k(p)$ indicates the reward associated to the $k$-th transmission for packet $p$.

% The formulation is general enough that by setting $\gamma_0=0$ the objective converges to a packet basis, similar to the objective for the formulation described in \ref{MDP formulation}; by choosing $0 < \gamma_0 < 1$ the objective instead becomes a discounted sum of future rewards. We can imagine the first case as conditioning \ac{DT} on intermediate goals for each packet. 

% \textcolor{blue}{In the following sections we present results obtained by setting $\gamma_0 = 0$ or, alternatively, by simply computing average returns on a window with fixed size of $M$ transitions, discounting rewards at each transmission.}


% \subsubsection{Conditioning at inference}
% At inference time, we propose three different ways of conditioning the generation of actions. (1) \textbf{VANILLA} consists in fixing a target \ac{RTG} value $\omega$ for each packet, $\omega$ is fixed at the first transmission and adjusted in case of retransmissions; (2) \textbf{3GPP}, similarly to VANILLA, at each first packet transmission selects a target \ac{RTG} value according to the \ac{3GPP} \ac{CQI} Table 5.2.2.1-3 in \cite{3rd_generation_partnership_project_3gpp_technical_2024}, depending on the \ac{CQI} value reported by the \ac{UE} inside the state; (3) \textbf{AVG} conditions each step with the same value of average \ac{RTG} as a target. 

\subsection{Decision Transformers Design for LA}

Hereafer, we describe how we adapted the \ac{DT} architecture for the link adaptation problem. We introduce two changes: one to the attention layer, and one for the positional embedding.
\begin{figure}[t]
    \centering
    % Resize the combined TikZ images to fit within the column width
    \resizebox{\linewidth}{!}{%
    \input{tikz_imgs/img_attention_mask}
    }
    \caption{\textbf{At training time}, the modified definition of the attention mask (right matrix) prevents the tokens associated to $p_2$ and $p_4$ from attending $p_1$, as its reward is not available at the time an MCS index is requested for $p_2$ and $p_4$. The left matrix shows the original attention mask definition.}
    \label{fig: attn mask}
\end{figure}


% \begin{figure}
%     \centering
%     % Resize the combined TikZ images to fit within the column width
%     \resizebox{\linewidth}{!}{%
%     \input{tikz_imgs/img_sequence_builing}
%     }
%     \caption{Given a trajectory $\tau$ (relative to a single \ac{UE}), input sequence (a) is built by setting $K=4$ while sequence (b) is built with $n_p=2$. The first index in the notation $t_{i,j}$ identifies the transmission count while the second is a unique packet id. A same color also identifies transmissions for a same packet.}
%     \label{fig: sequence building}
% \end{figure}

\subsubsection{Attention masking for delayed feedback}

A significant challenge in training a \ac{DT} architecture for \ac{LA} is preventing the leakage of future data during the training process. To perform inference, historical rewards are only available upon a base station receiving a \ac{HARQ} feedback (either positive or negative) for previous packet transmissions. Consequently, it is essential to ensure that \ac{DT}'s outputs during training rely solely on information available in real-time, avoiding any use of future data that would not be accessible in an actual deployment.

To describe the proposed modification we need to introduce some notation. First, for a trajectory: \[\tau=(\underbrace{s_0}_{X_{0}},\underbrace{a_0}_{X_1},\underbrace{r_0}_{X_2},\dots, \underbrace{s_K}_{X_{3K}}, \underbrace{a_K}_{X_{3K+1}}, \underbrace{r_K}_{X_{3K+2}}),\]
let $(X_0, X_1,\dots, X_{3K+2})$ be the corresponding sequence of tokens fed as input to the \ac{DT}. Secondly, define $t_a(p)$ and $t_r(p)$ to be the instants in time at which, respectively,  the action for packet $p$ is scheduled and the associated reward signal is available. Lastly, indicate by $p(X)$ the mapping $X\mapsto p$ between a token to the corresponding packet. Then, the attention mask between any two tokens $X_i,X_j $ is given by:
\[
\hbox{\texttt{attn\_mask}}(X_i,X_j) = \mathbf{1}\{ t_r(p(X_i)) \leq t_a(p(X_j))\}.
\]
 In other words, if we have not yet received any reward for packet $p(X_i)$, then the tokens of the packet $p(X_j)$ should not be affected by the tokens of packet $p(X_i)$. \cref{fig: attn mask} describes such a formulation visually.

\input{plots}
% Formally, by referring to the instant in time at which the action for packet $i$ is scheduled with $t_{a,i}$ and the instant in time the associated reward signal is received with $t_{r,i}$, we apply:
% \begin{align}
%         \begin{array}{rcl}
%             \text{given a sequence of tokens }\left[T_0, T_1, ..., T_{3 \cdot \text{seq\_len}-1} \right], \\
%             \forall T_i,T_j, \text{ if } t_{r,i} > t_{a,j} \text{ then } attn(i,j) = -\infty,
%         \end{array}
%     \end{align}
% where $attn(i,j)$ represents the un-normalized attention score between token~$i$~and~$j$. 



\subsubsection{Temporal embeddings}
% \ac{LA} is a real-time process where states (sim. actions) are observed at points in time that are not equidistant between each other. The DT architecture was designed for processes with an equidistant sampling. We propose to capture the correlation in time between successive packet transmissions by modifying the \ac{DT} positional encoding. 
\ac{LA} is a real-time process with states (sim. actions) observed at irregular intervals, whereas the \ac{DT} architecture assumes equidistant sampling. To capture the temporal correlations between successive packet transmissions of a \ac{UE}, we consider the following modifications of the \ac{DT}'s positional encoding:
\begin{enumerate}
    \item \textbf{\Ac{BE}}: as a baseline, we implement a minor modification to the original encoder from \cite{chen_decision_2021}, where embeddings are learned based on each token's index within the sequence ($i \in [0, K-1]$).
    \item \textbf{\Ac{LT} encoding}: 
    embeddings are learned using a linear layer with $(\Delta {t}_i)_{i=0}^K$ as input, where $\Delta t_i= t_a(p(X_i)) - t_a(p(X_0))$. Hence, $\Delta {t}_i$ is a measure of the relative time  between the $i$-th token and the first one.
    Note that tokens within the same packet have identical relative timestamps, allowing the \ac{DT} to associate the reward to the corresponding state and action.

    \item \textbf{\Ac{CT} encoding}: inspired by \cite{zuo2020transformer, zhang2023continuous},  the $k$-th element of the positional embedding vector for token $X_i$ is computed as:
\begin{equation}
    PE(\Delta t_i, k) = \begin{cases}
    \sin\left(\displaystyle \frac{\Delta t_i / 100}{{C}^{\frac k {d_\text{model}}}}\right) & \text{ for even } k, \\[4ex]
    \cos\left(\displaystyle \frac {\Delta t_i / 100} {C^{\frac {k-1} {d_\text{model}}}}\right) & \text{ for odd } k,
    \end{cases}
    \end{equation}
    where $d_{\text{model}}$ is a user-chosen constant (see also  \cite{zhang2023continuous}).
\end{enumerate}


==> old_versions/backup_2024_11_17/6_experiments_20241118..tex <==
\section{Numerical Results}\label{sec:experiments}
In this section, we empirically compare the considered offline \ac{RL} methods using an industry-grade simulator. We evaluate their performance in terms of throughput, experienced \ac{BLER}, and \ac{UE} \ac{SE} across all \ac{MIMO} layers allocated for transmission. Specifically, we investigate: (1) whether offline \ac{RL} methods can match the performance of the behavioral policy and of OLLA; (2) how the behavioral policy affects performance of these methods; and (3) whether our modifications to the \ac{DT} design improve \ac{LA} performance.

% This section compares empirically the results of the considered offline \ac{RL} methods with an industry-grade simulator. We  assess their performance in terms of throughput, experienced \ac{BLER} and \ac{UE} \ac{SE}, computed across all \ac{MIMO} layers allocated for the transmission.
% Specifically, we want to address the following points: (1)~whether offline \ac{RL} methods can match the performance of the behavioral policy and the considered baselines; (2)~how much the performance is affected by the behavioral policy; (3)~whether the modifications to the \ac{DT} design are useful for improving \ac{LA} performance.

\subsection{Environment, Methods and Data Collection}
\label{subsec:collection}
We now describe: the environment used to collect the data and test the methods; the methods considered in simulations; the data collection process.
\subsubsection{Environment} All simulations have been run on an internal Ericsson \ac{RAN} simulator platform compliant with the \ac{3GPP} \ac{5G} standard specification. The software infrastructure allows running multiple independent network simulations of pre-defined length in parallel, each specifying a different seed. 
%All simulations consider a multi-cell \ac{mMIMO} system with \acp{UE} randomly dropped in the simulated network area and full buffer traffic. 
We consider a \ac{TDD} 5G system operating at a 3.5GHz carrier frequency, with PHY layer numerology $\mu=0$ of the \ac{3GPP} technical specifications 38.211 and \ac{SU-MIMO} transmission.
%single-user Multi-Input Multi-Output (SU-MIMO) transmission. 
Each base station is configured with a \ac{mMIMO} %MIMO (mMIMO) 
8x4x2 antenna array. 
We consider 1 site, 3 sectors, and a fixed number of 10 UEs with full buffer traffic, thereby experiencing stable interference conditions.  For each simulation (i.e., a seed) the duration is 5 seconds.

\subsubsection{Methods} We compare the performance of two value-based offline \ac{RL} algorithms, \ac{BCQ} \cite{fujimoto2019off} and \ac{CQL} \cite{kumar_conservative_2020}, with \ac{DT}. 
%In its discrete variant, \ac{BCQ} \cite{fujimoto_benchmarking_2019} tackles the distributional shift issue by restricting the support of action selection to a subset of actions whose probability is at least $\tau$ times the probability of the action most likely to be selected by the behavioral policy. On the other hand, \ac{CQL} \cite{kumar_conservative_2020} modifies the training objective to minimize, alongside the Bellman error, the estimates of the q-values to learn lower-bounded estimates that are not overly optimistic, which is a known issue in offline \ac{RL}. We design the \ac{DT} agent as described in Section \ref{DT modifications}. Choices regarding the hyperparameters are detailed in Table \ref{table: hyperparameters}.
Three baselines have been considered. The first one is the \ac{OLLA} approach introduced in  \cref{sec:problem formulation}, the second one is simple \ac{BC} and as a last one we consider the performance of the behavioral \ac{DQN} policy. Performance evaluation has been conducted across $50$ randomized scenarios simulations, choices regarding the hyperparameters are detailed in the appendix. 
%Table \ref{table: hyperparameters}


\subsubsection{Data Collection}
We collected training data by interacting with the environment using two DQN policies. A first dataset, $\mathcal{D}_{\rm opt}$, was collected using a DQN policy $\pi_{\rm opt}$ that was trained until convergence; a second dataset, $\mathcal{D}_{\rm s-opt}$, was collected using a DQN policy $\pi_{\rm s-opt}$ that was trained on half the data (compared to $\pi_{\rm opt}$). This approach tests whether offline RL algorithms can infer optimal behavior from non-optimal training data in LA. %Additionally, we logged a unique ID for each UE requesting transmission alongside each transition tuple, allowing us to reconstruct sequences of packets for each UE.
We collected data across $20$ seeds, resulting in datasets of $\sim 400K$ transitions. The two \ac{DQN} policies have been trained online on, respectively, $100$ seeds for collecting $\mathcal D_\text{opt}$, and $50$ for $\mathcal D_\text{s-opt}$. %\sam{sam: should we mention d3rlpy?}


% We generated 150 randomized scenarios during training that randomize across several variables (e.g., UEs movement and traffic). Each scenario lasted $5$ seconds.  

% Additional simulation assumptions related to the network scenario are summarized in Table 7.1 (values per simulation seed).


% Training data is collected by direct interaction with the environment using a previously trained \ac{RL} policy.  We choose to consider two training datasets, $\mathcal{D}_\text{opt}$ and $\mathcal{D}_\text{s-opt}$, respectively containing optimal and sub-optimal behavior. Both are collected with a \ac{DQN} policy: while the first one is trained up to convergence, the second one is trained on half the data. By doing this, we hope to put to the test the potential of offline \ac{RL} algorithms to infer optimal behavior even from non-optimal training data in \ac{LA}.  Additionally, we found it helpful to log a unique ID associated with the \ac{UE} requesting the transmission alongside the tuple representing each transition. This allows us to reconstruct sequences of packets for each \ac{UE}.

% \textcolor{red}{We believe that similar findings would be obtained by training on datasets containing real-world data collected by the currently deployed rule-based algorithms. REMOVE AND TALK IN THE INTRODUCTION}






\begin{table*}[t!]
\centering
\begin{minipage}{0.48\linewidth}  % First table in half of the page width
    \centering
    \caption{Comparison of the offline RL methods trained on $\mathcal{D}_{\rm opt}$. \\ OLLA (x\%) refers to OLLA with a fixed BLER target of x\%.}
    \setlength{\tabcolsep}{8pt} % Adjust the column spacing
    \begin{tabular}{lccc}
    \hline
    \toprule\toprule
        \ac{LA} algorithm & Throughput & \ac{SE} & \ac{BLER} \\
    \toprule
        OLLA ($10\%$) & 14.76 Mbps   & 6.21 bps/Hz   & 0.13     \\
        OLLA ($30\%$) & 15.51 Mbps   & 6.87 bps/Hz   & 0.30     \\
        OLLA ($50\%$) & 15.16 Mbps   & 6.92 bps/Hz   & 0.49     \\
        OLLA ($70\%$) & 14.77 Mbps   & 6.81 bps/Hz   & 0.66     \\
        OLLA ($90\%$) & 14.71 Mbps   & 6.84 bps/Hz   & 0.83     \\
        DQN$_{\rm opt}$   & 16.02 Mbps   & 7.50 bps/Hz   & 0.32     \\
        BC            & 16.10 Mbps   & 7.53 bps/Hz   & 0.30     \\
        BCQ           & 16.11 Mbps   & 7.53 bps/Hz   & 0.30     \\
        CQL           & 16.10 Mbps   & 7.52 bps/Hz   & 0.30     \\
        DT            & 16.07 Mbps   & 7.46 bps/Hz   & 0.31     \\
    \bottomrule\bottomrule
    \hline
    \end{tabular}
    \vspace{0.25cm} % Adjust vertical space between table and caption
    \label{table: opt table}
\end{minipage}
\hspace{0.02\linewidth}  % Small space between the two tables
\begin{minipage}{0.48\linewidth}  % Second table in half of the page width
    \centering
    \caption{Comparison of the offline RL methods trained on $\mathcal{D}_{\rm s-opt}$. \\ OLLA (x\%) refers to OLLA with a fixed BLER target of x\%.}
    \setlength{\tabcolsep}{8pt} % Adjust the column spacing
    \begin{tabular}{lccc}
    \hline
    \toprule\toprule
        \ac{LA} algorithm & Throughput & \ac{SE} & \ac{BLER} \\
    \toprule
        OLLA ($10\%$) & 14.76 Mbps   & 6.21 bps/Hz   & 0.13     \\
        OLLA ($30\%$) & 15.51 Mbps   & 6.87 bps/Hz   & 0.30     \\
        OLLA ($50\%$) & 15.16 Mbps   & 6.92 bps/Hz   & 0.49     \\
        OLLA ($70\%$) & 14.77 Mbps   & 6.81 bps/Hz   & 0.66     \\
        OLLA ($90\%$) & 14.71 Mbps   & 6.84 bps/Hz   & 0.83     \\
        DQN$_{\rm s-opt}$ & 15.89 Mbps   & 7.45 bps/Hz   & 0.33     \\
        BC            & 16.00 Mbps   & 7.50 bps/Hz   & 0.31     \\
        BCQ           & 16.00 Mbps   & 7.60 bps/Hz   & 0.34     \\
        CQL           & 16.05 Mbps   & 7.59 bps/Hz   & 0.33     \\
        DT            & 15.67 Mbps   & 7.25 bps/Hz   & 0.36     \\
    \bottomrule\bottomrule
    \hline
    \end{tabular}
    \vspace{0.25cm} % Adjust vertical space between table and caption
    \label{table: s-opt table}
\end{minipage}
\end{table*}


\subsection{General Results}

\cref{table: opt table,table: s-opt table} present the  results of in terms of throughput, \ac{BLER} and \ac{SE}: offline \ac{RL} models in  \cref{table: opt table} have been trained on $\mathcal{D}_{\rm opt}$, while models in  \cref{table: s-opt table} on $\mathcal{D}_{\rm s-opt}$. When considering $\mathcal{D}_{\rm opt}$, we notice how the offline \ac{RL} methods achieve comparable results across all the considered metrics, with \ac{CQL} and \ac{BCQ} scoring slightly better than \ac{DT}. Yet, they are only able to match the performance of the \ac{BC} baseline.
However, when considering suboptimal training data $\mathcal{D}_{\rm s-opt}$, the differences are more noticeable.   \ac{CQL} reaches almost the same performance as models trained on $\mathcal{D}_\text{opt}$  in terms of \ac{SE}. On the other hand, when trained on data that is suboptimal, \ac{DT} is not able to match the performance of the behavioral policy. Our results for both settings show that \ac{BC} seems to work sufficiently well on this use-case. \sam{Plots in Fig. \ref{cdf} look at the CDF curves resulting from the experiments on $\mathcal{D}_{\rm opt}$.




\subsection{Considerations on the \ac{DT} design}
In \cref{table:pe and conditioning - throughput} we show results for different combinations of the positional encoder and conditioning methods proposed in  \cref{sec:method} for the Decision Transformer (we only consider results obtained by training on $\mathcal{D}_\text{opt}$).

Including temporal information about packet distribution using the \ac{LT} encoding appears to be beneficial compared to both BE and \ac{CT} encoding, with these two achieving similar performance. Specifically, learning embeddings directly from the actual timestamps of packet transmissions leads to substantial performance improvements, while using an encoding based on trigonometric functions (i.e., \ac{CT}) results in worse performance.

%Including information about the distribution of packets in time with the use of \ac{LT} encoding appears to be beneficial with respect to both the BE and \ac{CT} encoding, with these two achieving very similar performance. Interestingly, using the timestamps of packet transmissions to learn embeddings (i.e.: \ac{LT}) brings substantial improvements to performance, while an encoding based on trigonometric functions (i.e.: \ac{CT}) achieves worse performance. 

Regarding \ac{RTG} conditioning, our results in \cref{table:pe and conditioning - throughput} indicate that \ac{3GPP} conditioning achieves better throughput than both VANILLA and DAVG conditioning across all types of positional encoding. We observed similar results in terms of \ac{BLER} and \ac{SE}, which are not included here for brevity. This evidence supports our hypothesis that conditioning differently based on channel conditions is beneficial.

%Concerning \ac{RTG} conditioning, our results in  \cref{table:pe and conditioning - throughput} indicate that \ac{3GPP} conditioning achieves better throughput\footnote{We observed similar results in terms of \ac{BLER} and \ac{SE}, which are not included for ease of presentation.} compared to VANILLA and AVG conditioning, across all types of positional encoding. This evidence supports our hypothesis that it is reasonable to condition differently depending on the channel conditions.

For the VANILLA and DAVG conditioning types, we conditioned on the 90\% quantile of the distribution of RTGs in the training dataset (filtered at the first retransmission in the case of VANILLA conditioning). The average future rewards are computed over a fixed window size of $35$ steps, with a discount factor $\gamma = 0.8$. The results reported here have been obtained following the first of the two approaches to trajectory definition introduced in Section \ref{trajectory definition}, with $H=32$.

 %Results for the VANILLA and AVG conditioning types are obtained by conditioning on the $90\%$ quantile of the distribution of \acp{RTG} in the training dataset (filtered at the first retransmission, in case of vanilla conditioning). \textcolor{red}{Average, future rewards are computed on a fixed window size of $35$ steps, with $\gamma=0.8$.}


\begin{table}[]
\centering
\caption{Comparison of different types of position encoding and RTG conditioning. Best in \textbf{bold}, second best in red.}
\renewcommand{\arraystretch}{1.25}
\begin{tabular}{lccc}
\toprule\toprule
PE type    & VANILLA       & 3GPP          & DAVG           \\ \hline
BE          & 15.75 Mbps & 15.83 Mbps & 15.76 Mbps \\
CT              & 15.35 Mbps & 15.86 Mbps & 15.73 Mbps \\
LT & \textcolor{red}{16.01 Mbps} & \textbf{16.07 Mbps} & 15.66 Mbps \\
\bottomrule\bottomrule
\end{tabular}
\label{table:pe and conditioning - throughput}
\end{table}

\subsection{Analysis of Outcome Conditioning}
\label{RTG conditioning}

\begin{table}[t!]
    \centering
    \setlength{\tabcolsep}{3pt}
    \caption{Performance obtained by conditioning on increasing, fixed, RTG values at inference for models including variable numbers of packets inside their sequence (vanilla).}
    \begin{tabular}{llllll}
    \toprule\toprule
    $n_p$ & Metrics      & 3GPP     & $\omega=1.71$  & $\omega=3.86$ & $\omega=7.57$ \\ \hline
         & Th.put    & 15.73 Mbps & 15.30 Mbps & 13.80 Mbps & 13.94 Mbps \\
    1    & BLER          & 0.37       & 0.33       & 0.42       & 0.83       \\
         & SE            & 7.45 bps/Hz & 7.14 bps/Hz & 6.92 bps/Hz & 7.19 bps/Hz \vspace{3mm} \\
         & Th.put    & 15.72 Mbps & 15.08 Mbps & 13.75 Mbps & 13.98 Mbps \\
    2    & BLER          & 0.38       & 0.31       & 0.41       & 0.82       \\
         & SE            & 7.45 bps/Hz & 7.08 bps/Hz & 6.87 bps/Hz & 7.25 bps/Hz \vspace{3mm} \\
         & Th.put    & 16.02 Mbps & 15.93 Mbps & 15.45 Mbps & 14.06 Mbps \\
    4    & BLER          & 0.31       & 0.28       & 0.36       & 0.74       \\
         & SE            & 7.43 bps/Hz & 7.32 bps/Hz & 7.45 bps/Hz & 7.46 bps/Hz \vspace{3mm} \\
         & Th.put    & 16.04 Mbps & 16.01 Mbps & 15.96 Mbps & 14.49 Mbps \\
    8    & BLER          & 0.28       & 0.27       & 0.30       & 0.62       \\
         & SE            & 7.40 bps/Hz & 7.34 bps/Hz & 7.42 bps/Hz & 7.56 bps/Hz \vspace{3mm} \\
         & Th.put    & 16.02 Mbps & 15.93 Mbps & 15.45 Mbps & 14.06 Mbps \\
    12   & BLER          & 0.31       & 0.30       & 0.31       & 0.46       \\
         & SE            & 7.45 bps/Hz & 7.42 bps/Hz & 7.46 bps/Hz & 7.58 bps/Hz \vspace{3mm} \\
         & Th.put    & 16.02 Mbps & 15.93 Mbps & 15.45 Mbps & 14.06 Mbps \\
    16   & BLER          & 0.30       & 0.29       & 0.31       & 0.40       \\
         & SE            & 7.44 bps/Hz & 7.42 bps/Hz & 7.44 bps/Hz & 7.48 bps/Hz \\
    \bottomrule\bottomrule
    \end{tabular}
    \label{table: more-packets}
\end{table}

In this section, we analyze the \ac{RTG} conditioning of the \ac{DT}, as discussed in \cref{subsec:conditioning}. We start by considering input sequences that comprise transmissions related to a single packet (i.e., $n_p=1$), we then extend the analysis by incrementally increasing the number of packets included in the input sequences. This approach allows us to better observe the effect of conditioning on different \ac{RTG} values during inference and to determine the extent to which the \ac{DT} can replicate the target \ac{RTG} values.

%In this section we analyse the \ac{RTG} conditioning of the DT, as discussed in \cref{subsec:conditioning}. We start by considering input sequences comprising transmissions relative to one single packet (i.e.: $n_p=1$) and then extend the analysis to include an increasing number of packets to better observe the effect of conditioning on different values at inference and find out to what extent \ac{DT} can replicate target \ac{RTG} values.

\Cref{table: more-packets} shows the performance of \ac{DT} when we vary the target \ac{RTG} value $\omega$ across the $q\%$ quantiles of the training \ac{RTG} distribution, with $q\in \{20,60,100\}$. As expected, conditioning the action generation on higher target \ac{RTG} values causes the \ac{DT} to take more aggressive actions and leads to an increased frequency of retransmissions during testing, reflected by a higher \ac{BLER}. Conversely, we observe a decreasing trend in throughput, with the \ac{3GPP} baseline achieving the best performance due to the induced correlation between the target \ac{RTG} values and the channel conditions.

% \cref{table: more-packets} shows the performance of \ac{DT} by sweeping the value of the target \ac{RTG} value $\omega$ over the $q\%$ quantiles of the training distribution of \acp{RTG} (with $q \in [0.2, 0.6, 1.0]$). As expected, conditioning the generation of actions on increasing target values of \ac{RTG} causes \ac{DT} to take more aggressive actions and, as a consequence, retransmissions at inference time increase in frequency (\ac{BLER}); at the same time, we notice an opposite trend in terms of throughput, with \ac{3GPP} achieving yet again the best performance because of the induced correlation between the target value and channel conditions.

As we include more packets in the sequences, the average performance tends to improve. However, when experiments involve sequences with eight or more packets, the \ac{BLER} values converge to those achieved by the behavioral DQN policy. These results imply that while the \ac{DT} can effectively model short sequences of packet transmissions, incorporating longer sequences likely introduces too much variance. This increased variance may cause the \ac{DT} to default to simply cloning the behavioral policy, as suggested by the poor performance shown in \cref{table: s-opt table}. Consequently, this effect prevents the 
\ac{DT} from extrapolating optimal behavior from suboptimal data. \sam{See the Appendix in the complete version of the paper for more on this (ArXiv: https://arxiv.org/abs/2410.23031).}

%As more packets are included inside sequences, average performance seems to increase. However, alues of \ac{BLER} achieved across experiments with $8$ or more packets seem to converge to the value of \ac{BLER} achieved by the behavioral \ac{DQN} policy. These results imply that, while \ac{DT} seems to be able to correctly model short sequences of packet transmissions, considering longer sequences probably introduces too much variance causing \ac{DT} to revert to simple cloning of the behavioral policy and, as suggested by the poor performance shown in  \cref{table: s-opt table}, preventing the extrapolation of optimal behavior from suboptimal data.

% According to the definition introduced in Section \ref{DT modifications}, we start by considering input sequences comprising transmissions relative to one single packet (i.e.: $n_p=1$) to better observe the effect of conditioning on different values at inference and find out to what extent \ac{DT} can replicate target \ac{RTG} values.

% Table \ref{table:1-packet sweep} shows the performance of \ac{DT} by sweeping the value of the target \ac{RTG} value $\omega$ over the $q\%$ quantiles of the training distribution of \acp{RTG} (with $q \in [0.1, 0.2, ..., 1.0]$). As expected, conditioning the generation of actions on increasing target values of \ac{RTG} causes \ac{DT} to take actions that are more aggressive and, as a consequence, retransmissions at inference time increase in frequency (\ac{BLER}). Consequently, we observe that conditioning on a single high return regardless of channel conditions leads to worse throughput performance; indeed, Table \ref{table:pe and conditioning - throughput} shows that the best throughput is achieved by \ac{3GPP} conditioning, which correlates the \ac{RTG} conditioning variable to the observed channel state.

% Table \ref{table: more-packets} extends the very same analysis to include increasing numbers of packets inside input sequences. Similarly to what we could observe in the previous case, as we condition on bigger $\omega$ values the experienced \ac{BLER} grows and, at the same time, we notice a decreasing trend in terms of throughput; with \ac{3GPP} conditioning achieving yet again the best performance. Unsurprisingly, as longer input sequences are considered, we experience better results across all metrics (with a maximum found at $n_p=8$). However, the values of \ac{BLER} achieved across experiments with $8$ or more packets seem to converge to the value of \ac{BLER} achieved by the behavioral \ac{DQN} policy. These results imply that, while \ac{DT} seems to be able to correctly model short sequences of packet transmissions, considering longer sequences probably introduces too much variance causing \ac{DT} to revert to simple cloning of the behavioral policy and, as confirmed by the poor performance shown in Table \ref{table: s-opt table}, preventing the extrapolation of optimal behavior from suboptimal data.

==> old_versions/backup_2024_11_17/7_conclusions_20241118..tex <==
\section{Conclusion}\label{sec:conclusion}
In this paper, we explored offline \ac{RL} approaches for \ac{LA}. %Link Adaptation (LA). 
Our simulations showed offline \ac{RL} methods, being able to match the performance of state-of-the-art online \ac{RL} methods, to constitute a viable alternative to solve \ac{LA}. However, as mentioned in Section \ref{sec:introduction}, further work should be directed toward the study of an effective way to collect quality data that is, also,  feasible to implement in a live network. Additionally, although our findings are based on a simulator and a single setup, 
they may generalize to other data collection strategies.

Furthermore, we adapted the \ac{DT} architecture for \ac{LA}. We enhanced performance by modifying positional encoding and attention masks and by conditioning on channel quality indicators to handle irregular time intervals and to ensure causality. However, \ac{DT} struggles with the stochastic nature of \ac{LA} due to interference and varying channel conditions, which affect its ability to select optimal actions. In particular, we notice that while \ac{DT} is able to correctly condition the inference of optimal actions when dealing with sequences comprising few packet transmissions, when input sequences become longer the inherent variance of \ac{LA} makes it hard for \ac{DT} to model the stochasticity intrinsic to the process correctly.

Despite these challenges, our work provides valuable insights into applying machine learning in telecommunication networks and supports the use of offline \ac{RL} methods to train agents for live networks.

% Our simulations showed that offline \ac{RL} methods slightly improve upon the behavioral policy used for data collection, 
% starting from both optimal and suboptimal policies. 
 
% In this paper, we have addressed the problem of \ac{LA} by adopting alternative approaches to offline \ac{RL}. 

% Our thorough comparison run on a proprietary \ac{RAN} simulator has demonstrated the capabilities of the offline \ac{RL} methods we considered to obtain performances that slightly improve on the behavioral policy employed for collecting the training dataset, both in the case of optimal and suboptimal behavior. Despite employing datasets collected by a \ac{RL} trained online, we believe that similar findings may be valid regardless of the policy used for data collection. However, the use of the simulator poses some limitations to our work, and, also, the validity of our results is limited to one single simulation setup.

% One important contribution of this work is the sequence modeling framework we provide to solve \ac{LA} using a \ac{DT} architecture. The modifications we proposed contribute to the performance of the vanilla architecture when employed as a solution to the use case, in particular: the adjustments to the positional encoding definition are relevant as a way to represent the distribution of consecutive steps of an \ac{MDP} in which steps do not happen in discrete series of timesteps, the new definition of the attention mask guarantees causality at training time in a delayed-feedback setting and, finally, we found beneficial to correlate the target value used for conditioning the inference of optimal actions with an indication of the channel quality. Unfortunately, our results show \ac{DT} to be very liable to the stochasticity of the \ac{LA} process (due to stochastic interference and time- and frequency-varying channel conditions), preventing the model from correctly modeling the distribution of sequence realizations and, therefore, correctly conditioning the selection of optimal actions.

% Nonetheless, we believe this work to constitute a valuable contribution to the literature of \ac{ML} in telecommunication networks and a great starting point for those practitioners considering offline \ac{RL} methods to overcome the problems associated with training agents in live networks.




==> old_versions/backup_2024_11_18/0_abstract.tex <==

% Original abstract
\iffalse
\begin{comment}
% State the problem, your approach and solution, and the main contributions of the paper. Include little if any background and motivation. Be factual but comprehensive. The material in the abstract should not be repeated later word for word in the paper.
Recent work has shown the potential of applying reinforcement learning (RL) to radio resource management (RRM) in radio access networks (RAN) thanks to their ability to learn complex parameter relationships by interaction with an unknown environment.
However, real-world RAN deployments are challenging as the training phase may temporarily degrade the system’s performance up to, potentially, triggering link failure procedures.
To address such issues, we consider offline RL methods, which allow agents to be trained on previously collected datasets of transitions. 
Thereafter, we propose two alternative formulations for the Link Adaptation (LA) functionality in the context of the 3$^\text{rd}$~Generation Partnership Project (3GPP): the first one is motivated by the need to frame LA for the use of \mbox{value-based} offline RL methods, while the second one re-defines some aspects to adapt the problem to a sequence modeling framework and exploiting the capabilities of Decision Transformer (DT).
Our study, supported by an internal RAN system simulator platform compliant with the 3GPP 5G standard specifications, shows how offline RL methods can obtain better performance than rule-based baselines and achieve slightly better results than online RL algorithms. However, we find that excessive stochasticity prevents DT from effectively conditioning the inference of optimal actions.
\end{comment}
\fi

\iffalse
\begin{abstract}
Contemporary radio access networks -- such as the Long Term Evolution and New Radio systems specified by the $3^{rd}$ Generation Partnership Project -- employ link adaption (LA) algorithms to determine the modulation and coding schemes that take into account the prevailing propagation conditions and are near-optimal in terms of the achieved spectral efficiency 
%under block error rate targets. 
LA is a challenging task in the presence of mobility, fast fading and imperfect channel quality information and limited knowledge of the receiver characteristics at the transmitter, which render model-based LA algorithms complex and suboptimal. Model-based LA is especially difficult as connected user equipment devices become increasingly heterogeneous in terms of receiver capabilities, antenna configurations and hardware characteristics. 
Recognizing these difficulties, previous works have proposed reinforcement learning (RL) for LA, which face deployment 
difficulties due to their potential negative impacts on live performance. 
Therefore, in this paper we propose batch-constrained deep Q-learning and conservative Q-learning for LA, 
which facilitate offline RL that can be trained on data acquired from live networks without minimal or no intrusive
effects on the network operation. 
Our numerical results indicate that both schemes can provide superior performance compared with 
that of state-of-the-art online RL methods when a proper decision transformer is employed at the transmitter.
\gf{\it GF: Consistency check between the title and abstract: all words of te title should appear and be explained in the abstract.}
\end{abstract}
\fi

\begin{comment}
\begin{abstract}
To adapt to the prevailing propagation conditions, contemporary radio access networks employ link adaption (LA) algorithms that are near-optimal in terms of achieved spectral efficiency to optimize the modulation and coding schemes. 
%under block error rate targets. 
LA is a challenging task in the presence of mobility, fast fading, imperfect channel quality information and limited knowledge of the receiver characteristics at the transmitter, which render model-based LA algorithms complex and suboptimal. Model-based LA is especially difficult as connected user equipment devices become increasingly heterogeneous in terms of receiver capabilities, antenna configurations and hardware characteristics. 
Recognizing these difficulties, previous works have proposed reinforcement learning (RL) for LA, which, however, faces deployment difficulties due to potential negative impacts on live performance. 
%Therefore, in this paper we propose batch-constrained deep Q-learning and conservative Q-learning for LA,  which facilitate offline RL that can be trained on data acquired from live networks without minimal or no intrusive effects on the network operation. 
%Therefore, this paper propose three offline RL designs for LA using batch-constrained deep Q-learning, conservative Q-learning and decision transformers, to demonstrate that LA models can be trained on data acquired from live networks with minimal or no intrusive effects on the network operation. Our numerical results indicate that offline RL algorithms can achieve performance of state-of-the-art online RL methods when data is collected with a proper behavioral policy.
%
%Therefore, this paper investigates offline RL methods for LA that can be trained on data acquired from live networks with minimal or no intrusive effects on the network operation. We propose three LA designs based on batch-constrained deep Q-learning, conservative Q-learning, and decision transformers, showing that offline RL algorithms can achieve performance of state-of-the-art online RL methods when data is collected with a proper behavioral policy.
To address this challenge, this paper considers offline RL to learn LA policies from data acquired in live networks with minimal or no intrusive effects on the network operation. We propose three LA designs based on batch-constrained deep Q-learning, conservative Q-learning, and decision transformers, showing that offline RL algorithms can achieve performance of state-of-the-art online RL methods when data is collected with a proper behavioral policy.
\end{abstract}  
\end{comment}
% revision by PS 
\begin{abstract}

\Ac{LA} is an essential function in modern wireless communication systems that dynamically adjusts the transmission rate of a communication link to match time- and frequency-varying radio link conditions.
%
However, factors such as user mobility, fast fading, imperfect channel quality information, and aging of measurements make LA challenging to model, leading to reliance on suboptimal, rule-based algorithms. 
%
To bypass the need for explicit modeling, recent research has introduced online \ac{RL} approaches. Yet, these approaches face deployment challenges, as training in live networks can potentially degrade real-time performance.
%

To address this challenge, this paper considers offline RL to learn LA policies~\iffalse from data acquired in live networks\fi with minimal or no intrusive effects on the network operation. 
%
We propose three LA designs based on batch-constrained deep Q-learning, conservative Q-learning, and decision transformers, showing that offline RL algorithms can achieve performance of state-of-the-art online RL methods when data is collected with a proper behavioral policy.
\end{abstract}

==> old_versions/backup_2024_11_18/1_introduction.tex <==
\section{Introduction}\label{sec:introduction}
\begin{comment}
The increasing complexity of \ac{RRM} functionalities across successive generations of mobile broadband systems, coupled with the expanding variety of deployment scenarios \cite{calabrese_learning_2018}, has driven research efforts focused on leveraging the vast amount of data available within the network from measurements and system observations \cite{calabrese_learning_2018, generalization_2024}. 

\Ac{ML} methods and, in particular, \ac{RL} have recently gained attention as a solution to address the complex control problems involved in \ac{RRM} for \acp{RAN} where time- and frequency-varying channel conditions often make rule-based algorithms suboptimal. Due to their ability to learn directly from experienced behavior and to adapt to changing environment conditions, \ac{RL} methods are being considered to replace traditional rule-based \ac{RAN} functionalities with models learned from data \cite{gronland2024constrained,mollerstedt2024model}. However, training \ac{RL} agents in a live network requires algorithms to explore the state-action space in order to learn an optimal policy, at the cost of taking actions that may be suboptimal \cite{lattimore2020bandit,russo2024model}.

In this paper, we focus on the problem of \ac{LA}, a fundamental functionality of \ac{RRM} dynamically adjusting the transmission rate of a communication link based on the channel conditions reported by the \ac{UE}. We will consider the downlink communication between a base station and the \ac{UE}, but similar findings are reusable for the uplink case. In a data-rich environment such as the \ac{RAN} one, the recent advancements in ML and, at the same time, hardware, present an opportunity to tackle the problem of link adaptation with a strongly data-driven approach \cite{calabrese_learning_2018}. A data-driven approach directly acting on the link adaptation parameters could address the shortcomings associated with current solutions to \ac{LA} that frame it as a control problem and, as shown in multiple works such as \cite{geiser_drlla_2022}, improve performance.

With the goal of overcoming the challenges associated with the training phase of \ac{RL} agents mentioned above, we consider a family of \ac{RL} algorithms referred to as \textbf{offline \ac{RL}}. Offline \ac{RL} algorithms aim at learning policies from fixed datasets of transitions previously collected by a, possibly unknown, behavioral policy. This approach is attractive for critical applications, like \acp{RAN} operations, where online learning methods could be costly to implement or negatively affect system performance, especially during training. 

The main contributions of this work include: \textbf{(1)} a thorough evaluation and comparison of the performance of the various offline \ac{RL} algorithms designed for \ac{LA} using an event-driven system-level simulator compliant with the \ac{3GPP} \ac{5G} NG-RAN system; \textbf{(2)} a new sequence modeling framework necessary to solve \ac{LA} using the \ac{DT} architecture; \textbf{(3)} the design of an offline \ac{RL} algorithm based on \ac{DT}, including a new positional encoding definition; \textbf{(4)} the definition of a new objective function for the \ac{LA} problem allowing multiple, alternative ways of conditioning the inference with \ac{DT}.

The choice of considering \ac{DT} is driven by the capability to well-generalize over different tasks and data distributions which appears evident with transformer for, especially, \ac{NLP}. Similarly, we hope \ac{DT} to be able to adapt to different types of network traffic, facilitating the deployment of a same model over different network sites.

\begin{itemize}
    \item Highlight contributions, including how to construct the sequence in training and inference
    \item Add comment on choice of baseline for comparison (e.g., why we do not relate to prior published papers)
\end{itemize}

\end{comment}
%----


Modern radio access and wireless networks -- such as the \ac{5G} \ac{NR} systems -- employ model-based \ac{LA} algorithms to adapt the \ac{MCS} to time-- and frequency-varying channel conditions to maintain high spectral efficiency\iffalse while adhering to \ac{BLER} targets\fi ~\cite{duran_self-optimization_2015, blanquez-casado_eolla_2016, Blanquez-Casado:19, Ramireddy:22, Nicolini:23}. Both in \ac{TDD} and \ac{FDD} systems, \ac{LA} in the \ac{DL} relies on \ac{CSI} reports provided by the \ac{UE} that include the \ac{CQI}, a rank indicator, and a precoder matrix indicator~\cite{3rd_generation_partnership_project_3gpp_technical_2024}.

As \ac{CSI} reports may be inaccurate and rapidly age due to variations in channel and interference conditions, an \ac{OLLA} scheme is typically adopted to adjust \ac{SINR} estimates inferred from inaccurate or aged~\acp{CQI} to adhere to \ac{BLER} targets based on the \ac{HARQ} feedback~\cite{duran_self-optimization_2015}. Nonetheless, user mobility, fast fading, limited receiver-side information at the transmitter, as well as the heterogeneity of \acp{UE} population, e.g., in terms of receiver and hardware capabilities, render \ac{RRM} problems in \acp{RAN}, like \ac{LA}, complex control tasks to model~\cite{Chen:23, generalization_2024}.

Recognizing the challenges faced by model-based approaches, \ac{ML} methods, such as \ac{RL}, have recently gained attention to address the complex control problems in \acp{RAN} \cite{calabrese_learning_2018}, where time- and frequency-varying channel conditions often make rule-based algorithms suboptimal. The ability of \ac{RL} to learn directly from experienced behavior and to adapt to changes in the environment makes it appealing to replace traditional rule-based \ac{RAN} functionalities with models learned from data~\cite{generalization_2024}. Several works have applied this approach to \ac{LA}, starting with tabular~\cite{Bruno:14} and bandit~\cite{saxena_reinforcement_2021} approaches, adaptations of \ac{OLLA} based on Q-learning~\cite{Chen:23}, and \ac{DQN}-based designs intended to replace \ac{OLLA}~\cite{generalization_2024}.
%
However, training \ac{RL} agents in live networks requires algorithms to explore the state-action space to learn~an optimal policy, at the cost of taking suboptimal actions that may temporarily affect the network performance~\cite{generalization_2024, russo2024model}.

To address this adverse effect of \ac{RL}, recent works have proposed offline \ac{RL}, which aims at learning an optimal policy from a \emph{static dataset} of transitions produced by a behavioral policy, thus avoiding direct interactions with the environment while training~\cite{levine_offline_2020-1, janner2021offline, schweighofer2022dataset, Kumar:23, lyu2022mildly}. The inability to improve the training dataset during the training phase 
binds the quality and the behavior of the learned policy to the quality and state-action coverage of the available data. As such, distribution shift and out-of-distribution behavior, that is, a mismatch between the training and testing trajectory distributions, can render the learned policy ineffective.
%As the training dataset is not augmented during training, the quality and the behavior of the learned policy is constrained by the quality and state-action coverage of the available data. As such, distribution shift and out-of-distribution behavior, that is, a mismatch between the training and testing trajectories, can render the learned policy ineffective. %Thus employing offline \ac{RL} in complex real-time control problems, such as \ac{LA}, is non-trivial.
%\gf{\it GF: One paragraph about offline RL and the out-of-distribution and distribution shift problems and the concept 
%of transformers, as well as maybe other main concepts that must not come out of the blue later (maybe attention mechanisms ?).}
%
Thus, employing offline \ac{RL} to replace complex real-time \ac{RRM} control functions in \acp{RAN}, such as \ac{LA}, is non-trivial and presents two main challenges: firstly, the ability of an offline \ac{RL} design to achieve, when trained with proper data, optimal performance, e.g., comparable with an policy learned online; secondly, the design of a non-invasive behavioral policy to collect rich data in live networks without affecting performance.
\begin{comment}
    To capitalize the advantages of \ac{RL} over rule-based approaches while reducing the potentially negative impact of active exploration on the \acp{RAN} operation, this paper considers offline RL to design LA in 5G networks. We propose three LA designs  based on \ac{BCQ}~\cite{fujimoto_off-policy_2019}, \ac{CQL}~\cite{kumar_conservative_2020}, and \ac{DT}~\cite{chen_decision_2021}. While for \ac{BCQ} and \ac{CQL} we model the \ac{LA} problem as a partially observable \ac{MDP}, for \ac{DT} we consider a sequence modeling approach, where an \ac{LA} action for a packet transmission (or retransmission) is inferred based on a sequence of historical states, actions and rewards. Our results show that offline \ac{RL} algorithms can achieve performance of state-of-the-art online \ac{RL} when data is collected with a proper behavioral policy.
\end{comment}

This paper focuses on the first challenge considering offline \ac{RL} for \ac{LA} in \ac{5G} networks. We present three \ac{LA} designs based on \ac{BCQ}~\cite{fujimoto2019off}, \ac{CQL}~\cite{kumar_conservative_2020}, and \ac{DT}~\cite{chen_decision_2021}, with  a trained \ac{DQN} model \cite{mnih_playing_2013} acting as a behavioral policy for data collection. While for \ac{BCQ} and \ac{CQL} we model the \ac{LA} problem as a partially observable \ac{MDP}, \ac{DT} requires a sequence modeling approach, where a \ac{LA} action is inferred using a sequence of historical states, actions and rewards, allowing to optimize long-term rewards, e.g.,~average throughput or spectral efficiency. Our results show that offline \ac{RL} can achieve the performance of online \ac{RL} and outperform practical state-of-the-art \ac{LA} based on \ac{OLLA}  when data is collected with a proper behavioral policy.



%% REMOVED 4 ARXIV %%
{\color{black}The rest of the paper is organized as follows. Section~\ref{sec:background}~introduces preliminary concepts, Section~\ref{sec:problem formulation} formally describes the problem of \ac{LA} while Section~\ref{sec:problem} presents the \ac{BCQ} and \ac{CQL} design for \ac{LA}. Section~\ref{sec:method} frames \ac{LA} as a sequence modeling problem, presenting a \ac{DT}-based design. Section~\ref{sec:experiments} discusses numerical results, while Section~\ref{sec:conclusion} concludes the paper.}

\begin{comment}
to employ \ac{BCQ}  and \ac{CQL} 
for \ac{LA} in 5G networks, which are
value-based algorithms for offline \ac{RL} \cite{fujimoto_off-policy_2019}, \cite{kumar_conservative_2020}.  
In its discrete variant, \ac{BCQ} tackles the distributional shift issue by restricting the support 
of action selection to a subset of actions whose probability is at least $\tau>0$ times the probability 
of the action most likely selected by the behavioral policy, \gf{where $\tau$ is ... }  \cite{fujimoto_benchmarking_2019}. 
In contrast, \ac{CQL} modifies the training objective to minimize -- alongside the Bellman error \cite{Sutton:14} -- 
the estimates of the Q-values to learn lower-bounded estimates that are not overly optimistic \cite{kumar_conservative_2020}.
%which is a known issue in offline \ac{RL}  \cite{kumar_conservative_2020}.
\gf{\it GF: Need $\sim 2$ more sentences on (1) why using BCQ and CQL is challenging to employ specifically for LA and (2) how we address these challenges (at a very high level), "the punch line". 
This is just a teaser that motivates the reviewer/reader to read further.}    

\sam{SAM: mention reason for data collection with dqn maybe}

\gf{\it GF: 1. Check the consistency across the title, abstract, index terms and intro. 2. The intro should not exceed 1 page.}

\textbf{Possible ways to present contributions}
\begin{itemize}
    \item focus more broadly on offline RL
    \item offline RL modelling for link adaptation using CQL, BCQ and DT. More effort needed to design DT.
    \item evelautaion with industrial simulator
    \item be open about data collection policy
    \item show that we can replicate performance of DQN, and discuss remaining problems
    \item future work...
\end{itemize}

\end{comment}






==> old_versions/backup_2024_11_18/2_background.tex <==
\section{Preliminaries}\label{sec:background}
This section reviews some of the key concepts and introduces notation that will be useful in the sequel.

\subsection{Elements of \ac{RL}}

\ac{RL} frames the interaction between an agent and the environment as a \ac{MDP} \cite{Sutton:14,puterman2014markov}, defined by the tuple: $(\mathcal{S, A, P}, r)$. Here, $\mathcal{S}$ is the state-space, $\mathcal{A}$ is the action-space, $\mathcal{P}$ is the transition probability function (also known as transition dynamics), $r:\mathcal{S}\times\mathcal{A}\times\mathcal{S}\to\mathbb{R}$ is the reward function.
In an online setting, at each time-step $t$ the agent chooses an action $a_t$ according to some Markovian policy $\pi:{\cal S}\to {\cal A}$, which is function of the current state $s_t$ of the MDP, and observes the next state $s_{t+1}$, distributed according to $P(\cdot|s_t,a_t)$, and a reward $r_t$. 
For episodic MDPs, with a finite terminal state, the goal of the agent is to find a policy $\pi$ maximizing the expected collected reward $\mathbb{E}^\pi[G_t|s_0\sim \mu]$ for some initial state distribution $\mu$, where
$
    G_t = \sum_{k=0}^T r_{t+k},
$
and $T$ indicates the terminal step. In the context of \textit{continuing task}, where $T$ is not naturally defined, or may be infinite, the goal is to maximize the collected discounted reward, defined with a  discount factor $\gamma\in (0,1)$ as $
    \mathbb{E}^\pi[\sum_{k=0}^\infty \gamma^k r_{t+k+1}|s_0\sim \mu]
$.
\begin{comment}
In settings where $T$ is not naturally defined, we introduce the notion of \textit{continuing task} and re-define the return to include the discount factor $\gamma$: $
    G_t = \sum_{k+0}^\infty \gamma^k r_{t+k+1}.
$
\end{comment}

\subsection{Offline RL}
Differently from the online RL setting, in offline RL \cite{levine_offline_2020} the agent learns a policy from a previously collected dataset of experiences $\mathcal{D} = \{( s_t^i, a_t^i, r_{t}^i,s_{t+1}^i)_i\}$ (collected using a behavioral policy $\pi_\beta$).
As a consequence, the amount of data, and its quality, play a crucial role in offline RL, since the agent is not able to interact with the environment in an online fashion to collect new data. 
%While the goal of offline \ac{RL} remains the maximization of returns, in this framework agents no longer interact with the environment during training to collect new transitions using a behavioral policy $\pi_\beta$. 
%Instead, the learning algorithm shall derive a sufficient understanding of the \ac{MDP} dynamics exclusively from transitions available in a static \textit{training dataset} $\mathcal{D} = \{( s_t^i, a_t^i, s_{t+1}^i, r_{t+1}^i)_i\}$ collected by a behavioral policy $\pi_\beta$ prior to training. 
The inability to explore the state-action space during training may result in a distributional shift between the distribution under which the policy $\pi$ is trained and the one on which it will be evaluated \cite{levine_offline_2020}.

To address this issue, some approaches constraint how much the learned policy $\pi$ differs from the behavioral policy~$\pi_\beta$, while other methods penalize the learned $Q$-values. For example, with discrete action spaces, \ac{BCQ} tackles the distributional shift issue by restricting the support  of action selection to a subset of actions whose probability exceeds the probability  of the action most likely selected by the behavioral policy by a minimum threshold~\cite{fujimoto_benchmarking_2019}.
%
In contrast, \ac{CQL} \cite{kumar_conservative_2020} uses a \emph{pessimism} principle: it modifies the training objective to minimize, alongside the Bellman error \cite{Sutton:14}, the estimates of the Q-values to learn lower-bounded estimates that are~not overly optimistic. A comprehensive survey can be found~in~\cite{levine_offline_2020}.


 


\begin{comment}
    While the goal is still the maximization of returns, in the offline \ac{RL} framework agents no longer have the ability to interact with the environment and collect additional transitions using the behavioral policy. This limits the possibility of exploring the state-action space to the transitions included in a static \textit{training dataset} $\mathcal{D} = \{( s_t^i, a_t^i, s_{t+1}^i, r_{t+1}^i)_i\}$, forcing the learning algorithm to derive a sufficient understanding of the \ac{MDP} dynamics exclusively from the available transitions. The challenge addressed by offline \ac{RL} is the distributional shift between the distribution under which the function approximator (policy, value function, or model) is trained and the one on which it will be evaluated. The simplest solution consists in bounding the distributional shift by constraining how much the learned policy $\pi$ differs from the behavioral policy $\pi_\beta$, with different algorithms employing slightly different approaches. A comprehensive review can be found in~\cite{levine_offline_2020}.
\end{comment}

%\\

% \textcolor{blue}{This work is going to consider \ac{BCQ} \cite{fujimoto_off-policy_2019} and \ac{CQL} \cite{kumar_conservative_2020}, two of the main value-based algorithms for offline \ac{RL}. In its discrete variant, \ac{BCQ} \cite{fujimoto_benchmarking_2019} tackles the distributional shift issue by restricting the support of action selection to a subset of actions whose probability is at least $\tau$ times the probability of the action most likely to be selected by the behavioral policy. On the other hand, \ac{CQL} \cite{kumar_conservative_2020} modifies the training objective to minimize, alongside the Bellman error, the estimates of the Q-values to learn lower-bounded estimates that are not overly optimistic, which is a known issue in offline \ac{RL} }


%     \begin{figure*}
%     \centering
%     \begin{minipage}{.49\textwidth}
%     \includegraphics[width=\textwidth]{Figures/olla_v1.2.png}
%     \caption{Visual description of the functioning of Link Adaptation.}
%     \label{fig:olla schema}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{.49\textwidth}
%     \includegraphics[width=\textwidth]{Figures/sequence_1.png}
%     \caption{Episodes in our MDP formulation for LA. Each box represents a TTI, and acknowledgements use the same color as the transmission they respond to. Between TTI 5 and 7 two packets are active, with episodes 1 and 2 overlapping. \textcolor{red}{TODO: make picture more narrow}}
%     \label{fig:sequence_1}
%     \end{minipage}
% \end{figure*}

\subsection{Sequence Modeling and Decision Transformer} 
Sequence modeling involves training auto-regressive models (such as the \ac{DT} \cite{chen_decision_2021}) on sequential data to capture patterns and make future predictions. Since the goal in \ac{RL}~is~to produce a sequence of actions leading to high cumulative rewards, one can re-frame the RL problem in terms of sequence modeling.

The \ac{DT} is a particular auto-regressive architecture used in sequence modeling that exploits the capabilities of GPT2~\cite{radford_language_2019} to perform sequential decision making. For each time step $t$ of a trajectory, \ac{DT}  uses sequences of $3$ embedded tokens: the state $s_t$, the action $a_t$, and the \ac{RTG} $\hat R_t = \sum_{t'=t}^T r_{t'}$. 
At inference time the \ac{RTG} allows to condition the output of the network to generate optimal actions by specifying \textit{future target} returns.
% Note that it is of particular importance  the \ac{RTG}: at inference time it allows to condition the output of the network by specifying \textit{future target} returns.
The model is trained by predicting the action $a_t$ at each time-step of the sequence. Overall, this architecture allows to bypass the need for bootstrapping to propagate returns, one of the key destabilizing elements in offline \ac{RL}.






==> old_versions/backup_2024_11_18/3_problem.tex <==
\section{Problem Formulation}\label{sec:problem formulation}
We consider the problem of \ac{LA} in the downlink of multi-cellular \acp{RAN}. The aim of LA is to dynamically adapt the transmission rate of individual packet transmissions to time- and frequency-varying channel conditions and radio interference. In \ac{5G} systems, this is achieved by selecting a set of \ac{MCS} parameters encoded by an integer taking value in the range~$\{0,31\}$,  known as the \ac{MCS} index~\cite{3rd_generation_partnership_project_3gpp_technical_2024}. Each \ac{MCS} index corresponds to a modulation order, code rate, and spectral efficiency to be used for transmitting a data packet to the \ac{UE}.

State-of-the-art \ac{LA} algorithms used in real-time \acp{RAN} combine two control loops executed on a sub-millisecond~timescale: an \ac{ILLA} converts the latest \ac{CQI} reported by the \ac{UE} into an initial \ac{SINR} estimate; an \ac{OLLA} scheme adjusts such an estimate (e.g., to compensate inaccuracies or aging of the \ac{CQI}) based on the \ac{HARQ} feedback (i.e., either positive or negative acknowledgments) received from the \ac{UE} for previous packet transmissions. The goal of the \ac{OLLA} is to maximize the link spectral efficiency while adhering to a desired \ac{BLER} target. As variants of this approach are widely adopted in today's communication systems, we consider it as reference for performance comparison in Section~\ref{sec:experiments}. 



%In this section, we first present \ac{LA} as framed for solving it as a control problem and then provide a formulation as a \ac{MDP}: we are going to consider this alternative formulation for training and evaluation of value-based offline \ac{RL} methods as well as data collection.


    
%\subsection{Pure Control Formulation}\label{olla}
%Traditional \ac{LA} algorithms rely on the combination of an inner- and \ac{OLLA} to reconstruct an estimate of the \ac{UE} \ac{SINR}: the \ac{ILLA} converts a \ac{CQI} to an initial estimate according to some pre-defined, link level curves while \ac{OLLA} adjusts such an estimate to take into account uncertainties in the \ac{CQI} transmission by means of a feedback loop acting on the received \ac{HARQ} signals (i.e., either positive or negative acknowledgments). \Ac{OLLA} algorithms circumvent the inherent complexity in modeling link adaptation by fixing a target \ac{BLER} value, defined as the experienced frequency of packet retransmissions. %\textcolor{red}{However, while several transmissions are required for OLLA to converge to the \ac{SINR} adjustments meeting the desired \ac{BLER}, traffic for most \acp{UE} consists of short bursts of transmissions. Furthermore, most implementations require to specify a fixed \ac{BLER}, which is not optimal for all channel conditions. Figure \ref{fig:olla schema} provides a visual description of the \ac{LA} process, highlighting the different stages of the above-described solution. THIS MAY BE REMOVED AND STAY ONLY IN THE INTRO?}


==> old_versions/backup_2024_11_18/4_LA_as_offline_RL.tex <==
\section{Link Adaptation as an Offline RL Problem}\label{sec:problem}
This section explores how \ac{LA} can be solved with offline \ac{RL}. \sam{We propose a \ac{MDP} formulation enabling agents to learn from experiences generated by any \ac{UE} within the network, collected in static datasets in the form of $(s_t,a_t,r_{t+1},s_{t+1})$ tuples. Being particularly well-suited both for online and offline \ac{RL} approaches, we consider such a formulation not only for training \ac{BCQ} and \ac{CQL} agents but also for collecting data using a behavioral \ac{DQN} policy, trained online.}


% We begin by presenting our \ac{MDP} formulation of LA and then discuss how offline \ac{RL} methods, like \ac{BCQ} and \ac{CQL}, can be applied to solve this \ac{MDP} formulation.

%     \begin{figure}
%     \centering

%     \includegraphics[width=0.5\textwidth]{tikz_imgs}
%     \caption{Episodes in our MDP formulation for LA. Each box represents a TTI, and acknowledgements use the same color as the transmission they respond to. Between TTI 5 and 7 two packets are active, with episodes 1 and 2 overlapping. \textcolor{red}{TODO: make picture more narrow}}
%     \label{fig:sequence_1}
% \end{figure}

\begin{figure}
    \centering
    % Resize the combined TikZ images to fit within the column width
    \resizebox{\linewidth}{!}{%
    \input{tikz_imgs/img_harq_example}
    }
    \caption{Episodes in our \ac{MDP} formulation for LA. Each box represents a \ac{TTI}, and acknowledgments use the same color as the transmission they respond to. Note that episodes 1 and 2 overlap between \ac{TTI} 5 and 12.}
    \label{fig:sequence_1}
\end{figure}
\subsection{\ac{MDP} Formulation}  

We model \ac{LA} as an episodic \ac{MDP} in which an episode (or trajectory) $\tau=(s_0,a_0,r_0,\dots, s_T,a_T,r_T)$  corresponds to the lifespan of a \ac{UE}'s data packet from its first transmission to, alternatively, a successful reception or the packet being dropped after four retransmissions (as illustrated in~\cref{fig:sequence_1}). As such, the episode's length $T$ is bounded to five steps (each corresponding to a transmission of the packet).
\begin{itemize}
    \item The state $s_t \in \mathbb{R}^n$ is a  vector of semi-static and dynamic information characterizing the serving cell, the \ac{UE} design, as well as radio measurements, channel state information, \ac{HARQ} feedback, and more\footnote{The exact list of states cannot be disclosed as it is based on Ericsson's internal research work.}.
    \item The action $a_t\in \{0,\dots,27\}$ takes an integer, representing one of 28 \ac{MCS} indices for data transmissions, as defined by the \ac{5G} specifications~\cite{3rd_generation_partnership_project_3gpp_technical_2024}. When dealing with a re-transmission, that is $t\geq 1$,  the simulator maps the agent's action to a reserved \ac{MCS} index in the interval $\{28,\dots,31\}$, as per \ac{5G} specifications.
    \item  The reward signal $r_t=r(s_t,a_t)$ is function of the \ac{SE} of the packet transmission. 
\end{itemize}

Additionally, as the \ac{UE}'s \ac{HARQ} process supports multiple active packets at any given time, multiple \ac{UE}'s episodes may overlap in time (as in the example in~\cref{fig:sequence_1}). 

% \subsection{Solving LA with Offline \ac{RL}}
% The proposed \ac{MDP} modeling enables an \ac{RL} agent to learn from experiences generated by any \ac{UE} within the network. Hence, it is particularly well-suited both for online and offline \ac{RL} approaches thanks to the large amounts of data collected in the network. 

% We consider this formulation to train a \ac{DQN} policy  to serve as behavioral policy for data collection as well as performance reference for offline \ac{RL}. As training data samples for offline \ac{RL} consist of state-action-reward tuples $(s_t,a_t,r_t)$, we can consider the evaluation and training of value-based and actor-critic methods~\cite{Sutton:14}.  

% We propose two offline \ac{RL} algorithms for \ac{LA} based on \ac{BCQ}~\cite{fujimoto2019off}, and \ac{CQL}~\cite{kumar_conservative_2020}, respectively. 

% {\color{red}[@Alessio, @Samuele]: could we add a couple of sentences to indicate in what way you designed these algorithms for LA? It does not need to long}

%Training data samples for offline \ac{RL} are represented by state-action-reward tuples $(s_t,a_t,r_t)$, which allows for the evaluation and training of value-based and actor-critic methods \cite{Sutton:14}. Consequently, this formulation is particularly well-suited for use with offline \ac{RL}, as it can exploit the large amounts of data collected in the network to train a policy using a fixed dataset \cite{levine_offline_2020}.

%{\color{blue} [PS]: I would add here a description of the LA design based on BCQ and CQL and move the sequence modeling paragraph to the beginning of Sec IV}
\begin{comment}
  \paragraph{Sequence modeling}
However, there are some shortcomings with this modeling of LA. Firstly, such formulation optimizes only over one packet at the time, without considering sequences of multiple packets. Secondly, since packet arrivals are unknown and channel conditions are time-varying, the overall stochastic process we aim to control can be more generally framed as a \emph{contextual} \ac{MDP} \cite{hallak2015contextual}. A contextual \ac{MDP} is a specific type of \ac{MDP} that includes an underlying time-varying hidden parameter (context) affecting the transition dynamics—such as packet arrivals and channel conditions. Managing such a process is generally more complex than controlling a classical \ac{MDP} \cite{kaelbling1998planning}. To address these complexities, we propose a sequence modeling approach \cite{janner2021offline,emmons_rvs_2021}, a method to efficiently handle sequences of data.  
\end{comment}
    



==> old_versions/backup_2024_11_18/5_sequence_modelling_for_LA.tex <==
\section{Sequence Modeling for Link Adaptation}\label{sec:method}

The previous \ac{MDP} formulation of \ac{LA}, and thereby the related offline \ac{RL} designs,  present some shortcomings. Firstly, such formulation optimizes the return for individual packets. Thus, it may not capitalize that sequences of packets can experience correlated channel conditions that would allow to optimize longer-term metrics (e.g., \ac{UE} throughput). Secondly, since packet arrivals are unknown and channel conditions are time-varying, the overall stochastic process we aim to control can be more generally framed as a \emph{contextual} \ac{MDP} \cite{hallak2015contextual}. A contextual \ac{MDP} is a specific type of \ac{MDP} that includes an underlying time-varying hidden parameter (context) affecting the transition dynamics—such as packet arrivals and channel conditions. Managing such a process is generally more complex than controlling a classical \ac{MDP} \cite{kaelbling1998planning}. 

To address these complexities, \ps{we reformulate offline \ac{RL} for \ac{LA} as a sequence modeling problem \cite{janner2021offline,emmons_rvs_2021}\iffalse, a method to efficiently handle sequences of data\fi~and propose a solution that extends and adaptations the \ac{DT} design \cite{chen_decision_2021}.}
%We then outline our contributions in adapting the original \ac{DT} design \cite{chen_decision_2021} to the \ac{LA} problem.

\subsection{RL via Supervised Learning (RvS)}
%Sequence modeling involves training auto-regressive models on sequential data to capture patterns and make future predictions. Since the main goal in \ac{RL} is to produce a sequence of actions leading to high cumulative rewards, we can re-frame the RL problem in terms of sequence modeling.

By framing RL as a sequence modeling problem, we can better capture the time-varying interactions in the underlying process. This approach {\color{red} simplifies various design decisions} and leverages the strengths of sequence models in handling temporal dependencies.

We consider the \ac{RvS} learning approach for offline RL proposed in \cite{emmons_rvs_2021}. This approach takes as input a dataset ${\cal D}=\{\tau\}$ of trajectories of experience and outputs an \emph{outcome-conditioned} policy $\pi_\theta(a_t\mid s_t,\omega)$ that optimizes
\begin{equation}
    \max_\theta \mathbb{E}_{\tau \sim {\cal D}}\left[\sum_{t=0}^{|\tau|-1} \mathbb{E}_{\omega \sim f(\omega\mid \tau_t)}\left[ \ln \pi_\theta(a_t\mid s_t,\omega)\right]\right],
\end{equation}
where $\tau_t=\{s_t,a_t,r_t,s_{t+1},\dots\}$ denotes the trajectory starting at time $t$, $|\tau|$ denotes the trajectory length, and $f(\omega|\tau)$  denotes the distribution over outcomes $\omega$ that occur in a trajectory. These outcomes are user-chosen, and can be, for example:
\begin{itemize}
    \item \emph{Goal-oriented}: $\omega=\{s_{h}=s\}$, that is, $f(\omega|\tau)$ indicates the likelihood of visiting state $s$ at step $h$.
    \item \emph{Reward-oriented}: $\omega=\sum_{n\geq t}\gamma^{n-t} r_n$, and $f(\omega|\tau)$ indicates the likelihood of achieving a certain total discounted  reward starting from $t$. Such conditioning is also referred to as \emph{return-to-go} (RTG).
\end{itemize}
At inference-time, then, the user can choose to condition the policy according to the desired objective.

\subsection{RvS Learning for LA}
To formulate  \ac{LA}  in terms of the \ac{RvS} learning framework, we introduce a trajectory definition that extends beyond the lifespan of a single packet, departing from the previous \ac{MDP} formulation.  After that, we introduce different ways to condition the policy $\pi_\theta$.
 %After that, we introduce our proposed reward-oriented conditioning, as well as  a particular type of ci
%This extension allows us to leverage a \ac{DT} approach for \ac{LA}, benefiting from the transformer's ability to perform long-term credit assignment by considering long sequences spanning multiple packet transmissions.


\subsubsection{Trajectory definition} \label{trajectory definition} We consider fixed-horizon trajectories $\tau=\{s_0,a_0,r_0,\dots, s_H,a_H,r_H\}$, which include  transmissions of packets belonging to a specific \ac{UE}.

%. Letting $3K$ denote the transformer's context size, each sequence can include tokens corresponding to up to $K$ transmissions, with extra positions filled using padding tokens.
We consider two alternative approaches to construct $\tau$:

\begin{enumerate}[label=\alph*)]
    \item \emph{Recent transmissions}:  $\tau$ consists of the most recent $K$ transmissions of the \ac{UE} considered (hence $H=K$).
    \item \emph{Consecutive packets}: $\tau$ includes only up to  $n_p$ of a \ac{UE}'s most recent consecutive packets. Since a packet can be retransmitted at most four times upon its initial transmission, we have that $H\in\{n_p,\dots, 5n_p\}$.
\end{enumerate}
At training time, {\color{red} we sample trajectories of data from the dataset ${\cal D}$ using one of these two approaches}, and, if needed, extra positions in  $\tau$ are filled using padding tokens.

% To formulate the \ac{LA} functionality as a sequence modeling problem, we introduce a trajectory definition that departs from the previous \ac{MDP} formulation and extends the episode horizon beyond the lifespan of a packet. This allows us to leverage a \ac{DT} approach for \ac{LA} and benefit from the transformer's ability in performing long-term credit assignment by considering long sequences of tokens that span across transmissions for multiple packets. Specifically, we define a trajectory to include all the transmissions of packets belonging to a certain \ac{UE} in a simulation. Letting $3K$ denote the context size of the transformer, tokens relative to up to $K$ transmissions can be included in each sequence, with extra positions being filled with padding tokens. We consider two alternative approaches: (1) a sequence consisting of the most recent $K$ transmissions relative to a certain \ac{UE}; (2) a sequence including transmissions relative to $n_p$ of a \ac{UE}'s most recent consecutive packets. Considering~$5$ as the maximum number of retransmission, each sequence will include a number of transmissions in $[n_p, 5n_p]$. 



% \subsection{DT design modifications}
% \label{DT modifications}
% \ac{LA} has some fundamental differences when compared to standard \ac{RL} baselines such as those considered in the original \ac{DT} paper \cite{chen_decision_2021}. In this section, we present the main modifications to its design that we found necessary for our use case.


\subsubsection{Outcome conditioning}\label{subsec:conditioning} We propose the following three ways to condition the policy $\pi_\theta$ for \ac{LA}:
\begin{enumerate}[label=\alph*)]
    \item {\bf VANILLA}: This is a simple conditioning that consists in fixing a target \ac{RTG} value $\omega$ for each packet $p$. At training time, the \ac{RTG} at the $k$-th step of a packet is computed as  $\omega=\sum_{t=k}^{T(p)} \gamma^{t-k} r_k(p)$, where $r_k(p)$ indicates the reward associated to the $k$-th transmission for packet $p$, $\gamma \in(0,1]$, and  $T(p)$ is a random variable indicating the termination step for the transmission of packet $p$. At inference time, the \ac{RTG} is fixed to a pre-defined value at the first transmission and adjusted in case of retransmissions (we expand on this in~\cref{sec:experiments}).

    \item {\bf DAVG}: The VANILLA approach has the same shortcomings of the MDP formulation proposed in \cref{sec:problem}. An alternative is to condition according to a \ac{DAVG} of  future rewards. Letting $n$ denote the $n$-th step in a sequence of continuous transmissions from a UE, at training time we condition according to:
    \[
           \omega=(1-\gamma)\sum_{t=n}^\infty \gamma^{t-n}r_t,
    \]
    with $\gamma \in(0,1)$.   At inference time, as for the VANILLA case, we condition according to some pre-defined value.
    \item {\bf 3GPP}: Lastly, we propose a novel conditioning method based on the observation that the reward signal, as mentioned in \cref{sec:problem}, is directly related to the spectral efficiency of the channel. Therefore, we condition the policy $\pi_\theta$ according to a nominal spectral efficiency value given the channel quality. Specifically, at each first packet transmission, depending on the \ac{CQI} value reported by the \ac{UE} in the state $s$, we use the corresponding nominal spectral efficiency from the \ac{CQI} Table 5.2.2.1\text{-}3 of the \ac{3GPP} specification~\cite{3rd_generation_partnership_project_3gpp_technical_2024} as the target \ac{RTG} value.
\end{enumerate}






% When shifting to a trajectory definition including all of a \ac{UE}'s transmissions it becomes unfeasible to compute \acp{RTG} on an infinite horizon. Furthermore, in radio communications, packets’ transmissions that are distant in time are roughly independent and the knowledge about future rewards is unlikely to be useful for generating optimal actions for earlier packets. Taking inspiration from the framework described by Emmons et al. in \cite{emmons_rvs_2021}, we propose the following expression as a new objective definition for \ac{LA}:

% \begin{itemize}
%     \item VANILLA: 
%         \begin{equation}
%             V(p)=\mathbb{E}\left[\sum_{k=0}^{T(p)} r_k(p)\right].
%         \end{equation}
%     \item AVG
%         \begin{equation}
%             RTG(i_0)=\mathbb E_{\tau \sim \mathcal{D}} \left[\sum_{i=i_0}^{|\tau|-1} \gamma_0^{i-i_0}r_i\right], 
%         \end{equation}
% \end{itemize}

% \begin{equation}
% \label{equation:final objective definition}
%     \mathbb E_{\Upsilon \sim \rho} \left[\sum_{n=n_0}^\infty \gamma_0^{t_n-t_{n_0}}V(p_n)\right], 
% \end{equation}
% where with $V(p)$ we refer to the value of a packet, defined as:
% \begin{equation}
%     V(p)=\mathbb{E}\left[\sum_{k=0}^{T(p)}\gamma_1^k r_k(p)\right].
% \end{equation}

% In such a formulation, $\Upsilon$ denotes a sequence of packets transmitted at random times, where $\rho$ is the distribution over packets and time. $\gamma_0$ and $\gamma_1$ are discount factors respectively affecting the sum of the values of successive packets and successive retransmissions for a single packet. $t_n$ is the time of transmission of packet $n$, with $t_{n_0}$ being the time of transmission of the first packet of the sequence. $T(p)$ is a random variable indicating the termination step for the transmission of packet $p$. Finally, $r_k(p)$ indicates the reward associated to the $k$-th transmission for packet $p$.

% The formulation is general enough that by setting $\gamma_0=0$ the objective converges to a packet basis, similar to the objective for the formulation described in \ref{MDP formulation}; by choosing $0 < \gamma_0 < 1$ the objective instead becomes a discounted sum of future rewards. We can imagine the first case as conditioning \ac{DT} on intermediate goals for each packet. 

% \textcolor{blue}{In the following sections we present results obtained by setting $\gamma_0 = 0$ or, alternatively, by simply computing average returns on a window with fixed size of $M$ transitions, discounting rewards at each transmission.}


% \subsubsection{Conditioning at inference}
% At inference time, we propose three different ways of conditioning the generation of actions. (1) \textbf{VANILLA} consists in fixing a target \ac{RTG} value $\omega$ for each packet, $\omega$ is fixed at the first transmission and adjusted in case of retransmissions; (2) \textbf{3GPP}, similarly to VANILLA, at each first packet transmission selects a target \ac{RTG} value according to the \ac{3GPP} \ac{CQI} Table 5.2.2.1-3 in \cite{3rd_generation_partnership_project_3gpp_technical_2024}, depending on the \ac{CQI} value reported by the \ac{UE} inside the state; (3) \textbf{AVG} conditions each step with the same value of average \ac{RTG} as a target. 

\subsection{Decision Transformers Design for LA}

Hereafer, we describe how we adapted the \ac{DT} architecture for the link adaptation problem. We introduce two changes: one to the attention layer, and one for the positional embedding.
\begin{figure}[t]
    \centering
    % Resize the combined TikZ images to fit within the column width
    \resizebox{\linewidth}{!}{%
    \input{tikz_imgs/img_attention_mask}
    }
    \caption{\textbf{At training time}, the modified definition of the attention mask (right matrix) prevents the tokens associated to $p_2$ and $p_4$ from attending $p_1$, as its reward is not available at the time an MCS index is requested for $p_2$ and $p_4$. The left matrix shows the original attention mask definition.}
    \label{fig: attn mask}
\end{figure}


% \begin{figure}
%     \centering
%     % Resize the combined TikZ images to fit within the column width
%     \resizebox{\linewidth}{!}{%
%     \input{tikz_imgs/img_sequence_builing}
%     }
%     \caption{Given a trajectory $\tau$ (relative to a single \ac{UE}), input sequence (a) is built by setting $K=4$ while sequence (b) is built with $n_p=2$. The first index in the notation $t_{i,j}$ identifies the transmission count while the second is a unique packet id. A same color also identifies transmissions for a same packet.}
%     \label{fig: sequence building}
% \end{figure}

\subsubsection{Attention masking for delayed feedback}

\begin{comment}
A significant challenge in training a \ac{DT} architecture for \ac{LA} is preventing the leakage of future data during the training process. To perform inference, historical rewards are only available upon a base station receiving a \ac{HARQ} feedback (either positive or negative) for previous packet transmissions. Hence, it is essential to ensure that \ac{DT}'s outputs during training rely solely on information available in real-time, avoiding any use of future data that would not be accessible in an actual deployment.
\end{comment}
A significant challenge in training a \ac{DT} architecture for \ac{LA} is preventing the leakage of future data during the training process. \ps{During training, it is essential to ensure that \ac{DT}'s inference outputs rely solely on information available as in real-time}, avoiding any use of future data that would not be accessible in an actual deployment. As historical rewards are only available upon a base station receiving a \ac{HARQ} feedback (either positive or negative) for previous packet transmissions, \ps{we propose an attention masking to cope with such delayed feedback}.

\begin{comment}
To describe the proposed modification we need to introduce some notation. First, for a trajectory: \[\tau=(\underbrace{s_0}_{X_{0}},\underbrace{a_0}_{X_1},\underbrace{r_0}_{X_2},\dots, \underbrace{s_K}_{X_{3K}}, \underbrace{a_K}_{X_{3K+1}}, \underbrace{r_K}_{X_{3K+2}}),\]
let $(X_0, X_1,\dots, X_{3K+2})$ be the corresponding sequence of tokens fed as input to the \ac{DT}. Secondly, define $t_a(p)$ and $t_r(p)$ to be the instants in time at which, respectively,  the action for packet $p$ is scheduled and the associated reward signal is available. Lastly, indicate by $p(X)$ the mapping $X\mapsto p$ between a token to the corresponding packet. Then, the attention mask between any two tokens $X_i,X_j $ is given by:
\[
\hbox{\texttt{attn\_mask}}(X_i,X_j) = \mathbf{1}\{ t_r(p(X_i)) \leq t_a(p(X_j))\}.
\]
 In other words, if we have not yet received any reward for packet $p(X_i)$, then the tokens of the packet $p(X_j)$ should not be affected by the tokens of packet $p(X_i)$. \cref{fig: attn mask} describes such a formulation visually.
\end{comment}

\ps{To this end, we model a trajectory~$\tau$~as} \[\tau=(\underbrace{s_0}_{X_{0}},\underbrace{a_0}_{X_1},\underbrace{r_0}_{X_2},\dots, \underbrace{s_K}_{X_{3K}}, \underbrace{a_K}_{X_{3K+1}}, \underbrace{r_K}_{X_{3K+2}}),\]
\ps{where $(X_0, X_1,\dots, X_{3K+2})$ indicates the associated sequence of input tokens, and we define $t_a(p)$ and $t_r(p)$ as the time at which, respectively,  the action for packet $p$ is scheduled and the associated reward signal is available. The proposed attention mask between any two tokens $X_i,X_j $ is}
\[
\hbox{\texttt{attn\_mask}}(X_i,X_j) = \mathbf{1}\{ t_r(p(X_i)) \leq t_a(p(X_j))\},
\]
\ps{where $p(X)$ is a mapping between a token $X$ and the associated packet $p$.
As illustrated in \cref{fig: attn mask}, the mask assures that if a reward for a packet $p(X_i)$ is not received when an action for a packet $p(X_j)$ is taken, then tokens of packet $p(X_j)$ should not be affected by the tokens of packet $p(X_i)$.}

\input{plots}
% Formally, by referring to the instant in time at which the action for packet $i$ is scheduled with $t_{a,i}$ and the instant in time the associated reward signal is received with $t_{r,i}$, we apply:
% \begin{align}
%         \begin{array}{rcl}
%             \text{given a sequence of tokens }\left[T_0, T_1, ..., T_{3 \cdot \text{seq\_len}-1} \right], \\
%             \forall T_i,T_j, \text{ if } t_{r,i} > t_{a,j} \text{ then } attn(i,j) = -\infty,
%         \end{array}
%     \end{align}
% where $attn(i,j)$ represents the un-normalized attention score between token~$i$~and~$j$. 

\iffalse
\ps{To this end, we model a trajectory~$\tau$~as} \[\tau=(\underbrace{s_0}_{X_{0}},\underbrace{a_0}_{X_1},\underbrace{r_0}_{X_2},\dots, \underbrace{s_K}_{X_{3K}}, \underbrace{a_K}_{X_{3K+1}}, \underbrace{r_K}_{X_{3K+2}}),\]
where $(X_0, X_1,\dots, X_{3K+2})$ \ps{indicates the} sequence of input tokens, and we define $t_a(p)$ and $t_r(p)$ as the time at which, respectively,  the action for packet $p$ is scheduled and the associated reward signal is available. Lastly, \ps{we let $p(X)$ denote a mapping between a token $X$ to the corresponding packet $p$.} The proposed attention mask for delayed feedback between any two tokens $X_i,X_j $ can then be expressed as
\[
\hbox{\texttt{attn\_mask}}(X_i,X_j) = \mathbf{1}\{ t_r(p(X_i)) \leq t_a(p(X_j))\}.
\]
In other words, if we have not yet received any reward for packet $p(X_i)$, then the tokens of the packet $p(X_j)$ should not be affected by the tokens of packet $p(X_i)$. \cref{fig: attn mask} describes such a formulation visually.
\fi

\subsubsection{Temporal embeddings}
% \ac{LA} is a real-time process where states (sim. actions) are observed at points in time that are not equidistant between each other. The DT architecture was designed for processes with an equidistant sampling. We propose to capture the correlation in time between successive packet transmissions by modifying the \ac{DT} positional encoding. 
\ac{LA} is a real-time process with \ps{states, actions, and rewards} observed at irregular intervals, whereas the \ac{DT} architecture assumes equidistant sampling. \ps{To handle irregular observations, we propose three positional encodings that capture temporal correlations between successive packet transmissions of a \ac{UE}:}
%
%To capture the temporal correlations between successive packet transmissions of a \ac{UE}, we consider the following modifications of the \ac{DT}'s positional encoding:
\begin{enumerate}
    \item \textbf{\Ac{BE}}: as a baseline, we implement a minor modification to the original encoder from \cite{chen_decision_2021}, where embeddings are learned based on each token's index within the sequence ($i \in [0, K-1]$).
    \item \textbf{\Ac{LT} encoding}: 
    embeddings are learned using a linear layer with $(\Delta {t}_i)_{i=0}^K$ as input, where $\Delta t_i= t_a(p(X_i)) - t_a(p(X_0))$. Hence, $\Delta {t}_i$ is a measure of the relative time  between the $i$-th token and the first one.
    Note that tokens within the same packet have identical relative timestamps, allowing the \ac{DT} to associate the reward to the corresponding state and action.

    \item \textbf{\Ac{CT} encoding}: inspired by \cite{zuo2020transformer, zhang2023continuous},  the $k$-th element of the positional embedding vector for token $X_i$ is computed as:
\begin{equation}
    PE(\Delta t_i, k) = \begin{cases}
    \sin\left(\displaystyle \frac{\Delta t_i / 100}{{C}^{\frac k {d_\text{model}}}}\right) & \text{ for even } k, \\[4ex]
    \cos\left(\displaystyle \frac {\Delta t_i / 100} {C^{\frac {k-1} {d_\text{model}}}}\right) & \text{ for odd } k,
    \end{cases}
    \end{equation}
    where $d_{\text{model}}$ is a user-chosen constant (see also  \cite{zhang2023continuous}).
\end{enumerate}


==> old_versions/backup_2024_11_18/6_experiments.tex <==
\section{Numerical Results}\label{sec:experiments}

In this section, we empirically compare the considered offline \ac{RL} methods using an industry-grade simulator. We evaluate their performance in terms of throughput, experienced \ac{BLER}, and \ac{UE} \ac{SE} across all \ac{MIMO} layers allocated for transmission. Specifically, we investigate: (1) whether offline \ac{RL} methods can match the performance of the behavioral policy and of OLLA; (2) how the behavioral policy affects performance of these methods; and (3) whether our modifications to the \ac{DT} design improve \ac{LA} performance.

% This section compares empirically the results of the considered offline \ac{RL} methods with an industry-grade simulator. We  assess their performance in terms of throughput, experienced \ac{BLER} and \ac{UE} \ac{SE}, computed across all \ac{MIMO} layers allocated for the transmission.
% Specifically, we want to address the following points: (1)~whether offline \ac{RL} methods can match the performance of the behavioral policy and the considered baselines; (2)~how much the performance is affected by the behavioral policy; (3)~whether the modifications to the \ac{DT} design are useful for improving \ac{LA} performance.

\subsection{Environment, Methods and Data Collection}
\label{subsec:collection}
We now describe: the environment used to collect the data and test the methods; the methods considered in simulations; the data collection process.
\subsubsection{Environment} All simulations have been run on an internal Ericsson \ac{RAN} simulator platform compliant with the \ac{3GPP} \ac{5G} standard specification. The software infrastructure allows running multiple independent network simulations of pre-defined length in parallel, each specifying a different seed. 
%All simulations consider a multi-cell \ac{mMIMO} system with \acp{UE} randomly dropped in the simulated network area and full buffer traffic. 
We consider a \ac{TDD} 5G system operating at a 3.5GHz carrier frequency, with PHY layer numerology $\mu=0$ of the \ac{3GPP} technical specifications 38.211 and \ac{SU-MIMO} transmission.
%single-user Multi-Input Multi-Output (SU-MIMO) transmission. 
Each base station is configured with a \ac{mMIMO} %MIMO (mMIMO) 
8x4x2 antenna array. 
We consider 1 site, 3 sectors, and a fixed number of 10 UEs with full buffer traffic, thereby experiencing stable interference conditions.  For each simulation (i.e., a seed) the duration is 5 seconds.

\subsubsection{Methods} We compare the performance of two value-based offline \ac{RL} algorithms, \ac{BCQ} \cite{fujimoto2019off} and \ac{CQL} \cite{kumar_conservative_2020}, with \ac{DT}. 
%In its discrete variant, \ac{BCQ} \cite{fujimoto_benchmarking_2019} tackles the distributional shift issue by restricting the support of action selection to a subset of actions whose probability is at least $\tau$ times the probability of the action most likely to be selected by the behavioral policy. On the other hand, \ac{CQL} \cite{kumar_conservative_2020} modifies the training objective to minimize, alongside the Bellman error, the estimates of the q-values to learn lower-bounded estimates that are not overly optimistic, which is a known issue in offline \ac{RL}. We design the \ac{DT} agent as described in Section \ref{DT modifications}. Choices regarding the hyperparameters are detailed in Table \ref{table: hyperparameters}.
Three baselines have been considered. The first one is the \ac{OLLA} approach introduced in  \cref{sec:problem formulation}, the second one is simple \ac{BC} and as a last one we consider the performance of the behavioral \ac{DQN} policy. Performance evaluation has been conducted across $50$ randomized scenarios simulations, {\color{red}choices regarding the hyperparameters are detailed in the appendix}. 
%Table \ref{table: hyperparameters}


\subsubsection{Data Collection}
We collected training data by interacting with the environment using two DQN policies. A first dataset, $\mathcal{D}_{\rm opt}$, was collected using a DQN policy $\pi_{\rm opt}$ that was trained until convergence; a second dataset, $\mathcal{D}_{\rm s-opt}$, was collected using a DQN policy $\pi_{\rm s-opt}$ that was trained on half the data (compared to $\pi_{\rm opt}$). This approach tests whether offline RL algorithms can infer optimal behavior from non-optimal training data in LA. %Additionally, we logged a unique ID for each UE requesting transmission alongside each transition tuple, allowing us to reconstruct sequences of packets for each UE.
We collected data across $20$ seeds, resulting in datasets of $\sim 400K$ transitions. The two \ac{DQN} policies have been trained online on, respectively, $100$ seeds for collecting $\mathcal D_\text{opt}$, and $50$ for $\mathcal D_\text{s-opt}$. %\sam{sam: should we mention d3rlpy?}


% We generated 150 randomized scenarios during training that randomize across several variables (e.g., UEs movement and traffic). Each scenario lasted $5$ seconds.  

% Additional simulation assumptions related to the network scenario are summarized in Table 7.1 (values per simulation seed).


% Training data is collected by direct interaction with the environment using a previously trained \ac{RL} policy.  We choose to consider two training datasets, $\mathcal{D}_\text{opt}$ and $\mathcal{D}_\text{s-opt}$, respectively containing optimal and sub-optimal behavior. Both are collected with a \ac{DQN} policy: while the first one is trained up to convergence, the second one is trained on half the data. By doing this, we hope to put to the test the potential of offline \ac{RL} algorithms to infer optimal behavior even from non-optimal training data in \ac{LA}.  Additionally, we found it helpful to log a unique ID associated with the \ac{UE} requesting the transmission alongside the tuple representing each transition. This allows us to reconstruct sequences of packets for each \ac{UE}.

% \textcolor{red}{We believe that similar findings would be obtained by training on datasets containing real-world data collected by the currently deployed rule-based algorithms. REMOVE AND TALK IN THE INTRODUCTION}






\begin{table*}[t!]
\centering
\begin{minipage}{0.48\linewidth}  % First table in half of the page width
    \centering
    \caption{Comparison of the offline RL methods trained on $\mathcal{D}_{\rm opt}$. \\ OLLA (x\%) refers to OLLA with a fixed BLER target of x\%.}
    \setlength{\tabcolsep}{8pt} % Adjust the column spacing
    \begin{tabular}{lccc}
    \hline
    \toprule\toprule
        \ac{LA} algorithm & Throughput & \ac{SE} & \ac{BLER} \\
    \toprule
        OLLA ($10\%$) & 14.76 Mbps   & 6.21 bps/Hz   & 0.13     \\
        OLLA ($30\%$) & 15.51 Mbps   & 6.87 bps/Hz   & 0.30     \\
        OLLA ($50\%$) & 15.16 Mbps   & 6.92 bps/Hz   & 0.49     \\
        OLLA ($70\%$) & 14.77 Mbps   & 6.81 bps/Hz   & 0.66     \\
        OLLA ($90\%$) & 14.71 Mbps   & 6.84 bps/Hz   & 0.83     \\
        DQN$_{\rm opt}$   & 16.02 Mbps   & 7.50 bps/Hz   & 0.32     \\
        BC            & 16.10 Mbps   & 7.53 bps/Hz   & 0.30     \\
        BCQ           & 16.11 Mbps   & 7.53 bps/Hz   & 0.30     \\
        CQL           & 16.10 Mbps   & 7.52 bps/Hz   & 0.30     \\
        DT            & 16.07 Mbps   & 7.46 bps/Hz   & 0.31     \\
    \bottomrule\bottomrule
    \hline
    \end{tabular}
    \vspace{0.25cm} % Adjust vertical space between table and caption
    \label{table: opt table}
\end{minipage}
\hspace{0.02\linewidth}  % Small space between the two tables
\begin{minipage}{0.48\linewidth}  % Second table in half of the page width
    \centering
    \caption{Comparison of the offline RL methods trained on $\mathcal{D}_{\rm s-opt}$. \\ OLLA (x\%) refers to OLLA with a fixed BLER target of x\%.}
    \setlength{\tabcolsep}{8pt} % Adjust the column spacing
    \begin{tabular}{lccc}
    \hline
    \toprule\toprule
        \ac{LA} algorithm & Throughput & \ac{SE} & \ac{BLER} \\
    \toprule
        OLLA ($10\%$) & 14.76 Mbps   & 6.21 bps/Hz   & 0.13     \\
        OLLA ($30\%$) & 15.51 Mbps   & 6.87 bps/Hz   & 0.30     \\
        OLLA ($50\%$) & 15.16 Mbps   & 6.92 bps/Hz   & 0.49     \\
        OLLA ($70\%$) & 14.77 Mbps   & 6.81 bps/Hz   & 0.66     \\
        OLLA ($90\%$) & 14.71 Mbps   & 6.84 bps/Hz   & 0.83     \\
        DQN$_{\rm s-opt}$ & 15.89 Mbps   & 7.45 bps/Hz   & 0.33     \\
        BC            & 16.00 Mbps   & 7.50 bps/Hz   & 0.31     \\
        BCQ           & 16.00 Mbps   & 7.60 bps/Hz   & 0.34     \\
        CQL           & 16.05 Mbps   & 7.59 bps/Hz   & 0.33     \\
        DT            & 15.67 Mbps   & 7.25 bps/Hz   & 0.36     \\
    \bottomrule\bottomrule
    \hline
    \end{tabular}
    \vspace{0.25cm} % Adjust vertical space between table and caption
    \label{table: s-opt table}
\end{minipage}
\end{table*}


\subsection{General Results}

\cref{table: opt table,table: s-opt table} present the  results of in terms of throughput, \ac{BLER} and \ac{SE}: offline \ac{RL} models in  \cref{table: opt table} have been trained on $\mathcal{D}_{\rm opt}$, while models in  \cref{table: s-opt table} on $\mathcal{D}_{\rm s-opt}$. When considering $\mathcal{D}_{\rm opt}$, we notice how the offline \ac{RL} methods achieve comparable results across all the considered metrics, with \ac{CQL} and \ac{BCQ} scoring slightly better than \ac{DT}. Yet, they are only able to match the performance of the \ac{BC} baseline.
However, when considering suboptimal training data $\mathcal{D}_{\rm s-opt}$, the differences are more noticeable.   \ac{CQL} reaches almost the same performance as models trained on $\mathcal{D}_\text{opt}$  in terms of \ac{SE}. On the other hand, when trained on data that is suboptimal, \ac{DT} is not able to match the performance of the behavioral policy. Our results for both settings show that \ac{BC} seems to work sufficiently well on this use-case. \sam{Plots in Fig. \ref{cdf} look at the CDF curves resulting from the experiments on $\mathcal{D}_{\rm opt}$.




\subsection{Considerations on the \ac{DT} design}
In \cref{table:pe and conditioning - throughput} we show results for different combinations of the positional encoder and conditioning methods proposed in  \cref{sec:method} for the Decision Transformer (we only consider results obtained by training on $\mathcal{D}_\text{opt}$).

Including temporal information about packet distribution using the \ac{LT} encoding appears to be beneficial compared to both BE and \ac{CT} encoding, with these two achieving similar performance. Specifically, learning embeddings directly from the actual timestamps of packet transmissions leads to substantial performance improvements, while using an encoding based on trigonometric functions (i.e., \ac{CT}) results in worse performance.

%Including information about the distribution of packets in time with the use of \ac{LT} encoding appears to be beneficial with respect to both the BE and \ac{CT} encoding, with these two achieving very similar performance. Interestingly, using the timestamps of packet transmissions to learn embeddings (i.e.: \ac{LT}) brings substantial improvements to performance, while an encoding based on trigonometric functions (i.e.: \ac{CT}) achieves worse performance. 

Regarding \ac{RTG} conditioning, our results in \cref{table:pe and conditioning - throughput} indicate that \ac{3GPP} conditioning achieves better throughput than both VANILLA and DAVG conditioning across all types of positional encoding. We observed similar results in terms of \ac{BLER} and \ac{SE}, which are not included here for brevity. This evidence supports our hypothesis that conditioning differently based on channel conditions is beneficial.

%Concerning \ac{RTG} conditioning, our results in  \cref{table:pe and conditioning - throughput} indicate that \ac{3GPP} conditioning achieves better throughput\footnote{We observed similar results in terms of \ac{BLER} and \ac{SE}, which are not included for ease of presentation.} compared to VANILLA and AVG conditioning, across all types of positional encoding. This evidence supports our hypothesis that it is reasonable to condition differently depending on the channel conditions.

For the VANILLA and DAVG conditioning types, we conditioned on the 90\% quantile of the distribution of RTGs in the training dataset (filtered at the first retransmission in the case of VANILLA conditioning). The average future rewards are computed over a fixed window size of $35$ steps, with a discount factor $\gamma = 0.8$. The results reported here have been obtained following the first of the two approaches to trajectory definition introduced in Section \ref{trajectory definition}, with $H=32$.

 %Results for the VANILLA and AVG conditioning types are obtained by conditioning on the $90\%$ quantile of the distribution of \acp{RTG} in the training dataset (filtered at the first retransmission, in case of vanilla conditioning). \textcolor{red}{Average, future rewards are computed on a fixed window size of $35$ steps, with $\gamma=0.8$.}


\begin{table}[]
\centering
\caption{Comparison of different types of position encoding and RTG conditioning. Best in \textbf{bold}, second best in red.}
\renewcommand{\arraystretch}{1.25}
\begin{tabular}{lccc}
\toprule\toprule
PE type    & VANILLA       & 3GPP          & DAVG           \\ \hline
BE          & 15.75 Mbps & 15.83 Mbps & 15.76 Mbps \\
CT              & 15.35 Mbps & 15.86 Mbps & 15.73 Mbps \\
LT & \textcolor{red}{16.01 Mbps} & \textbf{16.07 Mbps} & 15.66 Mbps \\
\bottomrule\bottomrule
\end{tabular}
\label{table:pe and conditioning - throughput}
\end{table}

\subsection{Analysis of Outcome Conditioning}
\label{RTG conditioning}

\begin{table}[t!]
    \centering
    \setlength{\tabcolsep}{3pt}
    \caption{Performance obtained by conditioning on increasing, fixed, RTG values at inference for models including variable numbers of packets inside their sequence (vanilla).}
    \begin{tabular}{llllll}
    \toprule\toprule
    $n_p$ & Metrics      & 3GPP     & $\omega=1.71$  & $\omega=3.86$ & $\omega=7.57$ \\ \hline
         & Th.put    & 15.73 Mbps & 15.30 Mbps & 13.80 Mbps & 13.94 Mbps \\
    1    & BLER          & 0.37       & 0.33       & 0.42       & 0.83       \\
         & SE            & 7.45 bps/Hz & 7.14 bps/Hz & 6.92 bps/Hz & 7.19 bps/Hz \vspace{3mm} \\
         & Th.put    & 15.72 Mbps & 15.08 Mbps & 13.75 Mbps & 13.98 Mbps \\
    2    & BLER          & 0.38       & 0.31       & 0.41       & 0.82       \\
         & SE            & 7.45 bps/Hz & 7.08 bps/Hz & 6.87 bps/Hz & 7.25 bps/Hz \vspace{3mm} \\
         & Th.put    & 16.02 Mbps & 15.93 Mbps & 15.45 Mbps & 14.06 Mbps \\
    4    & BLER          & 0.31       & 0.28       & 0.36       & 0.74       \\
         & SE            & 7.43 bps/Hz & 7.32 bps/Hz & 7.45 bps/Hz & 7.46 bps/Hz \vspace{3mm} \\
         & Th.put    & 16.04 Mbps & 16.01 Mbps & 15.96 Mbps & 14.49 Mbps \\
    8    & BLER          & 0.28       & 0.27       & 0.30       & 0.62       \\
         & SE            & 7.40 bps/Hz & 7.34 bps/Hz & 7.42 bps/Hz & 7.56 bps/Hz \vspace{3mm} \\
         & Th.put    & 16.02 Mbps & 15.93 Mbps & 15.45 Mbps & 14.06 Mbps \\
    12   & BLER          & 0.31       & 0.30       & 0.31       & 0.46       \\
         & SE            & 7.45 bps/Hz & 7.42 bps/Hz & 7.46 bps/Hz & 7.58 bps/Hz \vspace{3mm} \\
         & Th.put    & 16.02 Mbps & 15.93 Mbps & 15.45 Mbps & 14.06 Mbps \\
    16   & BLER          & 0.30       & 0.29       & 0.31       & 0.40       \\
         & SE            & 7.44 bps/Hz & 7.42 bps/Hz & 7.44 bps/Hz & 7.48 bps/Hz \\
    \bottomrule\bottomrule
    \end{tabular}
    \label{table: more-packets}
\end{table}

In this section, we analyze the \ac{RTG} conditioning of the \ac{DT}, as discussed in \cref{subsec:conditioning}. We start by considering input sequences that comprise transmissions related to a single packet (i.e., $n_p=1$), we then extend the analysis by incrementally increasing the number of packets included in the input sequences. This approach allows us to better observe the effect of conditioning on different \ac{RTG} values during inference and to determine the extent to which the \ac{DT} can replicate the target \ac{RTG} values.

%In this section we analyse the \ac{RTG} conditioning of the DT, as discussed in \cref{subsec:conditioning}. We start by considering input sequences comprising transmissions relative to one single packet (i.e.: $n_p=1$) and then extend the analysis to include an increasing number of packets to better observe the effect of conditioning on different values at inference and find out to what extent \ac{DT} can replicate target \ac{RTG} values.

\Cref{table: more-packets} shows the performance of \ac{DT} when we vary the target \ac{RTG} value $\omega$ across the $q\%$ quantiles of the training \ac{RTG} distribution, with $q\in \{20,60,100\}$. As expected, conditioning the action generation on higher target \ac{RTG} values causes the \ac{DT} to take more aggressive actions and leads to an increased frequency of retransmissions during testing, reflected by a higher \ac{BLER}. Conversely, we observe a decreasing trend in throughput, with the \ac{3GPP} baseline achieving the best performance due to the induced correlation between the target \ac{RTG} values and the channel conditions.

% \cref{table: more-packets} shows the performance of \ac{DT} by sweeping the value of the target \ac{RTG} value $\omega$ over the $q\%$ quantiles of the training distribution of \acp{RTG} (with $q \in [0.2, 0.6, 1.0]$). As expected, conditioning the generation of actions on increasing target values of \ac{RTG} causes \ac{DT} to take more aggressive actions and, as a consequence, retransmissions at inference time increase in frequency (\ac{BLER}); at the same time, we notice an opposite trend in terms of throughput, with \ac{3GPP} achieving yet again the best performance because of the induced correlation between the target value and channel conditions.

As we include more packets in the sequences, the average performance tends to improve. However, when experiments involve sequences with eight or more packets, the \ac{BLER} values converge to those achieved by the behavioral DQN policy. These results imply that while the \ac{DT} can effectively model short sequences of packet transmissions, incorporating longer sequences likely introduces too much variance. This increased variance may cause the \ac{DT} to default to simply cloning the behavioral policy, as suggested by the poor performance shown in \cref{table: s-opt table}. Consequently, this effect prevents the 
\ac{DT} from extrapolating optimal behavior from suboptimal data. \sam{See the Appendix in the complete version of the paper for more on this (ArXiv: https://arxiv.org/abs/2410.23031).}

%As more packets are included inside sequences, average performance seems to increase. However, alues of \ac{BLER} achieved across experiments with $8$ or more packets seem to converge to the value of \ac{BLER} achieved by the behavioral \ac{DQN} policy. These results imply that, while \ac{DT} seems to be able to correctly model short sequences of packet transmissions, considering longer sequences probably introduces too much variance causing \ac{DT} to revert to simple cloning of the behavioral policy and, as suggested by the poor performance shown in  \cref{table: s-opt table}, preventing the extrapolation of optimal behavior from suboptimal data.

% According to the definition introduced in Section \ref{DT modifications}, we start by considering input sequences comprising transmissions relative to one single packet (i.e.: $n_p=1$) to better observe the effect of conditioning on different values at inference and find out to what extent \ac{DT} can replicate target \ac{RTG} values.

% Table \ref{table:1-packet sweep} shows the performance of \ac{DT} by sweeping the value of the target \ac{RTG} value $\omega$ over the $q\%$ quantiles of the training distribution of \acp{RTG} (with $q \in [0.1, 0.2, ..., 1.0]$). As expected, conditioning the generation of actions on increasing target values of \ac{RTG} causes \ac{DT} to take actions that are more aggressive and, as a consequence, retransmissions at inference time increase in frequency (\ac{BLER}). Consequently, we observe that conditioning on a single high return regardless of channel conditions leads to worse throughput performance; indeed, Table \ref{table:pe and conditioning - throughput} shows that the best throughput is achieved by \ac{3GPP} conditioning, which correlates the \ac{RTG} conditioning variable to the observed channel state.

% Table \ref{table: more-packets} extends the very same analysis to include increasing numbers of packets inside input sequences. Similarly to what we could observe in the previous case, as we condition on bigger $\omega$ values the experienced \ac{BLER} grows and, at the same time, we notice a decreasing trend in terms of throughput; with \ac{3GPP} conditioning achieving yet again the best performance. Unsurprisingly, as longer input sequences are considered, we experience better results across all metrics (with a maximum found at $n_p=8$). However, the values of \ac{BLER} achieved across experiments with $8$ or more packets seem to converge to the value of \ac{BLER} achieved by the behavioral \ac{DQN} policy. These results imply that, while \ac{DT} seems to be able to correctly model short sequences of packet transmissions, considering longer sequences probably introduces too much variance causing \ac{DT} to revert to simple cloning of the behavioral policy and, as confirmed by the poor performance shown in Table \ref{table: s-opt table}, preventing the extrapolation of optimal behavior from suboptimal data.

==> old_versions/backup_2024_11_18/7_conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
In this paper, we explored offline \ac{RL} approaches for \ac{LA}. %Link Adaptation (LA). 
Our simulations showed offline \ac{RL} methods, being able to match the performance of state-of-the-art online \ac{RL} methods, to constitute a viable alternative to solve \ac{LA}. However, as mentioned in Section \ref{sec:introduction}, further work should be directed toward the study of an effective way to collect quality data that is, also,  feasible to implement in a live network. Additionally, although our findings are based on a simulator and a single setup, 
they may generalize to other data collection strategies.

Furthermore, we adapted the \ac{DT} architecture for \ac{LA}. We enhanced performance by modifying positional encoding and attention masks and by conditioning on channel quality indicators to handle irregular time intervals and to ensure causality. However, \ac{DT} struggles with the stochastic nature of \ac{LA} due to interference and varying channel conditions, which affect its ability to select optimal actions. In particular, we notice that while \ac{DT} is able to correctly condition the inference of optimal actions when dealing with sequences comprising few packet transmissions, when input sequences become longer the inherent variance of \ac{LA} makes it hard for \ac{DT} to model the stochasticity intrinsic to the process correctly.

Despite these challenges, our work provides valuable insights into applying machine learning in telecommunication networks and supports the use of offline \ac{RL} methods to train agents for live networks.

% Our simulations showed that offline \ac{RL} methods slightly improve upon the behavioral policy used for data collection, 
% starting from both optimal and suboptimal policies. 
 
% In this paper, we have addressed the problem of \ac{LA} by adopting alternative approaches to offline \ac{RL}. 

% Our thorough comparison run on a proprietary \ac{RAN} simulator has demonstrated the capabilities of the offline \ac{RL} methods we considered to obtain performances that slightly improve on the behavioral policy employed for collecting the training dataset, both in the case of optimal and suboptimal behavior. Despite employing datasets collected by a \ac{RL} trained online, we believe that similar findings may be valid regardless of the policy used for data collection. However, the use of the simulator poses some limitations to our work, and, also, the validity of our results is limited to one single simulation setup.

% One important contribution of this work is the sequence modeling framework we provide to solve \ac{LA} using a \ac{DT} architecture. The modifications we proposed contribute to the performance of the vanilla architecture when employed as a solution to the use case, in particular: the adjustments to the positional encoding definition are relevant as a way to represent the distribution of consecutive steps of an \ac{MDP} in which steps do not happen in discrete series of timesteps, the new definition of the attention mask guarantees causality at training time in a delayed-feedback setting and, finally, we found beneficial to correlate the target value used for conditioning the inference of optimal actions with an indication of the channel quality. Unfortunately, our results show \ac{DT} to be very liable to the stochasticity of the \ac{LA} process (due to stochastic interference and time- and frequency-varying channel conditions), preventing the model from correctly modeling the distribution of sequence realizations and, therefore, correctly conditioning the selection of optimal actions.

% Nonetheless, we believe this work to constitute a valuable contribution to the literature of \ac{ML} in telecommunication networks and a great starting point for those practitioners considering offline \ac{RL} methods to overcome the problems associated with training agents in live networks.




==> old_versions/backup_2024_11_25/0_abstract.tex <==

\begin{abstract}

\Ac{LA} is an essential function in modern wireless communication systems that dynamically adjusts the transmission rate of a communication link to match time- and frequency-varying radio link conditions.
%
However, factors such as user mobility, fast fading, imperfect channel quality information, and aging of measurements \gf{make the modeling of LA} challenging, which leads to \gf{relying} on suboptimal, rule-based algorithms. 
%
To bypass the need for explicit modeling, recent research has introduced online \ac{RL} approaches. Yet, these approaches face deployment challenges, as training in live networks can potentially degrade real-time performance.
%
To address this challenge, this paper considers offline RL \ps{as~a candidate} to learn LA policies with minimal effects~on the network operation. 
%
We propose three LA designs based on batch-constrained deep Q-learning, conservative Q-learning, and decision transformers. 
\gf{Our results show} that offline~RL algorithms can achieve the performance of state-of-the-art online RL methods when data is collected with a proper behavioral policy.
\end{abstract}

\acresetall % Must reset the usage of acronyms so that they get properly
% introduced in the main body as well !

==> old_versions/backup_2024_11_25/1_introduction.tex <==
\section{Introduction}\label{sec:introduction}

\begin{comment}
    Modern \acp{RAN} -- such as the \ac{5G} \ac{NR} system -- employ model-based \ac{LA} algorithms to adapt the \ac{MCS} to time-- and frequency-varying channel conditions to maintain high spectral efficiency\iffalse while adhering to \ac{BLER} targets\fi ~\cite{duran_self-optimization_2015, blanquez-casado_eolla_2016, Blanquez-Casado:19, Ramireddy:22, Nicolini:23}. Both in \ac{TDD} and \ac{FDD} systems, \ac{LA} in the \ac{DL} relies on \ac{CSI} reports provided by the \ac{UE} that include a \ac{CQI}, a rank indicator, and a precoder matrix indicator~\cite{3rd_generation_partnership_project_3gpp_technical_2024}.

    As \ac{CSI} reports may be inaccurate and rapidly age due to variations in channel and interference conditions, an \ac{OLLA} scheme is typically adopted to adjust \ac{SINR} estimates inferred from inaccurate or aged~\acp{CQI} to adhere to \ac{BLER} targets based on the \ac{HARQ} feedback~\cite{duran_self-optimization_2015}. Nonetheless, user mobility, fast fading, limited receiver-side information at the transmitter, as well as the heterogeneity of \acp{UE} population, e.g., in terms of receiver and hardware capabilities, render \ac{RRM} problems in \acp{RAN}, like \ac{LA}, complex control tasks to model~\cite{Chen:23, generalization_2024}.
\end{comment}


Modern \acp{RAN} -- such as the \ac{5G} \ac{NR} system -- employ model-based \ac{LA} algorithms to adapt the \ac{MCS} to time-- and frequency-varying channel conditions to maintain high spectral efficiency\iffalse while adhering to \ac{BLER} targets\fi ~\cite{duran_self-optimization_2015, blanquez-casado_eolla_2016, Blanquez-Casado:19, Ramireddy:22, Nicolini:23}. \gf{For} \ac{DL} communication, \ac{LA} relies on \ac{CSI} reports provided by the \ac{UE} that include a \ac{CQI}, a rank indicator, and a precoder matrix indicator~\cite{3rd_generation_partnership_project_3gpp_technical_2024}.
%
As \ac{CSI} reports may be inaccurate and rapidly age due to fast channel variations\iffalse variations in radio conditions\fi, an \ac{OLLA} scheme typically \gf{adjusts} \ac{SINR} estimates inferred from~\ac{CQI} values using \ac{HARQ} feedback~\cite{duran_self-optimization_2015}. Nonetheless, user mobility, fast fading, limited receiver-side information at the transmitter, as well as the heterogeneity of \acp{UE} population, e.g., in terms of receiver \iffalse and hardware\fi capabilities, \gf{render \ac{RRM} problems, such as \ac{LA}}, complex control tasks to model~\cite{Chen:23}.

Recognizing the challenges faced by model-based approaches, \ac{ML} methods, such as \ac{RL}, have recently gained attention to address \ac{RRM} problems in \acp{RAN}~\cite{calabrese_learning_2018}, where time- and frequency-varying channel conditions often make rule-based algorithms suboptimal. The ability of \ac{RL} to learn directly from experience and to adapt to changes in the environment makes it appealing to replace legacy rule-based \ac{RAN} functions with models learned from data~\cite{generalization_2024}. Several works have applied \ac{RL} to \ac{LA}, starting with tabular~\cite{Bruno:14} and bandit~\cite{saxena_reinforcement_2021} methods, adaptations of \ac{OLLA} based on Q-learning~\cite{Chen:23}, and \ac{DQN}-based designs intended to replace \ac{OLLA}~\cite{generalization_2024}.
%
However, training \ac{RL} agents in live networks requires to explore the state-action space to learn~an optimal policy, at the cost of taking suboptimal actions that may \gf{adversely} affect the network performance~\cite{russo2024model}.

To address this adverse effect of \ac{RL}, recent works have proposed offline \ac{RL}, which aims to learn learn an optimal policy from a \emph{static dataset} of transitions produced by a behavioral policy, thus avoiding direct interactions with the environment while training~\cite{levine_offline_2020-1, janner2021offline, schweighofer2022dataset, Kumar:23, lyu2022mildly}. The inability to improve the training dataset during training \gf{confines} the quality and the behavior of the learned policy to the quality and state-action coverage of the available data. As such, distribution shift and out-of-distribution behavior, that is, a mismatch between the training and testing trajectory distributions, can render the learned policy ineffective.
%As the training dataset is not augmented during training, the quality and the behavior of the learned policy is constrained by the quality and state-action coverage of the available data. As such, distribution shift and out-of-distribution behavior, that is, a mismatch between the training and testing trajectories, can render the learned policy ineffective. %Thus employing offline \ac{RL} in complex real-time control problems, such as \ac{LA}, is non-trivial.
%\gf{\it GF: One paragraph about offline RL and the out-of-distribution and distribution shift problems and the concept 
%of transformers, as well as maybe other main concepts that must not come out of the blue later (maybe attention mechanisms ?).}
%
Thus, employing offline \ac{RL} to replace complex real-time \ac{RRM} control functions in \acp{RAN}, such as \ac{LA}, is non-trivial and presents two main challenges: firstly, the ability of an offline \ac{RL} design to achieve, when trained with proper data, optimal performance, e.g., comparable with a policy learned online; secondly, the design of a non-invasive behavioral policy to collect rich data in live networks without affecting performance.
\begin{comment}
    To capitalize the advantages of \ac{RL} over rule-based approaches while reducing the potentially negative impact of active exploration on the \acp{RAN} operation, this paper considers offline RL to design LA in 5G networks. We propose three LA designs  based on \ac{BCQ}~\cite{fujimoto_off-policy_2019}, \ac{CQL}~\cite{kumar_conservative_2020}, and \ac{DT}~\cite{chen_decision_2021}. While for \ac{BCQ} and \ac{CQL} we model the \ac{LA} problem as a partially observable \ac{MDP}, for \ac{DT} we consider a sequence modeling approach, where an \ac{LA} action for a packet transmission (or retransmission) is inferred based on a sequence of historical states, actions and rewards. Our results show that offline \ac{RL} algorithms can achieve performance of state-of-the-art online \ac{RL} when data is collected with a proper behavioral policy.
\end{comment}

This paper focuses on the first challenge considering offline \ac{RL} for \ac{LA} in \ac{5G} networks. We present three \ac{LA} designs based on \ac{BCQ}~\cite{fujimoto2019off}, \ac{CQL}~\cite{kumar_conservative_2020}, and \ac{DT}~\cite{chen_decision_2021}, with  a trained \ac{DQN} model \cite{mnih_playing_2013} acting as a behavioral policy for data collection. While for \ac{BCQ} and \ac{CQL} we model the \ac{LA} problem as a partially observable \ac{MDP}, \ac{DT} requires a sequence modeling approach, where \gf{an} \ac{LA} action is inferred using a sequence of historical states, actions and rewards, allowing to optimize long-term rewards, e.g.,~average throughput or spectral efficiency. Our results show that offline \ac{RL} can achieve the performance of online \ac{RL} and outperform practical state-of-the-art \ac{LA} based on \ac{OLLA}  when data is collected with a proper behavioral policy.



%% REMOVED 4 ARXIV %%
The rest of the paper is organized as follows. Section~\ref{sec:background}~introduces preliminary concepts, Section~\ref{sec:problem formulation} formally describes the problem of \ac{LA} while Section~\ref{sec:problem} presents the \ac{BCQ} and \ac{CQL} design for \ac{LA}. Section~\ref{sec:method} frames \ac{LA} as a sequence modeling problem, presenting a \ac{DT}-based design. Section~\ref{sec:experiments} discusses numerical results, while Section~\ref{sec:conclusion} concludes the paper.

\begin{comment}
to employ \ac{BCQ}  and \ac{CQL} 
for \ac{LA} in 5G networks, which are
value-based algorithms for offline \ac{RL} \cite{fujimoto_off-policy_2019}, \cite{kumar_conservative_2020}.  
In its discrete variant, \ac{BCQ} tackles the distributional shift issue by restricting the support 
of action selection to a subset of actions whose probability is at least $\tau>0$ times the probability 
of the action most likely selected by the behavioral policy, \gf{where $\tau$ is ... }  \cite{fujimoto_benchmarking_2019}. 
In contrast, \ac{CQL} modifies the training objective to minimize -- alongside the Bellman error \cite{Sutton:14} -- 
the estimates of the Q-values to learn lower-bounded estimates that are not overly optimistic \cite{kumar_conservative_2020}.
%which is a known issue in offline \ac{RL}  \cite{kumar_conservative_2020}.
\gf{\it GF: Need $\sim 2$ more sentences on (1) why using BCQ and CQL is challenging to employ specifically for LA and (2) how we address these challenges (at a very high level), "the punch line". 
This is just a teaser that motivates the reviewer/reader to read further.}    

\sam{SAM: mention reason for data collection with dqn maybe}

\gf{\it GF: 1. Check the consistency across the title, abstract, index terms and intro. 2. The intro should not exceed 1 page.}

\textbf{Possible ways to present contributions}
\begin{itemize}
    \item focus more broadly on offline RL
    \item offline RL modelling for link adaptation using CQL, BCQ and DT. More effort needed to design DT.
    \item evelautaion with industrial simulator
    \item be open about data collection policy
    \item show that we can replicate performance of DQN, and discuss remaining problems
    \item future work...
\end{itemize}

\end{comment}






==> old_versions/backup_2024_11_25/2_background.tex <==
\section{Preliminaries}\label{sec:background}
This section reviews some of the key concepts and introduces notation that will be useful in the sequel.

\subsection{Elements of \ac{RL}}

\ac{RL} frames the interaction between an agent and the environment as a \ac{MDP} \cite{Sutton:14,puterman2014markov}, defined by the tuple: $(\mathcal{S, A, P}, r)$. Here, $\mathcal{S}$ is the state-space, $\mathcal{A}$ is the action-space, $\mathcal{P}$ is the transition probability function (also known as transition dynamics), $r:\mathcal{S}\times\mathcal{A}\times\mathcal{S}\to\mathbb{R}$ is the reward function.
In an online setting, at each time-step $t$ the agent chooses an action $a_t$ according to some Markovian policy $\pi:{\cal S}\to {\cal A}$, which is function of the current state $s_t$ of the MDP, and observes the next state $s_{t+1}$, distributed according to $P(\cdot|s_t,a_t)$, and a reward $r_t$. 
For episodic MDPs, with a finite terminal state, the goal of the agent is to find a policy $\pi$ maximizing the expected collected reward $\mathbb{E}^\pi[G_t|s_0\sim \mu]$ for some initial state distribution $\mu$, where
$
    G_t = \sum_{k=0}^T r_{t+k},
$
and $T$ indicates the terminal step. In the context of \textit{continuing task}, where $T$ is not naturally defined, or may be infinite, the goal is to maximize the collected discounted reward, defined with a  discount factor $\gamma\in (0,1)$ as $
    \mathbb{E}^\pi[\sum_{k=0}^\infty \gamma^k r_{t+k+1}|s_0\sim \mu]
$.
\begin{comment}
In settings where $T$ is not naturally defined, we introduce the notion of \textit{continuing task} and re-define the return to include the discount factor $\gamma$: $
    G_t = \sum_{k+0}^\infty \gamma^k r_{t+k+1}.
$
\end{comment}

\subsection{Offline RL}
Differently from the online \ac{RL} setting, in offline \ac{RL} \cite{levine_offline_2020} the agent learns a policy from a previously collected dataset of experiences $\mathcal{D} = \{( s_t^i, a_t^i, r_{t}^i,s_{t+1}^i)_i\}$ (collected using a behavioral policy $\pi_\beta$).
As a consequence, the amount of data, and its quality, play a crucial role in offline \ac{RL}, since the agent is not able to interact with the environment in an online fashion to collect new data. 
%While the goal of offline \ac{RL} remains the maximization of returns, in this framework agents no longer interact with the environment during training to collect new transitions using a behavioral policy $\pi_\beta$. 
%Instead, the learning algorithm shall derive a sufficient understanding of the \ac{MDP} dynamics exclusively from transitions available in a static \textit{training dataset} $\mathcal{D} = \{( s_t^i, a_t^i, s_{t+1}^i, r_{t+1}^i)_i\}$ collected by a behavioral policy $\pi_\beta$ prior to training. 
The inability to explore the state-action space during training may result in a distributional shift between the distribution under which the policy $\pi$ is trained and the one on which it will be evaluated \cite{levine_offline_2020}.

To address this issue, some approaches constraint how much the learned policy $\pi$ differs from the behavioral policy~$\pi_\beta$, while other methods penalize the learned $Q$-values. For example, with discrete action spaces, \ac{BCQ} tackles the distributional shift issue by \sam{modeling the data distribution resulting from data collection with a certain behavioral policy so that the support of action selection can be restricted to a fixed number of actions sampled from it \cite{fujimoto2019off}.}
%
In contrast, \ac{CQL} \cite{kumar_conservative_2020} uses a \emph{pessimism} principle: it modifies the training objective to minimize, alongside the Bellman error \cite{Sutton:14}, the estimates of the $Q$-values to learn lower-bounded estimates that are~not overly optimistic. A comprehensive survey can be found~in~\cite{levine_offline_2020}.


 


\begin{comment}
    While the goal is still the maximization of returns, in the offline \ac{RL} framework agents no longer have the ability to interact with the environment and collect additional transitions using the behavioral policy. This limits the possibility of exploring the state-action space to the transitions included in a static \textit{training dataset} $\mathcal{D} = \{( s_t^i, a_t^i, s_{t+1}^i, r_{t+1}^i)_i\}$, forcing the learning algorithm to derive a sufficient understanding of the \ac{MDP} dynamics exclusively from the available transitions. The challenge addressed by offline \ac{RL} is the distributional shift between the distribution under which the function approximator (policy, value function, or model) is trained and the one on which it will be evaluated. The simplest solution consists in bounding the distributional shift by constraining how much the learned policy $\pi$ differs from the behavioral policy $\pi_\beta$, with different algorithms employing slightly different approaches. A comprehensive review can be found in~\cite{levine_offline_2020}.
\end{comment}

%\\

% \textcolor{blue}{This work is going to consider \ac{BCQ} \cite{fujimoto_off-policy_2019} and \ac{CQL} \cite{kumar_conservative_2020}, two of the main value-based algorithms for offline \ac{RL}. In its discrete variant, \ac{BCQ} \cite{fujimoto_benchmarking_2019} tackles the distributional shift issue by restricting the support of action selection to a subset of actions whose probability is at least $\tau$ times the probability of the action most likely to be selected by the behavioral policy. On the other hand, \ac{CQL} \cite{kumar_conservative_2020} modifies the training objective to minimize, alongside the Bellman error, the estimates of the Q-values to learn lower-bounded estimates that are not overly optimistic, which is a known issue in offline \ac{RL} }


%     \begin{figure*}
%     \centering
%     \begin{minipage}{.49\textwidth}
%     \includegraphics[width=\textwidth]{Figures/olla_v1.2.png}
%     \caption{Visual description of the functioning of Link Adaptation.}
%     \label{fig:olla schema}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{.49\textwidth}
%     \includegraphics[width=\textwidth]{Figures/sequence_1.png}
%     \caption{Episodes in our MDP formulation for LA. Each box represents a TTI, and acknowledgements use the same color as the transmission they respond to. Between TTI 5 and 7 two packets are active, with episodes 1 and 2 overlapping. \textcolor{red}{TODO: make picture more narrow}}
%     \label{fig:sequence_1}
%     \end{minipage}
% \end{figure*}

\subsection{Sequence Modeling and Decision Transformer} 
Sequence modeling involves training auto-regressive models (such as the \ac{DT} \cite{chen_decision_2021}) on sequential data to capture patterns and make future predictions. Since the goal in \ac{RL}~is~to produce a sequence of actions leading to high cumulative rewards, one can re-frame the RL problem in terms of sequence modeling.

The \ac{DT} is a particular auto-regressive architecture used in sequence modeling that exploits the capabilities of GPT2~\cite{radford_language_2019} to perform sequential decision making. For each time step $t$ of a trajectory, \ac{DT}  uses sequences of $3$ embedded tokens: the state $s_t$, the action $a_t$, and the \ac{RTG} $\hat R_t = \sum_{t'=t}^T r_{t'}$. 
At inference time the \ac{RTG} allows to condition the output of the network to generate optimal actions by specifying \textit{future target} returns.
% Note that it is of particular importance  the \ac{RTG}: at inference time it allows to condition the output of the network by specifying \textit{future target} returns.
The model is trained by predicting the action $a_t$ at each time-step of the sequence. Overall, this architecture allows to bypass the need for bootstrapping to propagate returns, one of the key destabilizing elements in offline \ac{RL}.






==> old_versions/backup_2024_11_25/3_problem.tex <==
\section{Problem Formulation}\label{sec:problem formulation}
We consider the problem of \ac{LA} in the downlink of multi-cellular \acp{RAN}. The aim of LA is to dynamically adapt the transmission rate of individual packet transmissions to time- and frequency-varying channel conditions and radio interference. In \ac{5G} systems, this is achieved by selecting a set of \ac{MCS} parameters encoded by an integer taking value in the range~$\{0,31\}$,  known as the \ac{MCS} index~\cite{3rd_generation_partnership_project_3gpp_technical_2024}. Each \ac{MCS} index corresponds to a modulation order, code rate, and spectral efficiency to be used for transmitting a data packet to the \ac{UE}.

State-of-the-art \ac{LA} algorithms used in real-time \acp{RAN} combine two control loops executed on a sub-millisecond~timescale: an \ac{ILLA} converts the latest \ac{CQI} reported by the \ac{UE} into an initial \ac{SINR} estimate; an \ac{OLLA} scheme adjusts such an estimate (e.g., to compensate inaccuracies or aging of the \ac{CQI}) based on the \ac{HARQ} feedback (i.e., either positive or negative acknowledgments) received from the \ac{UE} for previous packet transmissions. The goal of the \ac{OLLA} is to maximize the link spectral efficiency while adhering to a desired \ac{BLER} target. As variants of this approach are widely adopted in today's communication systems, we consider it as reference for performance comparison in Section~\ref{sec:experiments}. 



%In this section, we first present \ac{LA} as framed for solving it as a control problem and then provide a formulation as a \ac{MDP}: we are going to consider this alternative formulation for training and evaluation of value-based offline \ac{RL} methods as well as data collection.


    
%\subsection{Pure Control Formulation}\label{olla}
%Traditional \ac{LA} algorithms rely on the combination of an inner- and \ac{OLLA} to reconstruct an estimate of the \ac{UE} \ac{SINR}: the \ac{ILLA} converts a \ac{CQI} to an initial estimate according to some pre-defined, link level curves while \ac{OLLA} adjusts such an estimate to take into account uncertainties in the \ac{CQI} transmission by means of a feedback loop acting on the received \ac{HARQ} signals (i.e., either positive or negative acknowledgments). \Ac{OLLA} algorithms circumvent the inherent complexity in modeling link adaptation by fixing a target \ac{BLER} value, defined as the experienced frequency of packet retransmissions. %\textcolor{red}{However, while several transmissions are required for OLLA to converge to the \ac{SINR} adjustments meeting the desired \ac{BLER}, traffic for most \acp{UE} consists of short bursts of transmissions. Furthermore, most implementations require to specify a fixed \ac{BLER}, which is not optimal for all channel conditions. Figure \ref{fig:olla schema} provides a visual description of the \ac{LA} process, highlighting the different stages of the above-described solution. THIS MAY BE REMOVED AND STAY ONLY IN THE INTRO?}


==> old_versions/backup_2024_11_25/4_LA_as_offline_RL.tex <==
\section{Link Adaptation as an Offline RL Problem}\label{sec:problem}
This section explores how \ac{LA} can be solved with offline \ac{RL}. \sam{We first propose a \ac{MDP} formulation which we not only consider for training offline \ac{RL} agents but, being particularly well-suited for online approaches as well, also for performing data collection. Then, we introduce the minimal modifications that are needed, given the chosen \ac{MDP} formulation, to adapt the \ac{BCQ} and \ac{CQL} algorithms to the \ac{LA} setting.}


% We begin by presenting our \ac{MDP} formulation of LA and then discuss how offline \ac{RL} methods, like \ac{BCQ} and \ac{CQL}, can be applied to solve this \ac{MDP} formulation.

%     \begin{figure}
%     \centering

%     \includegraphics[width=0.5\textwidth]{tikz_imgs}
%     \caption{Episodes in our MDP formulation for LA. Each box represents a TTI, and acknowledgements use the same color as the transmission they respond to. Between TTI 5 and 7 two packets are active, with episodes 1 and 2 overlapping. \textcolor{red}{TODO: make picture more narrow}}
%     \label{fig:sequence_1}
% \end{figure}

\begin{figure}
    \centering
    % Resize the combined TikZ images to fit within the column width
    \resizebox{\linewidth}{!}{%
    \input{tikz_imgs/img_harq_example}
    }
    \caption{Episodes in our \ac{MDP} formulation for LA. Each box represents a \ac{TTI}, and acknowledgments use the same color as the transmission they respond to. Note that episodes 1 and 2 overlap between \ac{TTI} 5 and 12.}
    \label{fig:sequence_1}
\end{figure}
\subsection{\ac{MDP} Formulation}  

We model \ac{LA} as an episodic \ac{MDP} in which an episode (or trajectory) $\tau=(s_0,a_0,r_0,\dots, s_T,a_T,r_T)$  corresponds to the lifespan of a \ac{UE}'s data packet from its first transmission to, alternatively, a successful reception or the packet being dropped after four retransmissions (as illustrated in~\cref{fig:sequence_1}). As such, the episode's length $T$ is bounded to five steps (each corresponding to a transmission of the packet).
\begin{itemize}
    \item The state $s_t \in \mathbb{R}^n$ is a vector of semi-static and dynamic information characterizing the serving cell, the \ac{UE} design, as well as radio measurements, channel state information, \ac{HARQ} feedback, and more\footnote{The exact list of states cannot be disclosed as it is based on Ericsson's internal research work.}.
    \item The action $a_t\in \{0,\dots,27\}$ takes an integer, representing one of 28 \ac{MCS} indices for data transmissions, as defined by the \ac{5G} specifications~\cite{3rd_generation_partnership_project_3gpp_technical_2024}. When dealing with a re-transmission, that is $t\geq 1$,  the simulator maps the agent's action to a reserved \ac{MCS} index in the interval $\{28,\dots,31\}$, as per \ac{5G} specifications.
    \item  The reward signal $r_t=r(s_t,a_t)$ is function of the \ac{SE} of the packet transmission. 
\end{itemize}

Additionally, as the \ac{UE}'s \ac{HARQ} process supports multiple active packets at any given time, multiple \ac{UE}'s episodes may overlap in time (as in the example in~\cref{fig:sequence_1}). 

\subsection{\ac{BCQ} and \ac{CQL} for Link Adaptation}
\sam{We train both algorithms on static datasets of transitions in the form of $(s_t,a_t,r_{t+1},s_{t+1})$ tuples. The definition of the episode on a packet basis enables agents to learn from experience generated by any \ac{UE} within the network. The formulation detailed above allows \gf{to adapt} \ac{CQL} and \ac{BCQ} to \ac{LA} with minimum effort: in particular, when dealing with a finite set of actions, such as \ps{those representing \ac{MCS} indices selectable for} \ac{LA}, \ac{BCQ} can overcome the need to explicitly model the distribution of actions in the dataset by simply computing probabilities for each action being selected by the behavioral policy. 
\gf{Therefore}, inspired by \cite{fujimoto_benchmarking_2019}, we restrict the support of action selection to a subset of actions whose probability exceeds the probability of the action most likely selected by the behavioral policy by a minimum threshold. \ps{For training a \ac{CQL} policy}, instead, we control the \textit{tradeoff-factor} {\color{red}by selecting fixed values of $\alpha$} instead of relying on the automatic tuning used in \cite{kumar_conservative_2020} \ps{for} continuous action spaces.}


% \ps{We need to add a description of how a link adpatation policy can be trained for BCQ and CQL}


% \subsection{Solving LA with Offline \ac{RL}}
% The proposed \ac{MDP} modeling enables an \ac{RL} agent to learn from experiences generated by any \ac{UE} within the network. Hence, it is particularly well-suited both for online and offline \ac{RL} approaches thanks to the large amounts of data collected in the network. 

% We consider this formulation to train a \ac{DQN} policy  to serve as behavioral policy for data collection as well as performance reference for offline \ac{RL}. As training data samples for offline \ac{RL} consist of state-action-reward tuples $(s_t,a_t,r_t)$, we can consider the evaluation and training of value-based and actor-critic methods~\cite{Sutton:14}.  

% We propose two offline \ac{RL} algorithms for \ac{LA} based on \ac{BCQ}~\cite{fujimoto2019off}, and \ac{CQL}~\cite{kumar_conservative_2020}, respectively. 

% {\color{red}[@Alessio, @Samuele]: could we add a couple of sentences to indicate in what way you designed these algorithms for LA? It does not need to long}

%Training data samples for offline \ac{RL} are represented by state-action-reward tuples $(s_t,a_t,r_t)$, which allows for the evaluation and training of value-based and actor-critic methods \cite{Sutton:14}. Consequently, this formulation is particularly well-suited for use with offline \ac{RL}, as it can exploit the large amounts of data collected in the network to train a policy using a fixed dataset \cite{levine_offline_2020}.

%{\color{blue} [PS]: I would add here a description of the LA design based on BCQ and CQL and move the sequence modeling paragraph to the beginning of Sec IV}
\begin{comment}
  \paragraph{Sequence modeling}
However, there are some shortcomings with this modeling of LA. Firstly, such formulation optimizes only over one packet at the time, without considering sequences of multiple packets. Secondly, since packet arrivals are unknown and channel conditions are time-varying, the overall stochastic process we aim to control can be more generally framed as a \emph{contextual} \ac{MDP} \cite{hallak2015contextual}. A contextual \ac{MDP} is a specific type of \ac{MDP} that includes an underlying time-varying hidden parameter (context) affecting the transition dynamics—such as packet arrivals and channel conditions. Managing such a process is generally more complex than controlling a classical \ac{MDP} \cite{kaelbling1998planning}. To address these complexities, we propose a sequence modeling approach \cite{janner2021offline,emmons_rvs_2021}, a method to efficiently handle sequences of data.  
\end{comment}
    



==> old_versions/backup_2024_11_25/5_sequence_modelling_for_LA.tex <==
\section{Sequence Modeling for Link Adaptation}\label{sec:method}

The previous \ac{MDP} formulation of \ac{LA}, and thereby the related offline \ac{RL} designs,  present some shortcomings. Firstly, such formulation optimizes the return for individual packets. Thus, it may not capitalize that sequences of packets can experience correlated channel conditions that would allow to optimize longer-term metrics (e.g., \ac{UE} throughput). Secondly, since packet arrivals are unknown and channel conditions are time-varying, the overall stochastic process we aim to control can be more generally framed as a \emph{contextual} \ac{MDP} \cite{hallak2015contextual}. A contextual \ac{MDP} is a specific type of \ac{MDP} that includes an underlying time-varying hidden parameter (context) affecting the transition dynamics—such as packet arrivals and channel conditions. Managing such a process is generally more complex than controlling a classical \ac{MDP} \cite{kaelbling1998planning}. 

To address these complexities, \ps{we reformulate offline \ac{RL} for \ac{LA} as a sequence modeling problem \cite{janner2021offline,emmons_rvs_2021}\iffalse, a method to efficiently handle sequences of data\fi~and propose a solution that extends and adapts the \ac{DT} design \cite{chen_decision_2021}.}
%We then outline our contributions in adapting the original \ac{DT} design \cite{chen_decision_2021} to the \ac{LA} problem.

\subsection{RL via Supervised Learning (RvS)}
%Sequence modeling involves training auto-regressive models on sequential data to capture patterns and make future predictions. Since the main goal in \ac{RL} is to produce a sequence of actions leading to high cumulative rewards, we can re-frame the RL problem in terms of sequence modeling.

By framing RL as a sequence modeling problem, we can better capture the time-varying interactions in the underlying process. This approach \iffalse{\color{red} simplifies various design decisions} and\fi leverages the strengths of sequence models in handling temporal dependencies.

We consider the \ac{RvS} learning approach for offline RL proposed in \cite{emmons_rvs_2021}. This approach takes as input a dataset ${\cal D}=\{\tau\}$ of trajectories of experience and outputs an \emph{outcome-conditioned} policy $\pi_\theta(a_t\mid s_t,\omega)$ that optimizes
\begin{equation}
    \max_\theta \mathbb{E}_{\tau \sim {\cal D}}\left[\sum_{t=0}^{|\tau|-1} \mathbb{E}_{\omega \sim f(\omega\mid \tau_t)}\left[ \ln \pi_\theta(a_t\mid s_t,\omega)\right]\right],
\end{equation}
where $\tau_t=\{s_t,a_t,r_t,s_{t+1},\dots\}$ denotes the trajectory starting at time $t$, $|\tau|$ denotes the trajectory length, and $f(\omega|\tau)$  denotes the distribution over outcomes $\omega$ that occur in a trajectory. These outcomes are user-chosen, and can be, for example:
\begin{itemize}
    \item \emph{Goal-oriented}: $\omega=\{s_{h}=s\}$, that is, $f(\omega|\tau)$ indicates the likelihood of visiting state $s$ at step $h$.
    \item \emph{Reward-oriented}: $\omega=\sum_{n\geq t}\gamma^{n-t} r_n$, and $f(\omega|\tau)$ indicates the likelihood of achieving a certain total discounted  reward starting from $t$. Such conditioning is also referred to as \emph{return-to-go} (RTG).
\end{itemize}
At inference-time, then, the user can choose to condition the policy according to the desired objective.

\subsection{RvS Learning for LA}
To formulate  \ac{LA}  in terms of the \ac{RvS} learning framework, we introduce a trajectory definition that extends beyond the lifespan of a single packet, departing from the previous \ac{MDP} formulation.  After that, we introduce different ways to condition the policy $\pi_\theta$.
 %After that, we introduce our proposed reward-oriented conditioning, as well as  a particular type of ci
%This extension allows us to leverage a \ac{DT} approach for \ac{LA}, benefiting from the transformer's ability to perform long-term credit assignment by considering long sequences spanning multiple packet transmissions.


\subsubsection{Trajectory definition} \label{trajectory definition} We consider fixed-horizon trajectories $\tau=\{s_0,a_0,r_0,\dots, s_H,a_H,r_H\}$, which include  transmissions of packets belonging to a specific \ac{UE}.

%. Letting $3K$ denote the transformer's context size, each sequence can include tokens corresponding to up to $K$ transmissions, with extra positions filled using padding tokens.
We consider two alternative approaches to construct $\tau$:

\begin{enumerate}[label=\alph*)]
    \item \emph{Recent transmissions}:  $\tau$ consists of the most recent $K$ transmissions of the \ac{UE} considered (hence $H=K$).
    \item \emph{Consecutive packets}: $\tau$ includes only up to  $n_p$ of a \ac{UE}'s most recent consecutive packets. Since a packet can be retransmitted at most four times upon its initial transmission, we have that $H\in\{n_p,\dots, 5n_p\}$.
\end{enumerate}
At training time, \sam{we sample trajectories of data from ${\cal D}$  according to one of these two approaches} and, if needed, extra positions in $\tau$ are filled using padding tokens.

% To formulate the \ac{LA} functionality as a sequence modeling problem, we introduce a trajectory definition that departs from the previous \ac{MDP} formulation and extends the episode horizon beyond the lifespan of a packet. This allows us to leverage a \ac{DT} approach for \ac{LA} and benefit from the transformer's ability in performing long-term credit assignment by considering long sequences of tokens that span across transmissions for multiple packets. Specifically, we define a trajectory to include all the transmissions of packets belonging to a certain \ac{UE} in a simulation. Letting $3K$ denote the context size of the transformer, tokens relative to up to $K$ transmissions can be included in each sequence, with extra positions being filled with padding tokens. We consider two alternative approaches: (1) a sequence consisting of the most recent $K$ transmissions relative to a certain \ac{UE}; (2) a sequence including transmissions relative to $n_p$ of a \ac{UE}'s most recent consecutive packets. Considering~$5$ as the maximum number of retransmission, each sequence will include a number of transmissions in $[n_p, 5n_p]$. 



% \subsection{DT design modifications}
% \label{DT modifications}
% \ac{LA} has some fundamental differences when compared to standard \ac{RL} baselines such as those considered in the original \ac{DT} paper \cite{chen_decision_2021}. In this section, we present the main modifications to its design that we found necessary for our use case.


\subsubsection{Outcome conditioning}\label{subsec:conditioning} We propose the following three ways to condition the policy $\pi_\theta$ for \ac{LA}:
\begin{enumerate}[label=\alph*)]
    \item {\bf VANILLA}: This is a simple conditioning that consists in fixing a target \ac{RTG} value $\omega$ for each packet $p$. At training time, the \ac{RTG} at the $k$-th step of a packet is computed as  $\omega=\sum_{t=k}^{T(p)} \gamma^{t-k} r_k(p)$, where $r_k(p)$ indicates the reward associated to the $k$-th transmission for packet $p$, $\gamma \in(0,1]$, and  $T(p)$ is a random variable indicating the termination step for the transmission of packet $p$. At inference time, the \ac{RTG} is fixed to a pre-defined value at the first transmission and adjusted in case of retransmissions (we expand on this in~\cref{sec:experiments}).

    \item {\bf \Ac{DAVG}}: The VANILLA approach has the same shortcomings of the MDP formulation proposed in \cref{sec:problem}. An alternative is to condition according to a \ac{DAVG} of  future rewards. Letting $n$ denote the $n$-th step in a sequence of continuous transmissions from a UE, at training time we condition according to:
    \[
           \omega=(1-\gamma)\sum_{t=n}^\infty \gamma^{t-n}r_t,
    \]
    with $\gamma \in(0,1)$.   At inference time, as for the VANILLA case, we condition according to some pre-defined value.
    \item {\bf \Ac{CCTR}}: \ps{As the definition of the reward signal (cf.~\cref{sec:problem}), directly relates to the channel's spectral efficiency, we propose a novel method that dynamically adapts the policy $\pi_\theta$'s conditioning based on the observed channel quality. Specifically, we consider the nominal spectral efficiency associated to the latest \ac{CQI} value reported by the \ac{UE} as \ac{RTG} target value for the first transmission of a packet, using Table 5.2.2.1\text{-}3 of the \ac{3GPP} specification~\cite{3rd_generation_partnership_project_3gpp_technical_2024}.} 
    %A similar approach could also be taken considering different reward definitions by choosing different reference mappings.
    %Lastly, we propose a novel conditioning method based on the observation that the reward signal, as mentioned in \cref{sec:problem}, directly relates to the channel's spectral efficiency. We therefore condition the policy $\pi_\theta$ according to a nominal spectral efficiency value given the channel quality. To this end, as \ac{RTG} target value, we use the nominal spectral efficiency associated to the latest \ac{CQI} value reported by the \ac{UE}, using Table 5.2.2.1\text{-}3 of the \ac{3GPP} specification~\cite{3rd_generation_partnership_project_3gpp_technical_2024}.
\end{enumerate}

%Lastly, we propose a novel conditioning method based on the observation that the reward signal, as mentioned in \cref{sec:problem}, is directly related to the spectral efficiency of the channel. Therefore, we condition the policy $\pi_\theta$ according to a nominal spectral efficiency value given the channel quality. Specifically, at each first packet transmission, depending on the \ac{CQI} value reported by the \ac{UE} in the state $s$, we use the corresponding nominal spectral efficiency from the \ac{CQI} Table 5.2.2.1\text{-}3 of the \ac{3GPP} specification~\cite{3rd_generation_partnership_project_3gpp_technical_2024} as the target \ac{RTG} value.




% When shifting to a trajectory definition including all of a \ac{UE}'s transmissions it becomes unfeasible to compute \acp{RTG} on an infinite horizon. Furthermore, in radio communications, packets’ transmissions that are distant in time are roughly independent and the knowledge about future rewards is unlikely to be useful for generating optimal actions for earlier packets. Taking inspiration from the framework described by Emmons et al. in \cite{emmons_rvs_2021}, we propose the following expression as a new objective definition for \ac{LA}:

% \begin{itemize}
%     \item VANILLA: 
%         \begin{equation}
%             V(p)=\mathbb{E}\left[\sum_{k=0}^{T(p)} r_k(p)\right].
%         \end{equation}
%     \item AVG
%         \begin{equation}
%             RTG(i_0)=\mathbb E_{\tau \sim \mathcal{D}} \left[\sum_{i=i_0}^{|\tau|-1} \gamma_0^{i-i_0}r_i\right], 
%         \end{equation}
% \end{itemize}

% \begin{equation}
% \label{equation:final objective definition}
%     \mathbb E_{\Upsilon \sim \rho} \left[\sum_{n=n_0}^\infty \gamma_0^{t_n-t_{n_0}}V(p_n)\right], 
% \end{equation}
% where with $V(p)$ we refer to the value of a packet, defined as:
% \begin{equation}
%     V(p)=\mathbb{E}\left[\sum_{k=0}^{T(p)}\gamma_1^k r_k(p)\right].
% \end{equation}

% In such a formulation, $\Upsilon$ denotes a sequence of packets transmitted at random times, where $\rho$ is the distribution over packets and time. $\gamma_0$ and $\gamma_1$ are discount factors respectively affecting the sum of the values of successive packets and successive retransmissions for a single packet. $t_n$ is the time of transmission of packet $n$, with $t_{n_0}$ being the time of transmission of the first packet of the sequence. $T(p)$ is a random variable indicating the termination step for the transmission of packet $p$. Finally, $r_k(p)$ indicates the reward associated to the $k$-th transmission for packet $p$.

% The formulation is general enough that by setting $\gamma_0=0$ the objective converges to a packet basis, similar to the objective for the formulation described in \ref{MDP formulation}; by choosing $0 < \gamma_0 < 1$ the objective instead becomes a discounted sum of future rewards. We can imagine the first case as conditioning \ac{DT} on intermediate goals for each packet. 

% \textcolor{blue}{In the following sections we present results obtained by setting $\gamma_0 = 0$ or, alternatively, by simply computing average returns on a window with fixed size of $M$ transitions, discounting rewards at each transmission.}


% \subsubsection{Conditioning at inference}
% At inference time, we propose three different ways of conditioning the generation of actions. (1) \textbf{VANILLA} consists in fixing a target \ac{RTG} value $\omega$ for each packet, $\omega$ is fixed at the first transmission and adjusted in case of retransmissions; (2) \textbf{3GPP}, similarly to VANILLA, at each first packet transmission selects a target \ac{RTG} value according to the \ac{3GPP} \ac{CQI} Table 5.2.2.1-3 in \cite{3rd_generation_partnership_project_3gpp_technical_2024}, depending on the \ac{CQI} value reported by the \ac{UE} inside the state; (3) \textbf{AVG} conditions each step with the same value of average \ac{RTG} as a target. 

\subsection{Decision Transformers Design for LA}

We next describe how we adapted the \ac{DT} architecture for the link adaptation problem. We introduce two changes: one to the attention layer, and one for the positional embedding.
\begin{figure}[t]
    \centering
    % Resize the combined TikZ images to fit within the column width
    \resizebox{\linewidth}{!}{%
    \input{tikz_imgs/img_attention_mask}
    }
    \caption{\textbf{At training time}, the proposed attention mask (right matrix) prevents the tokens associated to $p_2$ and $p_4$ from attending $p_1$, as its reward is not available at the time an MCS index is requested for $p_2$ and $p_4$. The left matrix shows the original attention mask definition.}
    \label{fig: attn mask}
\end{figure}


% \begin{figure}
%     \centering
%     % Resize the combined TikZ images to fit within the column width
%     \resizebox{\linewidth}{!}{%
%     \input{tikz_imgs/img_sequence_builing}
%     }
%     \caption{Given a trajectory $\tau$ (relative to a single \ac{UE}), input sequence (a) is built by setting $K=4$ while sequence (b) is built with $n_p=2$. The first index in the notation $t_{i,j}$ identifies the transmission count while the second is a unique packet id. A same color also identifies transmissions for a same packet.}
%     \label{fig: sequence building}
% \end{figure}

\subsubsection{Attention masking for delayed feedback}

\begin{comment}
A significant challenge in training a \ac{DT} architecture for \ac{LA} is preventing the leakage of future data during the training process. To perform inference, historical rewards are only available upon a base station receiving a \ac{HARQ} feedback (either positive or negative) for previous packet transmissions. Hence, it is essential to ensure that \ac{DT}'s outputs during training rely solely on information available in real-time, avoiding any use of future data that would not be accessible in an actual deployment.
\end{comment}
A significant challenge in training a \ac{DT} architecture for \ac{LA} is preventing the leakage of future data during the training process. \ps{Specifically, the \ac{DT}'s inference outputs must rely solely on information available as in real-time}, avoiding any use of future data that would not be accessible in an actual deployment. As historical rewards are only available upon a base station receives a \ac{HARQ} feedback (either positive or negative) for previous packet transmissions, \ps{we propose an attention masking that copes with such delayed feedback while enforcing causality}.

\ps{To this end, we model a trajectory~$\tau$~as} \[\tau=(\underbrace{s_0}_{X_{0}},\underbrace{a_0}_{X_1},\underbrace{r_0}_{X_2},\dots, \underbrace{s_K}_{X_{3K}}, \underbrace{a_K}_{X_{3K+1}}, \underbrace{r_K}_{X_{3K+2}}),\]
\ps{where $(X_0, X_1,\dots, X_{3K+2})$ indicates the associated sequence of input tokens, and we define $t_a(p)$ and $t_r(p)$ as the time at which, respectively,  the action for packet $p$ is scheduled and the associated reward signal is available. The proposed attention mask between any two tokens $X_i,X_j $ is}
\[
\hbox{\texttt{attn\_mask}}(X_i,X_j) = \mathbf{1}\{ t_r(p(X_i)) \leq t_a(p(X_j))\},
\]
\ps{where $p(X)$ is a mapping between a token $X$ and the associated packet $p$.
As illustrated in \cref{fig: attn mask}, the mask assures that if a reward for a packet $p(X_i)$ is not received when an action for a packet $p(X_j)$ is taken, then tokens of packet $p(X_j)$ should not be affected by the tokens of packet $p(X_i)$.}

\input{plots}
% Formally, by referring to the instant in time at which the action for packet $i$ is scheduled with $t_{a,i}$ and the instant in time the associated reward signal is received with $t_{r,i}$, we apply:
% \begin{align}
%         \begin{array}{rcl}
%             \text{given a sequence of tokens }\left[T_0, T_1, ..., T_{3 \cdot \text{seq\_len}-1} \right], \\
%             \forall T_i,T_j, \text{ if } t_{r,i} > t_{a,j} \text{ then } attn(i,j) = -\infty,
%         \end{array}
%     \end{align}
% where $attn(i,j)$ represents the un-normalized attention score between token~$i$~and~$j$. 

\iffalse
\ps{To this end, we model a trajectory~$\tau$~as} \[\tau=(\underbrace{s_0}_{X_{0}},\underbrace{a_0}_{X_1},\underbrace{r_0}_{X_2},\dots, \underbrace{s_K}_{X_{3K}}, \underbrace{a_K}_{X_{3K+1}}, \underbrace{r_K}_{X_{3K+2}}),\]
where $(X_0, X_1,\dots, X_{3K+2})$ \ps{indicates the} sequence of input tokens, and we define $t_a(p)$ and $t_r(p)$ as the time at which, respectively,  the action for packet $p$ is scheduled and the associated reward signal is available. Lastly, \ps{we let $p(X)$ denote a mapping between a token $X$ to the corresponding packet $p$.} The proposed attention mask for delayed feedback between any two tokens $X_i,X_j $ can then be expressed as
\[
\hbox{\texttt{attn\_mask}}(X_i,X_j) = \mathbf{1}\{ t_r(p(X_i)) \leq t_a(p(X_j))\}.
\]
In other words, if we have not yet received any reward for packet $p(X_i)$, then the tokens of the packet $p(X_j)$ should not be affected by the tokens of packet $p(X_i)$. \cref{fig: attn mask} describes such a formulation visually.
\fi

\subsubsection{Temporal embeddings}
% \ac{LA} is a real-time process where states (sim. actions) are observed at points in time that are not equidistant between each other. The DT architecture was designed for processes with an equidistant sampling. We propose to capture the correlation in time between successive packet transmissions by modifying the \ac{DT} positional encoding. 
\ac{LA} is a real-time process with \ps{states, actions, and rewards} observed at irregular intervals, whereas the \ac{DT} architecture assumes equidistant sampling. \ps{To handle irregular observations, we propose three positional encodings that capture temporal correlations between successive packet transmissions of a \ac{UE}:}
%
%To capture the temporal correlations between successive packet transmissions of a \ac{UE}, we consider the following modifications of the \ac{DT}'s positional encoding:
\begin{enumerate}
    \item \textbf{\Ac{BE}}: as a baseline, we implement a minor modification to the original encoder from \cite{chen_decision_2021}, where embeddings are learned based on each token's index within the sequence ($i \in [0, K-1]$).
    \item \textbf{\Ac{LT} encoding}: 
    embeddings are learned using a linear layer with $(\Delta {t}_i)_{i=0}^K$ as input, where $\Delta t_i= t_a(p(X_i)) - t_a(p(X_0))$. Hence, $\Delta {t}_i$ is a measure of the relative time  between the $i$-th token and the first one.
    Note that tokens within the same packet have identical relative timestamps, allowing the \ac{DT} to associate the reward to the corresponding state and action.

    \item \textbf{\Ac{CT} encoding}: inspired by \cite{zuo2020transformer, zhang2023continuous},  we compute the $k$-th element of the positional embedding vector for token $X_i$ as:
\begin{equation}
    \textup{PE}(\Delta t_i, k) = \begin{cases}
    \sin\left(\displaystyle \frac{\Delta t_i / 100}{{C}^{\frac k {d_\text{model}}}}\right) & \text{ for even } k, \\[4ex]
    \cos\left(\displaystyle \frac {\Delta t_i / 100} {C^{\frac {k-1} {d_\text{model}}}}\right) & \text{ for odd } k,
    \end{cases}
    \end{equation}
    where $d_{\text{model}}$ is a user-chosen constant (see also  \cite{zhang2023continuous}).
\end{enumerate}


==> old_versions/backup_2024_11_25/6_experiments.tex <==
\section{Numerical Results}\label{sec:experiments}

\begin{comment}
    In this section, we empirically compare the considered offline \ac{RL} methods using an industry-grade simulator. We evaluate their performance in terms of throughput, experienced \ac{BLER}, and \ac{UE} \ac{SE}\iffalse across all \ac{MIMO} layers allocated for transmission\fi. Specifically, we investigate: (1) whether offline \ac{RL} methods can match the performance of the behavioral policy and of OLLA; (2) how the behavioral policy affects performance of these methods; and (3) the impact of different design aspects of the \ac{DT} on \ac{LA} performance\iffalse whether our modifications to the \ac{DT} design improve \ac{LA} performance\fi.
\end{comment}

This section compares the various offline \ac{RL} designs for \ac{LA} using an industry-grade simulator. Specifically, we investigate: (1) whether offline \ac{RL} methods can match the performance of the behavioral policy and \ac{OLLA}; (2) how the behavioral policy affects performance of these methods; and (3) the impact of different design aspects of the \ac{DT} on \ac{LA} performance\iffalse whether our modifications to the \ac{DT} design improve \ac{LA} performance\fi.


\subsection{Environment and Data Collection}
\label{subsec:collection}
%We now describe: the environment used to collect the data and test the methods; the methods considered in simulations; the data collection process.
\begin{comment}
    \subsubsection{Environment} All simulations have been run on an internal Ericsson \ac{RAN} simulator platform compliant with the \ac{3GPP} \ac{5G} standard specification. The software infrastructure allows running multiple independent network simulations of pre-defined length in parallel, each specifying a different seed. 
%All simulations consider a multi-cell \ac{mMIMO} system with \acp{UE} randomly dropped in the simulated network area and full buffer traffic. 
We consider a \ac{TDD} 5G system operating at a 3.5GHz carrier frequency, with PHY layer numerology $\mu=0$ of the \ac{3GPP} technical specifications 38.211 and \ac{SU-MIMO} transmission.
Each base station is configured with a \ac{mMIMO} 8x4x2 antenna array. 
We consider a tri-sectorial site with 10 UEs with full randomly dropped and buffer traffic, which provides favorable condition for the \ac{OLLA} baseline. For each simulation (i.e., a seed) the duration is 5 seconds.
\end{comment}

\subsubsection{Environment} We rely on an Ericsson's proprietary \ac{RAN} simulator platform compliant with the \ac{3GPP} \ac{5G} technical specification. Specifically, we consider a \ac{TDD} 5G system operating at a 3.5GHz carrier frequency, with PHY layer numerology $\mu=0$ (cf. \ac{3GPP} TS 38.200 family) and \ac{SU-MIMO} transmission. Each simulation consists of a tri-sectorial site, with each sector served by a \ac{mMIMO} 8x4x2 antenna array, and 10 UEs with full buffer traffic randomly dropped in the site coverage area. Each simulation (i.e., seed) simulates 5 seconds (i.e., $\approx$5000 \acp{TTI}).  


\subsubsection{Data collection}
To investigate the potential of offline \ac{RL} to achieve optimal performance (e.g., comparable with a policy learned online) when trained with proper data,  we collect training data using two \ac{DQN} policies pre-trained online: A \ac{DQN} policy $\pi_{\rm opt}$ trained until convergence; and a sub-optimal \ac{DQN} policy $\pi_{\rm s-opt}$ trained with half the data of $\pi_{\rm opt}$. The latter allows us to analyze whether offline \ac{RL} algorithms can infer optimal behavior from sub-optimal training data. For each policy, we collected data across $20$ seeds, resulting into two datasets $\mathcal{D}_{\rm opt}$ and $\mathcal{D}_{\rm s-opt}$, respectively, of $\approx 400k$ transitions. %This approach tests whether offline \ac{RL} algorithms can infer optimal behavior from non-optimal training data in LA.

\begin{comment}
 We collected training data by interacting with the environment using two DQN policies. A first dataset, $\mathcal{D}_{\rm opt}$, was collected using a DQN policy $\pi_{\rm opt}$ that was trained until convergence; a second dataset, $\mathcal{D}_{\rm s-opt}$, was collected using a DQN policy $\pi_{\rm s-opt}$ that was trained on half the data (compared to $\pi_{\rm opt}$). This approach tests whether offline RL algorithms can infer optimal behavior from non-optimal training data in LA. %Additionally, we logged a unique ID for each UE requesting transmission alongside each transition tuple, allowing us to reconstruct sequences of packets for each UE.
We collected data across $20$ seeds, resulting in datasets of $\sim 400K$ transitions. The two \ac{DQN} policies have been trained online on, respectively, $100$ seeds for collecting $\mathcal D_\text{opt}$, and $50$ for $\mathcal D_\text{s-opt}$. %\sam{sam: should we mention d3rlpy?}   
\end{comment}

\begin{comment}
   \subsubsection{Methodology} 
We compare the performance of three \ac{LA} designs based on value-based offline \ac{RL}, with \ac{BCQ} \cite{fujimoto2019off} and \ac{CQL} \cite{kumar_conservative_2020}, and sequence modeling with \ac{DT}. We consider three baselines: the \ac{OLLA} approach introduced in~\cref{sec:problem formulation}, representing the state-of-the-art in real-world \acp{RAN}; a simple \ac{BC} approach, which learns to reproduce actions;  and the behavioral \ac{DQN} policy. We tested the algorithm using $50$ randomized simulation scenarios. We refer to \cite{Peri_2024} for an extended description. 
\end{comment}



\begin{table*}[t!]
\centering
\begin{minipage}{0.48\linewidth}  % First table in half of the page width
    \centering
    \caption{Comparison of the offline RL methods trained on $\mathcal{D}_{\rm opt}$. \\ OLLA (x\%) refers to OLLA with a fixed BLER target of x\%.}
    \setlength{\tabcolsep}{8pt} % Adjust the column spacing
    \begin{tabular}{lccc}
    \hline
    \toprule\toprule
        \ac{LA} algorithm & Throughput & \ac{SE} & \ac{BLER} \\
    \toprule
        OLLA ($10\%$) & 14.76 Mbps   & 6.21 bps/Hz   & 0.13     \\
        OLLA ($30\%$) & 15.51 Mbps   & 6.87 bps/Hz   & 0.30     \\
        OLLA ($50\%$) & 15.16 Mbps   & 6.92 bps/Hz   & 0.49     \\
        OLLA ($70\%$) & 14.77 Mbps   & 6.81 bps/Hz   & 0.66     \\
        OLLA ($90\%$) & 14.71 Mbps   & 6.84 bps/Hz   & 0.83     \\
        DQN$_{\rm opt}$   & 16.02 Mbps   & 7.50 bps/Hz   & 0.32     \\
        BC            & 16.10 Mbps   & 7.53 bps/Hz   & 0.30     \\
        BCQ           & 16.11 Mbps   & 7.53 bps/Hz   & 0.30     \\
        CQL           & 16.10 Mbps   & 7.52 bps/Hz   & 0.30     \\
        DT            & 16.07 Mbps   & 7.46 bps/Hz   & 0.31     \\
    \bottomrule\bottomrule
    \hline
    \end{tabular}
    \vspace{0.25cm} % Adjust vertical space between table and caption
    \label{table: opt table}
\end{minipage}
\hspace{0.02\linewidth}  % Small space between the two tables
\begin{minipage}{0.48\linewidth}  % Second table in half of the page width
    \centering
    \caption{Comparison of the offline RL methods trained on $\mathcal{D}_{\rm s-opt}$. \\ OLLA (x\%) refers to OLLA with a fixed BLER target of x\%.}
    \setlength{\tabcolsep}{8pt} % Adjust the column spacing
    \begin{tabular}{lccc}
    \hline
    \toprule\toprule
        \ac{LA} algorithm & Throughput & \ac{SE} & \ac{BLER} \\
    \toprule
        OLLA ($10\%$) & 14.76 Mbps   & 6.21 bps/Hz   & 0.13     \\
        OLLA ($30\%$) & 15.51 Mbps   & 6.87 bps/Hz   & 0.30     \\
        OLLA ($50\%$) & 15.16 Mbps   & 6.92 bps/Hz   & 0.49     \\
        OLLA ($70\%$) & 14.77 Mbps   & 6.81 bps/Hz   & 0.66     \\
        OLLA ($90\%$) & 14.71 Mbps   & 6.84 bps/Hz   & 0.83     \\
        DQN$_{\rm s-opt}$ & 15.89 Mbps  & 7.45 bps/Hz   & 0.33 \\
        BC            & 16.00 Mbps   & 7.50 bps/Hz   & 0.31     \\
        BCQ           & 16.00 Mbps   & 7.60 bps/Hz   & 0.34     \\
        CQL           & 16.05 Mbps   & 7.59 bps/Hz   & 0.33     \\
        DT            & 15.67 Mbps   & 7.25 bps/Hz   & 0.36     \\
    \bottomrule\bottomrule
    \hline
    \end{tabular}
    \vspace{0.25cm} % Adjust vertical space between table and caption
    \label{table: s-opt table}
\end{minipage}
\end{table*}


\subsection{General Results}

\begin{comment}
    \cref{table: opt table,table: s-opt table} present the  results of in terms of throughput, \ac{BLER} and \ac{SE}: offline \ac{RL} models in  \cref{table: opt table} have been trained on $\mathcal{D}_{\rm opt}$, while models in  \cref{table: s-opt table} on $\mathcal{D}_{\rm s-opt}$. When considering $\mathcal{D}_{\rm opt}$, we notice how the offline \ac{RL} methods achieve comparable results across all the considered metrics, with \ac{CQL} and \ac{BCQ} scoring slightly better than \ac{DT}. Yet, they are only able to match the performance of the \ac{BC} baseline.
However, the differences are more evident when considering suboptimal training data $\mathcal{D}_{\rm s-opt}$.   \ac{CQL} reaches almost the same performance as models trained on $\mathcal{D}_\text{opt}$  in terms of \ac{SE}. On the other hand, when trained on data that is suboptimal, \ac{DT} is not able to match the performance of the behavioral policy. Our results for both settings show that \ac{BC} seems to work sufficiently well on this use-case. \sam{Plots in Fig. \ref{cdf} look at the CDF curves resulting from the experiments on $\mathcal{D}_{\rm opt}$}. The results just mentioned are the best we could obtain experimenting with different design choices and hyperparameter configurations; specifically, the \ac{DT} results are obtained by sampling sequences including the most recent $H=32$ transitions and following the \ac{3GPP} conditioning approach.
\end{comment}

We compare the performance of our \ac{LA} designs based on value-based offline \ac{RL}, with \ac{BCQ} \cite{fujimoto2019off} and \ac{CQL} \cite{kumar_conservative_2020}, and sequence modeling with \ac{DT}. We evaluate their performance in terms of average \ac{UE} throughput, \ac{SE} and experienced \ac{BLER}. We consider three baselines: the \ac{OLLA} approach introduced in~\cref{sec:problem formulation}, representing the state-of-the-art in real-world \acp{RAN}; a simple \ac{BC} approach, which learns to reproduce actions;  and the behavioral \ac{DQN} policy. We tested the algorithm using $50$ randomized simulation scenarios. % We refer to \cite{Peri_2024} for an extended description

\cref{cdf} presents the \acp{CDF} of \ac{UE} throughput, \ac{SE} and experienced \ac{BLER} for the best configuration of each offline \ac{RL} \ac{LA} algorithm obtained experimenting with different design choices and hyperparameters and models trained using $\mathcal{D}_{\rm opt}$. For the \ac{DT} design, this implies sampling sequences that include the most recent $H=32$ transitions and applying the \ac{CCTR} conditioning approach. Furthermore, \cref{table: opt table,table: s-opt table} summarize the average results for all models trained using $\mathcal{D}_{\rm opt}$ and $\mathcal{D}_{\rm s-opt}$, respectively.


For model trained with $\mathcal{D}_{\rm opt}$, \cref{table: opt table} shows that all offline \ac{RL} methods achieve similar results across all the metrics, reaching the performance of the data collection policy $\pi_{\rm opt}$ and outperforming the industry baseline \ac{OLLA} by $\approx 8.8\%$ in average \ac{UE} throughput and $\approx 20.7\%$ in average \ac{UE} \ac{SE}.

With sub-optimal training data  $\mathcal{D}_{\rm s-opt}$, \cref{table: s-opt table} shows that \ac{CQL} and \ac{BCQ} reach approximately the same performance observed when trained on $\mathcal{D}_\text{opt}$, on pair with the behavioral policy $\mathrm{DQN}_{\rm s-opt}$ and \ac{BC}. However, in this case \ac{DT} shows a slight degradation compared to $\mathrm{DQN}_{\rm s-opt}$, but consistently outperforms the OLLA baseline.

\subsection{Considerations on the \ac{DT} Design}
Hereafter, we analyze in more details the effect of different design aspects of the \ac{DT}. \cref{table:pe and conditioning - throughput} summarizes the best results obtained for different combinations of the positional encoder and conditioning methods presented in \cref{sec:method}. For this analysis, we considered $\mathcal{D}_\text{opt}$ as training set and trajectories constructed with the \emph{recent transmissions} approach introduced in \cref{trajectory definition}, with $H=32$. For the VANILLA and DAVG conditioning, we conditioned on the 90\% quantile of the distribution of RTGs in the training dataset (filtered at the first retransmission in the case of VANILLA conditioning). The average future rewards are computed over a fixed window size of $35$ steps, with a discount factor $\gamma = 0.8$. 

For positional encoding, our results indicate that including temporal information about packet distribution is beneficial. Specifically, the \ac{LT} approach, which learns embeddings directly from the actual timestamps of packet transmissions, achieves better performance than \ac{BE} and \ac{CT}, which use encoding based on the token's index and trigonometric functions, respectively.


Furthermore, regarding \ac{RTG} conditioning, our results in \cref{table:pe and conditioning - throughput} indicate that \ac{CCTR} conditioning achieves better throughput than both VANILLA and DAVG conditioning across all types of positional encoding. We observed similar results in terms of \ac{BLER} and \ac{SE}, which are not included here for brevity. This demonstrates that, for the \ac{LA} problem, conditioning the model inference based on the channel state is important. %We further analyze this aspect in the next section.



\begin{comment}
    
\subsection{Considerations on the \ac{DT} Design}
In \cref{table:pe and conditioning - throughput} we show results for different combinations of the positional encoder and conditioning methods proposed in  \cref{sec:method} for the Decision Transformer (we only consider results obtained by training on $\mathcal{D}_\text{opt}$).

Including temporal information about packet distribution using the \ac{LT} encoding appears to be beneficial compared to both BE and \ac{CT} encoding, with these two achieving similar performance. Specifically, learning embeddings directly from the actual timestamps of packet transmissions leads to substantial performance improvements, while using an encoding based on trigonometric functions (i.e., \ac{CT}) results in worse performance.

%Including information about the distribution of packets in time with the use of \ac{LT} encoding appears to be beneficial with respect to both the BE and \ac{CT} encoding, with these two achieving very similar performance. Interestingly, using the timestamps of packet transmissions to learn embeddings (i.e.: \ac{LT}) brings substantial improvements to performance, while an encoding based on trigonometric functions (i.e.: \ac{CT}) achieves worse performance. 

Regarding \ac{RTG} conditioning, our results in \cref{table:pe and conditioning - throughput} indicate that \ac{CCTR} conditioning achieves better throughput than both VANILLA and DAVG conditioning across all types of positional encoding. We observed similar results in terms of \ac{BLER} and \ac{SE}, which are not included here for brevity. This evidence supports our hypothesis that conditioning differently based on channel conditions is beneficial.

%Concerning \ac{RTG} conditioning, our results in  \cref{table:pe and conditioning - throughput} indicate that \ac{CCTR} conditioning achieves better throughput\footnote{We observed similar results in terms of \ac{BLER} and \ac{SE}, which are not included for ease of presentation.} compared to VANILLA and AVG conditioning, across all types of positional encoding. This evidence supports our hypothesis that it is reasonable to condition differently depending on the channel conditions.

For the VANILLA and DAVG conditioning types, we conditioned on the 90\% quantile of the distribution of RTGs in the training dataset (filtered at the first retransmission in the case of VANILLA conditioning). The average future rewards are computed over a fixed window size of $35$ steps, with a discount factor $\gamma = 0.8$. The results reported here have been obtained following the first of the two approaches to trajectory definition introduced in Section \ref{trajectory definition}, with $H=32$.

 %Results for the VANILLA and AVG conditioning types are obtained by conditioning on the $90\%$ quantile of the distribution of \acp{RTG} in the training dataset (filtered at the first retransmission, in case of vanilla conditioning). \textcolor{red}{Average, future rewards are computed on a fixed window size of $35$ steps, with $\gamma=0.8$.}
\end{comment}

\begin{table}[]
\centering
\caption{Comparison of different types of position encoding and RTG conditioning. Best in \textbf{bold}, second best in red.
%\gf{\it GF: What is "PE" type in the below table and we spell it out ?}
}
\renewcommand{\arraystretch}{1.25}
\begin{tabular}{lccc}
\toprule\toprule
\gf{Pos. Emb.}     & VANILLA       & CCTR          & DAVG           \\ \hline
BE          & 15.75 Mbps & 15.83 Mbps & 15.76 Mbps \\
CT              & 15.35 Mbps & 15.86 Mbps & 15.73 Mbps \\
LT & \textcolor{red}{16.01 Mbps} & \textbf{16.07 Mbps} & 15.66 Mbps \\
\bottomrule\bottomrule
\end{tabular}
\label{table:pe and conditioning - throughput}
\end{table}

\subsection{Outcome Conditioning}
\label{RTG conditioning}

We further analyze the effect of model output conditioning for \ac{LA} with respect to (a) the type of conditioning (using the VANILLA and \ac{CCTR} approaches, cf. \cref{subsec:conditioning}); and (b) the sequence length (using the \emph{consecutive packets} approach).
%
\Cref{table: more-packets} summarizes the results, considering input sequences that comprise transmissions related to $n_p\in[1,\; 16]$ packets and, for VANILLA conditioning, three \ac{RTG} target values $\omega$ chosen as the $\{20,60,100\}$-quantiles of the training \ac{RTG} distribution.

%{\color{red} This approach allows us to better observe the effect of conditioning on different \ac{RTG} values during inference and to determine the extent to which the \ac{DT} can replicate the target \ac{RTG} values.}

For wireless applications, like \ac{LA}, conditioning the action generation to \ac{RTG} target values that reflect the radio conditions is instrumental to achieve good performance. This is demonstrated by the \ac{CCTR} approach, which adapts \ac{RTG} target value for each packet transmission using the nominal spectral efficiency corresponding to the latest \ac{CQI} reported by the \ac{UE}. On the other hand, conditioning the action generation to fixed \ac{RTG} target values that do not reflect the radio conditions, as in the VANILLA approach, can lead to substantial performance degradation. For instance, choosing a too high (fixed) \ac{RTG} target value causes the \ac{DT} to take more aggressive \ac{LA} actions, i.e., higher \ac{MCS} index, which leads to an increased frequency of retransmissions during testing, reflected by lower throughput and \ac{SE} and a higher \ac{BLER}.

Although the transformer architecture excels in learning from long sequences of information, for wireless applications that act directly on packet transmissions, like \ac{LA}, long sequences may not be desirable. In fact, when consecutive tokens in the sequence are associated to data packets transmitted far apart in time (e.g., more than the channel coherence time), learning auto-regressively from too aged historical tokens can induce variance and cause the \ac{DT} to clone the behavioral policy. For instance, \cref{table: more-packets} shows that, with \ac{CCTR} conditioning, the \ac{DT} benefits from including more packets in the sequence until $n_p=8$, while longer sequences does not yield better performance.  We refer to \cite{Peri_2024} for an extended analysis.

% The \ac{DT}, however, can effectively model short sequences of packet transmissions.

\begin{table}[t!]
    \centering
    \setlength{\tabcolsep}{3pt}
    \caption{Performance obtained by conditioning on increasing, fixed, RTG values at inference for models including variable numbers of packets inside their sequence (vanilla).}
    \begin{tabular}{llllll}
    \toprule\toprule
    $n_p$ & Metrics      & CCTR     & $\omega=1.71$  & $\omega=3.86$ & $\omega=7.57$ \\ \hline
         & Th.put    & 15.73 Mbps & 15.30 Mbps & 13.80 Mbps & 13.94 Mbps \\
    1    & BLER          & 0.37       & 0.33       & 0.42       & 0.83       \\
         & SE            & 7.45 bps/Hz & 7.14 bps/Hz & 6.92 bps/Hz & 7.19 bps/Hz \vspace{3mm} \\
         & Th.put    & 15.72 Mbps & 15.08 Mbps & 13.75 Mbps & 13.98 Mbps \\
    2    & BLER          & 0.38       & 0.31       & 0.41       & 0.82       \\
         & SE            & 7.45 bps/Hz & 7.08 bps/Hz & 6.87 bps/Hz & 7.25 bps/Hz \vspace{3mm} \\
         & Th.put    & 16.02 Mbps & 15.93 Mbps & 15.45 Mbps & 14.06 Mbps \\
    4    & BLER          & 0.31       & 0.28       & 0.36       & 0.74       \\
         & SE            & 7.43 bps/Hz & 7.32 bps/Hz & 7.45 bps/Hz & 7.46 bps/Hz \vspace{3mm} \\
         & Th.put    & 16.04 Mbps & 16.01 Mbps & 15.96 Mbps & 14.49 Mbps \\
    8    & BLER          & 0.28       & 0.27       & 0.30       & 0.62       \\
         & SE            & 7.40 bps/Hz & 7.34 bps/Hz & 7.42 bps/Hz & 7.56 bps/Hz \vspace{3mm} \\
         & Th.put    & 16.02 Mbps & 15.93 Mbps & 15.45 Mbps & 14.06 Mbps \\
    12   & BLER          & 0.31       & 0.30       & 0.31       & 0.46       \\
         & SE            & 7.45 bps/Hz & 7.42 bps/Hz & 7.46 bps/Hz & 7.58 bps/Hz \vspace{3mm} \\
         & Th.put    & 16.02 Mbps & 15.93 Mbps & 15.45 Mbps & 14.06 Mbps \\
    16   & BLER          & 0.30       & 0.29       & 0.31       & 0.40       \\
         & SE            & 7.44 bps/Hz & 7.42 bps/Hz & 7.44 bps/Hz & 7.48 bps/Hz \\
    \bottomrule\bottomrule
    \end{tabular}
    \label{table: more-packets}
\end{table}

\begin{comment}
    In this section, we analyze the \ac{RTG} conditioning of the \ac{DT}, as discussed in \cref{subsec:conditioning}. We start by considering input sequences that comprise transmissions related to a single packet (i.e., $n_p=1$), we then extend the analysis by incrementally increasing the number of packets included in the input sequences. This approach allows us to better observe the effect of conditioning on different \ac{RTG} values during inference and to determine the extent to which the \ac{DT} can replicate the target \ac{RTG} values.

%In this section we analyse the \ac{RTG} conditioning of the DT, as discussed in \cref{subsec:conditioning}. We start by considering input sequences comprising transmissions relative to one single packet (i.e.: $n_p=1$) and then extend the analysis to include an increasing number of packets to better observe the effect of conditioning on different values at inference and find out to what extent \ac{DT} can replicate target \ac{RTG} values.

\Cref{table: more-packets} shows the performance of \ac{DT} when we vary the target \ac{RTG} value $\omega$ across the $q\%$ quantiles of the training \ac{RTG} distribution, with $q\in \{20,60,100\}$. As expected, conditioning the action generation on higher target \ac{RTG} values causes the \ac{DT} to take more aggressive actions and leads to an increased frequency of retransmissions during testing, reflected by a higher \ac{BLER}. Conversely, we observe a decreasing trend in throughput, with the \ac{CCTR} baseline achieving the best performance due to the induced correlation between the target \ac{RTG} values and the channel conditions.

% \cref{table: more-packets} shows the performance of \ac{DT} by sweeping the value of the target \ac{RTG} value $\omega$ over the $q\%$ quantiles of the training distribution of \acp{RTG} (with $q \in [0.2, 0.6, 1.0]$). As expected, conditioning the generation of actions on increasing target values of \ac{RTG} causes \ac{DT} to take more aggressive actions and, as a consequence, retransmissions at inference time increase in frequency (\ac{BLER}); at the same time, we notice an opposite trend in terms of throughput, with \ac{CCTR} achieving yet again the best performance because of the induced correlation between the target value and channel conditions.

As we include more packets in the sequences, the average performance tends to improve. However, when experiments involve sequences with eight or more packets, the \ac{BLER} values converge to those achieved by the behavioral DQN policy. These results imply that while the \ac{DT} can effectively model short sequences of packet transmissions, incorporating longer sequences likely introduces too much variance. This increased variance may cause the \ac{DT} to default to simply cloning the behavioral policy, as suggested by the poor performance shown in \cref{table: s-opt table}. Consequently, this effect prevents the 
\ac{DT} from extrapolating optimal behavior from suboptimal data. We refer to \cite{Peri_2024} for an extended analysis.
\end{comment}

==> old_versions/backup_2024_11_25/7_conclusion.tex <==
\section{Concluding Remarks}
\label{sec:conclusion}
\begin{comment}
    In this paper, we designed three offline \ac{RL} algorithms, with the purpose of replacing the legacy \ac{OLLA} scheme with a scheme that learns from data without causing negative impact on the network performance. Specifically, we investigated the performance of \ac{BCQ}, \ac{CQL} and a \ac{DT}-based design, where a trained \ac{DQN} model served as the behavioral policy for data collection. The purpose of employing the \ac{DQN} for data collection is to investigate whether an offline \ac{RL} can achieve similar \ac{LA} performance as that achieved by online \ac{RL} when the offline \ac{RL} scheme is trained with proper data. To gain insight into the effect of data collection, both an optimal $\pi_{\rm opt}$ and a suboptimal $\pi_{\rm s-opt}$  \ac{DQN} policy -- which was trained with only half of the data used for the training of the $\pi_{\rm opt}$ policy -- were used. 
    %
    For the \ac{DT}-based design, we have modified  the associated (1) attention layer by suitable masking and 
    (2) the positional encoding in order to capture the temporal correlation between subsequent packet transmissions.
    %\gf{\it GF: Here we need to say something about BCQ and CQL.}
    
    The results indicate that the three offline \ac{RL} schemes considered in this work yield similar performance in terms of the achieved throughput, \ac{BLER} and \ac{SE}, which are also similar to those achieved by the online \ac{DQN} policy and outperform the \ac{OLLA} baseline. While there is no significant performance gap between the three offline \ac{RL} methods,  \ac{BCQ} and \ac{CQL} may have lower computational complexity than \ac{DT}. 
    \gf{\it GF: We need to justify this better, since this is the first time we mention complexity.}
    
    However, we stress that the results presented in this paper are limited to a specific network deployment scenario.  Achieving model generalization to \acp{RAN} operating over large geographical areas may require to train models on substantially larger data sets collected across the network, in which case the transformer architecture has proved more effective to extrapolate intricate patterns.
    \gf{\it GF: Where has it proved that ?}
    Therefore, investigating the performance of these offline \ac{RL} algorithms when operating over large \ac{RAN} deployments is an important future work.
\end{comment}


In this paper, we designed three offline \ac{RL} algorithms, with the purpose of replacing the legacy \ac{OLLA} scheme with a scheme that learns from data without causing negative impact on the network performance. Specifically, we investigated the performance of \ac{BCQ}, \ac{CQL} and a \ac{DT}-based design, where a trained \ac{DQN} model served as the behavioral policy for data collection. 
%The purpose of employing the \ac{DQN} for data collection is to investigate whether an offline \ac{RL} can achieve similar \ac{LA} performance as that achieved by online \ac{RL} when the offline \ac{RL} scheme is trained with proper data. 
To gain insight into the effect of data collection, both an optimal $\pi_{\rm opt}$ and a suboptimal $\pi_{\rm s-opt}$ \ac{DQN} policies -- which was trained with only half of the data used for training the $\pi_{\rm opt}$ policy -- were used. 
%
For the \ac{DT}-based design, we have modified (1) the associated attention layer by suitable masking and (2) the positional encoding definition in order to capture the temporal correlation between subsequent packet transmissions.
%\gf{\it GF: Here we need to say something about BCQ and CQL.}

The results indicate that the three offline \ac{RL} schemes considered in this work yield similar performance in terms of the achieved throughput, \ac{BLER} and \ac{SE} \ps{for \ac{LA}}, which are also similar to those achieved by the online \ac{DQN} policy and outperform the \ps{industry baseline \ac{OLLA} 
\gf{in terms of average \ac{UE} throughput (by $\approx 8.8\%$) and average \ac{SE} (by $\approx 20.7\%$).}}
%by $\approx 8.8\%$ in average \ac{UE} throughput and $\approx 20.7\%$ in average \ac{UE} \ac{SE}}. 

While there is no significant performance gap between the three offline \ac{RL} methods, \ps{our evaluations in this work considered a specific network deployment scenario. In this case, all algorithms could enjoy relatively small models, with \ac{BCQ} and \ac{CQL} using smaller models, and hence have lower computational complexity, than \ac{DT}. However, achieving model generalization over the \ac{RAN} environment, and thereby being able to deploy the same AI model across cells in large geographical areas, will require to train models on substantially larger data sets collected across the network deployment. As such, the ability of the transformer architecture to effectively learn and extrapolate intricate patterns from large dataset may lead to better performance.} Therefore, investigating the performance of these offline \ac{RL} algorithms when operating over large \ac{RAN} deployments is an important future work.

Finally, although a \ac{DQN}-based data collection is helpful for investigating whether offline  \ac{RL}  can achieve similar  \ac{LA}  performance as that achieved by online \ac{RL}, finding a non-intrusive data collection policy that properly explores the state-action space without affecting the system performance in live \acp{RAN} remains an open problem, which we are considering in our own future work.

%Finally, the purpose of employing the \ac{DQN} for data collection is to investigate whether offline \ac{RL} can achieve similar \ac{LA} performance as that achieved by online \ac{RL} when the offline \ac{RL} scheme is trained with proper data. \ps{However, while one may use a \ac{DQN} policy trained in simulators to collect data in the field, finding a non-intrusive data collection policy that can properly explore the state-action space without affecting the system performance in live \acp{RAN} remains an open problem which we are considering in our future work.}



\begin{comment}
Furthermore, we adopted the \ac{DT} architecture for \ac{LA}. 
We enhanced \gf{the} performance by modifying the associated (1) attention layer by suitable masking and the (2) positional encoding in order to capture the temporal correlation between subsequent packet transmissions.  
%positional encoding and attention masks and by conditioning on channel quality indicators to handle irregular time intervals and to ensure causality. 
\gf{\it GF: This is the first time we mention causality, so this comes a bit out of the blue here...}
\gf{The results indicate that} \ac{DT} struggles with the stochastic nature of \ac{LA} due to interference and varying channel conditions, which affect its ability to select the optimal \ac{LA} action. 
In particular, we notice that while \ac{DT} is able to correctly condition the inference of close-to-optimal actions when dealing with sequences comprising \gf{a few packet transmissions}. 
\gf{However,}
when \gf{the} input sequences become longer, the inherent variance of \gf{the propagation conditions and interference makes it hard for}
%\ac{LA} makes it hard for 
\ac{DT} to select the correct \ac{LA} action.
%model the stochasticity intrinsic to the process correctly.
\gf{\it GF: The conclusion only talks about DT and does not say much about BCQ and CQL...}
Despite these challenges, our work provides valuable insights into applying machine learning in telecommunication networks and supports the use of offline \ac{RL} methods to train agents for live networks. \gf{\it GF: The last sentence should talk about achieving similar result with offline RL as with online RL.}
\end{comment}

% Our simulations showed that offline \ac{RL} methods slightly improve upon the behavioral policy used for data collection, 
% starting from both optimal and suboptimal policies. 
 
% In this paper, we have addressed the problem of \ac{LA} by adopting alternative approaches to offline \ac{RL}. 

% Our thorough comparison run on a proprietary \ac{RAN} simulator has demonstrated the capabilities of the offline \ac{RL} methods we considered to obtain performances that slightly improve on the behavioral policy employed for collecting the training dataset, both in the case of optimal and suboptimal behavior. Despite employing datasets collected by a \ac{RL} trained online, we believe that similar findings may be valid regardless of the policy used for data collection. However, the use of the simulator poses some limitations to our work, and, also, the validity of our results is limited to one single simulation setup.

% One important contribution of this work is the sequence modeling framework we provide to solve \ac{LA} using a \ac{DT} architecture. The modifications we proposed contribute to the performance of the vanilla architecture when employed as a solution to the use case, in particular: the adjustments to the positional encoding definition are relevant as a way to represent the distribution of consecutive steps of an \ac{MDP} in which steps do not happen in discrete series of timesteps, the new definition of the attention mask guarantees causality at training time in a delayed-feedback setting and, finally, we found beneficial to correlate the target value used for conditioning the inference of optimal actions with an indication of the channel quality. Unfortunately, our results show \ac{DT} to be very liable to the stochasticity of the \ac{LA} process (due to stochastic interference and time- and frequency-varying channel conditions), preventing the model from correctly modeling the distribution of sequence realizations and, therefore, correctly conditioning the selection of optimal actions.

% Nonetheless, we believe this work to constitute a valuable contribution to the literature of \ac{ML} in telecommunication networks and a great starting point for those practitioners considering offline \ac{RL} methods to overcome the problems associated with training agents in live networks.

\begin{comment}
\section{Notes for future work}
\ps{Not sure if this should be a separate section or part of the conclusions / final remarks. However, I would like to add some comment on this:}
\ps{
\begin{itemize}
    \item Remark why we chose a DQN policy for data collection (going back to the challenges described in the intro)
    \item Add a remark that while offline RL may achieve the performance of an online policy, finding a non-intrusive data collection policy that properly explores the state-action space remains a challenge 
    \item Add a remark on the algorithms. Specifically while there is no significant performance gap between the three methods considered in this paper, BCQ and CQL may have lower computational complexity than DT. However, the results presented in this paper are limited to a specific network deployment scenario. Achieving model generalization over RAN environment may require to train models on substantially more data collected across the network, in which case the transformer architecture has proved more effective to extrapolate intricate patterns.
\end{itemize}
}
\end{comment}

==> old_versions/repo/1_introduction.tex <==

\begin{comment}
The increasing complexity of \ac{RRM} functionalities across successive generations of mobile broadband systems, coupled with the expanding variety of deployment scenarios \cite{calabrese_learning_2018}, has driven research efforts focused on leveraging the vast amount of data available within the network from measurements and system observations \cite{calabrese_learning_2018, generalization_2024}. 

\Ac{ML} methods and, in particular, \ac{RL} have recently gained attention as a solution to address the complex control problems involved in \ac{RRM} for \acp{RAN} where time- and frequency-varying channel conditions often make rule-based algorithms suboptimal. Due to their ability to learn directly from experienced behavior and to adapt to changing environment conditions, \ac{RL} methods are being considered to replace traditional rule-based \ac{RAN} functionalities with models learned from data \cite{gronland2024constrained,mollerstedt2024model}. However, training \ac{RL} agents in a live network requires algorithms to explore the state-action space in order to learn an optimal policy, at the cost of taking actions that may be suboptimal \cite{lattimore2020bandit,russo2024model}.

In this paper, we focus on the problem of \ac{LA}, a fundamental functionality of \ac{RRM} dynamically adjusting the transmission rate of a communication link based on the channel conditions reported by the \ac{UE}. We will consider the downlink communication between a base station and the \ac{UE}, but similar findings are reusable for the uplink case. In a data-rich environment such as the \ac{RAN} one, the recent advancements in ML and, at the same time, hardware, present an opportunity to tackle the problem of link adaptation with a strongly data-driven approach \cite{calabrese_learning_2018}. A data-driven approach directly acting on the link adaptation parameters could address the shortcomings associated with current solutions to \ac{LA} that frame it as a control problem and, as shown in multiple works such as \cite{geiser_drlla_2022}, improve performance.

With the goal of overcoming the challenges associated with the training phase of \ac{RL} agents mentioned above, we consider a family of \ac{RL} algorithms referred to as \textbf{offline \ac{RL}}. Offline \ac{RL} algorithms aim at learning policies from fixed datasets of transitions previously collected by a, possibly unknown, behavioral policy. This approach is attractive for critical applications, like \acp{RAN} operations, where online learning methods could be costly to implement or negatively affect system performance, especially during training. 

The main contributions of this work include: \textbf{(1)} a thorough evaluation and comparison of the performance of the various offline \ac{RL} algorithms designed for \ac{LA} using an event-driven system-level simulator compliant with the \ac{3GPP} \ac{5G} NG-RAN system; \textbf{(2)} a new sequence modeling framework necessary to solve \ac{LA} using the \ac{DT} architecture; \textbf{(3)} the design of an offline \ac{RL} algorithm based on \ac{DT}, including a new positional encoding definition; \textbf{(4)} the definition of a new objective function for the \ac{LA} problem allowing multiple, alternative ways of conditioning the inference with \ac{DT}.

The choice of considering \ac{DT} is driven by the capability to well-generalize over different tasks and data distributions which appears evident with transformer for, especially, \ac{NLP}. Similarly, we hope \ac{DT} to be able to adapt to different types of network traffic, facilitating the deployment of a same model over different network sites.

\begin{itemize}
    \item Highlight contributions, including how to construct the sequence in training and inference
    \item Add comment on choice of baseline for comparison (e.g., why we do not relate to prior published papers)
\end{itemize}

\end{comment}
%----
\iffalse
Proposed structure of Intro (basically follows the abstract, which ensures consistency):
\begin{itemize}
    \item 
    Previous works on link adaptation is an important and challenging task
    \item 
    Previous works on addressing LA with and without learning, what is the still unsolved problem with RL
    \item 
    Along a different research, line offline RL has attractive features but also challenges
    \item 
    Why offline RL is a good idea specifically for LA, what are the challenges and how we propose to solve those.
    Final punch line.
    \item 
    Structure of the paper.
\end{itemize}
\gf{\it GF: Important: Do not write "In this paper...." before the related works and the problem are discussed. Do not write about previous works after the "In this paper..." line has been formulated.}
\fi

Modern radio access and wireless networks -- such as the Long Term Evolution and New Radio systems specified by the $3^{rd}$ Generation Partnership Project -- \iffalse -- such as the 4th generation (4G) \ac{LTE} and 5th generation (5G) \ac{NR} systems specified by the \ac{3GPP} and 802.11 networks developed by the \ac{IEEE} --\fi employ \ac{LA} algorithms to adapt the modulation and coding schemes to the \ac{CSI} available at the transmitter and maintain high spectral efficiency while adhering to block error rate targets \cite{Bruno:14, duran_self-optimization_2015, Blanquez-Casado:19, Reddy:22, Ramireddy:22, Chen:23, Nicolini:23, Xu:19}. 
Specifically in 5G systems, several enhancements to 4G measurement reporting and protocols were added in order to ensure high performance in the \ac{DL} by supporting sophisticated \ac{LA} algorithms, that take into account \ac{CSI} reports, including the rank indicator, precoder matrix indicator and the \ac{CQI} \cite{Ramireddy:22}. 

In \ac{TDD} systems, \ac{LA} in the \ac{DL} is supported by the estimated state of the uplink assuming channel reciprocity, while \ac{FDD} systems request feedback from the served \ac{UE} devices to determine the \ac{LA} parameters, such as the appropriate \ac{MCS} for the imminent data transmission. \ac{CSI} reporting and \ac{LA} are challenging tasks
due to mobility, fast fading and and limited knowledge of the receiver characteristics at the transmitter, which render model-based link adaptation algorithms complex and suboptimal \cite{Chen:23}. 
Model-based LA is especially difficult as connected \acp{UE} become increasingly heterogeneous in terms of receiver capabilities, antenna configurations and hardware characteristics \cite{Bruno:14}. 

\begin{comment}
Recognizing these difficulties, previous works have proposed reinforcement learning (RL) for LA, 
which face deployment challenges in practice due to their potential negative impacts on live network performance. 
Therefore, in this paper we propose batch-constrained deep Q-learning and conservative Q-learning for LA, 
which facilitate offline RL that can be trained on data acquired from live networks without minimal or no intrusive
effects on the network operation. Our numerical results indicate that both schemes can provide superior performance compared with that of state-of-the-art online RL methods when a proper decision transformer is employed at the transmitter.
\end{comment}

\textbf{Recognizing} these challenges faced by model-based \ac{RRM} algorithms in general, and \ac{LA} in particular, \ac{ML} methods, such as \ac{RL}, have recently gained attention as a solution to address the complex control problems involved in these tasks,~\iffalse\ac{RRM} for \ac{LA},\fi where time- and frequency-varying channel conditions often make rule-based algorithms suboptimal. Due to their ability to learn directly from experienced behavior and to adapt to changing propagation conditions, \ac{RL} is appealing to replace traditional rule-based \ac{RAN} functionalities with models learned from data \cite{gronland2024constrained,mollerstedt2024model}. However, training \ac{RL} agents in live networks requires algorithms to explore the state-action space in order to learn an optimal policy, at the cost of taking actions that may be suboptimal and potentially even harmful for the live network \cite{lattimore2020bandit,russo2024model, Chen:23}. %\cite{Bruno:14, Makridis:20, Chen:23}. 
%
\textbf{Recognizing} these detrimental effects of \ac{RL}, several recent works have proposed offline \ac{RL}, which \gf{aims to identify policies with the maximum possible utility out of the available data and omitting environmental interaction} 
\cite{levine_offline_2020-1, janner2021offline, Schweighofer:21, Kumar:23, Lyu:24}.
Although offline \ac{RL} is appealing, it may suffer from distribution shift and the consequential out-of-distribution behavior if a mismatch between the training and testing trajectories arises due to its offline nature. 
Therefore, employing offline \ac{RL} to complex real-time control problems, such as \ac{LA}, is highly non-trivial.
%\gf{\it GF: One paragraph about offline RL and the out-of-distribution and distribution shift problems and the concept 
%of transformers, as well as maybe other main concepts that must not come out of the blue later (maybe attention mechanisms ?).}

To utilize the advantages of \ac{RL} over rule-based approaches to \ac{LA} without incurring potentially negative impacts on the operation of \acp{RAN}, in this paper we propose to employ \ac{BCQ}  and \ac{CQL} 
for \ac{LA} in 5G networks, which are
value-based algorithms for offline \ac{RL} \cite{fujimoto_off-policy_2019}, \cite{kumar_conservative_2020}.  
In its discrete variant, \ac{BCQ} tackles the distributional shift issue by restricting the support 
of action selection to a subset of actions whose probability is at least $\tau>0$ times the probability 
of the action most likely selected by the behavioral policy, \gf{where $\tau$ is ... }  \cite{fujimoto_benchmarking_2019}. 
In contrast, \ac{CQL} modifies the training objective to minimize -- alongside the Bellman error \cite{Sutton:14} -- 
the estimates of the Q-values to learn lower-bounded estimates that are not overly optimistic \cite{kumar_conservative_2020}.
%which is a known issue in offline \ac{RL}  \cite{kumar_conservative_2020}.
\gf{\it GF: Need $\sim 2$ more sentences on (1) why using BCQ and CQL is challenging to employ specifically for LA and (2) how we address these challenges (at a very high level), "the punch line". 
This is just a teaser that motivates the reviewer/reader to read further.}

The rest of this paper is structure as follows...

\sam{SAM: mention reason for data collection with dqn maybe}

\gf{\it GF: 1. Check the consistency across the title, abstract, index terms and intro. 2. The intro should not exceed 1 page.}

\textbf{Possible ways to present contributions}
\begin{itemize}
    \item focus more broadly on offline RL
    \item offline RL modelling for link adaptation using CQL, BCQ and DT. More effort needed to design DT.
    \item evelautaion with industrial simulator
    \item be open about data collection policy
    \item show that we can replicate performance of DQN, and discuss remaining problems
    \item future work...
\end{itemize}

==> old_versions/repo/2_background.tex <==

This section reviews some of the key concepts and introduces notation that will be useful in the sequel.

\subsection{Elements of \ac{RL}}

\ac{RL} frames the interaction between a \ac{RL} agent and an environment as a \ac{MDP} \cite{puterman2014markov,lattimore2020bandit}, defined by the tuple: $(\mathcal{S, A, P}, r, \gamma)$. Here, $\mathcal{S}$ is the state-space, $\mathcal{A}$ is the action-space, $\mathcal{P}$ is the transition probability function (also known as transition dynamics), $r:\mathcal{S}\times\mathcal{A}\times\mathcal{S}\to\mathbb{R}$ is the reward function, $\gamma \in (0,1)$ is a discount factor. At each of a series of discrete timesteps $t$: the environment presents a state $s_t$, the agent, according to a policy $\pi:\mathcal{S}\to\mathcal{A}$, selects an action $a_t$ and, following the probability function $\mathcal P$, the agent transitions to a new state $s_{t+1}$. The reward $r_{t+1}$ is awarded for each transition. The goal of the agent is to find a policy $\pi$ \textcolor{blue}{maximizing, as an objective function, the following expression of the total return}:
$
    G_t = r_{t+1} + r_{t+2} + r_{t+2} + ... = \sum_{k+0}^T r_{t+k},
$
where $T$ indicates a terminal timestep breaking the interaction in subsequences known as \textit{episodes}. In settings in which $T$ is not naturally defined, we introduce the notion of \textit{continuing task} and re-define the return to include the discount factor $\gamma$: $
    G_t = \sum_{k+0}^\infty \gamma^k r_{t+k+1}.
$

\subsection{Offline RL}
While the goal is still the maximization of returns, in the offline \ac{RL} framework agents no longer have the ability to interact with the environment and collect additional transitions using the behavioral policy. This limits the possibility of exploring the state-action space to the transitions included in a static dataset $\mathcal{D} = \{( s_t^i, a_t^i, s_{t+1}^i, r_{t+1}^i)\}$, forcing the learning algorithm to derive a sufficient understanding of the \ac{MDP} dynamics exclusively from the aforementioned \textit{training dataset}. The challenge addressed by offline \ac{RL} is the distributional shift between the distribution under which the function approximator (policy, value function, or model) is trained and the one on which it will be evaluated. The simplest solution consists in bounding the distributional shift by constraining how much the learned policy $\pi$ differs from the behavioral policy $\pi_\beta$, with different algorithms employing slightly different approaches. A comprehensive review can be found in~\cite{levine_offline_2020}.
\\

% \textcolor{blue}{This work is going to consider \ac{BCQ} \cite{fujimoto_off-policy_2019} and \ac{CQL} \cite{kumar_conservative_2020}, two of the main value-based algorithms for offline \ac{RL}. In its discrete variant, \ac{BCQ} \cite{fujimoto_benchmarking_2019} tackles the distributional shift issue by restricting the support of action selection to a subset of actions whose probability is at least $\tau$ times the probability of the action most likely to be selected by the behavioral policy. On the other hand, \ac{CQL} \cite{kumar_conservative_2020} modifies the training objective to minimize, alongside the Bellman error, the estimates of the Q-values to learn lower-bounded estimates that are not overly optimistic, which is a known issue in offline \ac{RL} }


%     \begin{figure*}
%     \centering
%     \begin{minipage}{.49\textwidth}
%     \includegraphics[width=\textwidth]{Figures/olla_v1.2.png}
%     \caption{Visual description of the functioning of Link Adaptation.}
%     \label{fig:olla schema}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{.49\textwidth}
%     \includegraphics[width=\textwidth]{Figures/sequence_1.png}
%     \caption{Episodes in our MDP formulation for LA. Each box represents a TTI, and acknowledgements use the same color as the transmission they respond to. Between TTI 5 and 7 two packets are active, with episodes 1 and 2 overlapping. \textcolor{red}{TODO: make picture more narrow}}
%     \label{fig:sequence_1}
%     \end{minipage}
% \end{figure*}

\subsection{Decision Transformer} 
Introduced by Chen et al. in \cite{chen_decision_2021}, \ac{DT} abstracts the problem of \ac{RL} as a sequence modeling problem, exploiting the capabilities of GPT2~\cite{radford_language_2019} to perform sequential decision making. \ac{DT} models sequences of tokens of three modalities; for each timestep~$t$ of a trajectory three tokens are obtained by embedding, respectively, the state $s_t$, the action $a_t$ and the \ac{RTG} $\hat R_t = \sum_{t'=t}^T r_{t'}$. The choice of modeling sequences of \acp{RTG} allows, at inference time, to conditionally generate optimal actions by specifying \textit{future target} returns. The model is trained to predict $a_t$ by sampling sequences of $3K$ tokens (corresponding to $K$ timesteps of the \ac{MDP}). This shift in the formulation of the problem allows to bypass the need for bootstrapping to propagate returns, one of the elements most known for destabilizing \ac{RL}, particularly in its offline form.

\subsection{Communication Networks}
\textbf{Revision notes}
\begin{itemize}
    \item Elevate to section level (e.g., problem formulation)
    \item Provide a brief system description together with LA problem
    \item LA formulation as control problem
    \item LA formulation as RL problem 
\end{itemize}


Mobile telecommunication networks consist of numerous base stations, each equipped with one or more antennas. These antennas facilitate data transmission between the network and multiple users, including devices like cell phones and computers, referred to as \acp{UE}.
The primary goal of \ac{LA} is to select suitable \ac{MCS} parameters for a transmission between a \ac{UE} and a base station. To this end, in \ac{5G} \acp{RAN} some \ac{CSI} is measured by the \ac{UE} (the receiver, in the downlink case) and communicated to the transmitter. The aim of LA is to dynamically adapt the transmission rate, hence the data payload, of individual packet transmissions to the time- and frequency-varying channel conditions and radio interference. Such information is conveniently encoded with a single integer value in $[0,31]$ known as the \ac{MCS} index, which represents the output of \ac{LA}.

In this section, we first present \ac{LA} as framed for solving it as a control problem and then provide a formulation as a \ac{MDP}: we are going to consider this alternative formulation for training and evaluation of value-based offline \ac{RL} methods as well as data collection.


    
\subsection{Pure Control Formulation}\label{olla}
Traditional \ac{LA} algorithms rely on the combination of an inner- and \ac{OLLA} to reconstruct an estimate of the \ac{UE} \ac{SINR}: the \ac{ILLA} converts a \ac{CQI} to an initial estimate according to some pre-defined, link level curves while \ac{OLLA} adjusts such an estimate to take into account uncertainties in the \ac{CQI} transmission by means of a feedback loop acting on the received \ac{HARQ} signals (i.e., either positive or negative acknowledgments). \Ac{OLLA} algorithms circumvent the inherent complexity in modeling link adaptation by fixing a target \ac{BLER} value, defined as the experienced frequency of packet retransmissions. \textcolor{red}{However, while several transmissions are required for OLLA to converge to the \ac{SINR} adjustments meeting the desired \ac{BLER}, traffic for most \acp{UE} consists of short bursts of transmissions. Furthermore, most implementations require to specify a fixed \ac{BLER}, which is not optimal for all channel conditions. Figure \ref{fig:olla schema} provides a visual description of the \ac{LA} process, highlighting the different stages of the above-described solution. THIS MAY BE REMOVED AND STAY ONLY IN THE INTRO?}


==> old_versions/repo/3_problem.tex <==
\section{Link Adaptation as an RL Problem}\label{sec:problem}
In this section, we explore how Link Adaptation (LA) can be framed as an RL problem. We begin by presenting our MDP formulation of LA.
% inspired by [reference]\end{comment}
Next, we briefly discuss how offline RL methods can be applied to solve this MDP formulation. Finally, we highlight the limitations of this approach and explain why it is necessary to consider sequential modeling.

%     \begin{figure}
%     \centering

%     \includegraphics[width=0.5\textwidth]{tikz_imgs}
%     \caption{Episodes in our MDP formulation for LA. Each box represents a TTI, and acknowledgements use the same color as the transmission they respond to. Between TTI 5 and 7 two packets are active, with episodes 1 and 2 overlapping. \textcolor{red}{TODO: make picture more narrow}}
%     \label{fig:sequence_1}
% \end{figure}

\begin{figure}
    \centering
    % Resize the combined TikZ images to fit within the column width
    \resizebox{\linewidth}{!}{%
    \input{tikz_imgs/img_harq_example}
    }
    \caption{Episodes in our MDP formulation for LA. Each box represents a TTI, and acknowledgements use the same color as the transmission they respond to. Between TTI 5 and 12 two packets are active, with episodes 1 and 2 overlapping.}
    \label{fig:sequence_1}
\end{figure}
\paragraph{MDP formulation and RL}  \ac{LA} can be modeled as an episodic \ac{MDP} $M$. An episode (or trajectory) $\tau=(s_0,a_0,r_0,\dots, s_T,a_T,r_T)$  corresponds to the lifespan of a \ac{UE}'s single packet. Therefore, the length $T$ of each episode is bounded, with at-most five steps (corresponding to a first packet transmission and, in case of failure(s), up to four re-transmissions).
\begin{itemize}
    \item The state $s_t \in \mathbb{R}^n$ is a  vector of semi-static information, characterizing the serving cell, two interfering cells, and \ac{UE} design, as well as dynamic information including radio measurements, channel state information, HARQ feedback, and more
    % {\color{blue} number of transmission, resource elements,...?}
    \footnote{The exact list of states cannot be disclosed as it is based on Ericsson's internal research work.}.
    \item The action $a_t\in \{0,\dots,27\}$ takes an integer, representing one of 28 \ac{MCS} indices for data transmissions, as defined by the \ac{5G} specifications~\cite{3rd_generation_partnership_project_3gpp_technical_2024}. When dealing with a re-transmission, that is $t\geq 1$,  the simulator maps the agent's action to an \ac{MCS} index in the interval $\{28,\dots,31\}$, as per \ac{5G} specifications.
    \item  The reward signal $r_t=r(s_t,a_t)$ is function of the \ac{SE} of a packet, and takes into account the transmission count of a packet. 
    %\textcolor{red}{citation to future burak paper?} {\color{blue} Should we give more details? it's a bit scarce.}
\end{itemize}

Additionally, as the \ac{UE}'s \ac{HARQ} process supports multiple active packets at any given time, multiple \ac{UE}'s episodes may overlap in time (see example in  \cref{fig:sequence_1}). 
This MDP modeling enables a \ac{RL} agent to learn from experiences generated by any User Equipment \ac{UE} within the network. Training data samples are represented by state-action-reward tuples $(s_t,a_t,r_t)$, which allows for the evaluation and training of value-based and actor-critic methods \cite{Sutton:14}. Consequently, this formulation is particularly well-suited for use with offline RL, as it can exploit the large amounts of data collected in the network to train a policy using a fixed dataset \cite{levine_offline_2020}.


%{\color{blue} [PS]: I would add here a description of the LA design based on BCQ and CQL and move the sequence modeling paragraph to the beginning of Sec IV}

\paragraph{Sequence modeling}
However, there are some shortcomings with this modeling of LA. Firstly, such formulation optimizes only over one packet at the time, without considering sequences of multiple packets. Secondly, since packet arrivals are unknown and channel conditions are time-varying, the overall stochastic process we aim to control can be more generally framed as a \emph{contextual} \ac{MDP} \cite{hallak2015contextual}. A contextual MDP is a specific type of MDP that includes an underlying time-varying hidden parameter (context) affecting the transition dynamics—such as packet arrivals and channel conditions. Managing such a process is generally more complex than controlling a classical MDP \cite{kaelbling1998planning}. To address these complexities, we propose a sequence modeling approach \cite{janner2021offline,emmons_rvs_2021}, a method to efficiently handle sequences of data.


==> old_versions/repo/4_method.tex <==
\section{Sequence Modeling for Link Adaptation}\label{sec:method}
%We want to consider alternative solutions to \ac{LA} making use of offline \ac{RL} methods. While the formulation of the problem presented in \cref{sec:problem}  allows evaluation and training of value-based methods on a fixed dataset without requiring any further modification to the model, some tweaking is necessary to exploit the potential of sequence-based architectures.
In this section, we introduce a revised problem formulation that is better suited for a sequence modeling framework.  We then outline our contributions in adapting the original \ac{DT} design \cite{chen_decision_2021} to the \ac{LA} problem.

\subsection{Reinforcement Learning via Supervised Learning}
Sequence modeling involves training auto-regressive models on sequential data to capture patterns and make future predictions. Since the main goal in \ac{RL} is to produce a sequence of actions leading to high cumulative rewards, we can re-frame the RL problem in terms of sequence modeling.

By framing RL as a sequence modeling problem, we can better capture the time-varying interactions in the underlying process. This approach simplifies various design decisions and leverages the strengths of sequence models in handling temporal dependencies.

We consider the \ac{RvS} learning approach for offline RL considered in \cite{emmons_rvs_2021}. This approach takes as input a dataset ${\cal D}=\{\tau\}$ of trajectories of experiences and outputs an \emph{outcome-conditioned} policy $\pi_\theta(a_t\mid s_t,\omega)$ that optimizes
\begin{equation}
    \max_\theta \mathbb{E}_{\tau \sim {\cal D}}\left[\sum_{t=0}^{|\tau|-1} \mathbb{E}_{\omega \sim f(\omega\mid \tau_t)}\left[ \ln \pi_\theta(a_t\mid s_t,\omega)\right]\right],
\end{equation}
where $|\tau|$ denotes the trajectory length, $\tau_t=\{s_t,a_t,r_t,s_{t+1},\dots\}$ denotes the trajectory starting at time $t$, and $f(\omega|\tau)$  denotes the distribution over outcomes $\omega$ that occur in a trajectory. These outcomes are user-chosen, and can be, for example:
\begin{itemize}
    \item \emph{Goal-oriented}: $\omega=\{s_{h}=s\}$, that is, $f(\omega|\tau)$ indicates the likelihood of visiting state $s$ at step $h$.
    \item \emph{Reward-oriented}: $\omega=\sum_{n\geq t}\gamma^{n-t} r_n$, and $f(\omega|\tau)$ indicates the likelihood of achieving a certain total discounted  reward starting from $t$. Such conditioning is also referred to as \emph{reward-to-go} (RTG).
\end{itemize}
At inference-time, then, the user can choose to condition the policy according to the desired objective.

\subsection{RvS Learning for Link Adaptation}
 To formulate  \ac{LA}  in terms of the RvS learning framework, we introduce a trajectory definition that extends beyond the lifespan of a single packet, departing from the previous \ac{MDP} formulation.  After that, we introduce different ways to condition the policy $\pi_\theta$.
 %After that, we introduce our proposed reward-oriented conditioning, as well as  a particular type of ci
%This extension allows us to leverage a \ac{DT} approach for \ac{LA}, benefiting from the transformer's ability to perform long-term credit assignment by considering long sequences spanning multiple packet transmissions.


\subsubsection{Trajectory definition} We consider fixed-horizon trajectories $\tau=\{s_0,a_0,r_0,\dots, s_H,a_H,r_H\}$, which include  transmissions of packets belonging to a specific \ac{UE}.

%. Letting $3K$ denote the transformer's context size, each sequence can include tokens corresponding to up to $K$ transmissions, with extra positions filled using padding tokens.
We consider two alternative approaches to construct $\tau$:
\begin{enumerate}
    \item \emph{Recent transmissions}:  $\tau$ consists of the most recent $K$ transmissions of the \ac{UE} considered (hence $H=K$).
    \item \emph{Consecutive packets}: $\tau$ includes only up to  $n_p$ of a \ac{UE}'s most recent consecutive packets. Since the maximum number of retransmissions is $5$, we have that $H\in\{n_p,\dots, 5n_p\}$.
\end{enumerate}

At training time we sample trajectories of data from the dataset ${\cal D}$ using one of these two approaches, and, if needed, extra positions in  $\tau$ are filled using padding tokens.

% To formulate the \ac{LA} functionality as a sequence modeling problem, we introduce a trajectory definition that departs from the previous \ac{MDP} formulation and extends the episode horizon beyond the lifespan of a packet. This allows us to leverage a \ac{DT} approach for \ac{LA} and benefit from the transformer's ability in performing long-term credit assignment by considering long sequences of tokens that span across transmissions for multiple packets. Specifically, we define a trajectory to include all the transmissions of packets belonging to a certain \ac{UE} in a simulation. Letting $3K$ denote the context size of the transformer, tokens relative to up to $K$ transmissions can be included in each sequence, with extra positions being filled with padding tokens. We consider two alternative approaches: (1) a sequence consisting of the most recent $K$ transmissions relative to a certain \ac{UE}; (2) a sequence including transmissions relative to $n_p$ of a \ac{UE}'s most recent consecutive packets. Considering~$5$ as the maximum number of retransmission, each sequence will include a number of transmissions in $[n_p, 5n_p]$. 



% \subsection{DT design modifications}
% \label{DT modifications}
% \ac{LA} has some fundamental differences when compared to standard \ac{RL} baselines such as those considered in the original \ac{DT} paper \cite{chen_decision_2021}. In this section, we present the main modifications to its design that we found necessary for our use case.


\subsubsection{Outcome conditioning}\label{subsec:conditioning} We propose the following three ways to condition the policy $\pi_\theta$:
\begin{enumerate}
    \item {\bf VANILLA}: this is a simple conditioning that consists in fixing a target \ac{RTG} value $\omega$ for each packet $p$. At training time, the RTG at the $k$-th step of a packet is computed as  $\omega=\sum_{t=k}^{T(p)} \gamma^{t-k} r_k(p)$, where $\gamma \in(0,1]$, $r_k(p)$ indicates the reward associated to the $k$-th transmission for packet $p$ and  $T(p)$ is a random variable indicating the termination step for the transmission of packet $p$. At inference time the RTG is fixed to some pre-defined value at the first transmission and adjusted in case of retransmissions (we discuss more about this in the numerical results).

    \item {\bf DAVG}: The VANILLA formulation has the same shortcomings of the MDP formulation proposed in \cref{sec:problem}. An alternative is to condition according to a discounted average of  future rewards. Letting $n$ denote the $n$-th step in a sequence of continuous transmissions from a UE, at training time we condition according to
    \[
           \omega=(1-\gamma)\sum_{t=n}^\infty \gamma^{t-n}r_t
    \]
    with $\gamma \in(0,1)$.   At inference time, as for the VANILLA case, we condition according to some pre-defined value.
    \item {\bf 3GPP}: Lastly, we propose a novel conditioning method based on the observation that the reward signal, as mentioned in \cref{sec:problem}, is directly related to the spectral efficiency of the channel. Therefore, we condition the policy $\pi_\theta$ according to a nominal spectral efficiency value given the channel quality. Specifically, at each first packet transmission, depending on the \ac{CQI} value reported by the \ac{UE} in the state $s$, we use the corresponding nominal spectral efficiency from the 3GPP \ac{CQI} Table 5.2.2.1-3 in \cite{3rd_generation_partnership_project_3gpp_technical_2024} as the target \ac{RTG} value.
\end{enumerate}






% When shifting to a trajectory definition including all of a \ac{UE}'s transmissions it becomes unfeasible to compute \acp{RTG} on an infinite horizon. Furthermore, in radio communications, packets’ transmissions that are distant in time are roughly independent and the knowledge about future rewards is unlikely to be useful for generating optimal actions for earlier packets. Taking inspiration from the framework described by Emmons et al. in \cite{emmons_rvs_2021}, we propose the following expression as a new objective definition for \ac{LA}:

% \begin{itemize}
%     \item VANILLA: 
%         \begin{equation}
%             V(p)=\mathbb{E}\left[\sum_{k=0}^{T(p)} r_k(p)\right].
%         \end{equation}
%     \item AVG
%         \begin{equation}
%             RTG(i_0)=\mathbb E_{\tau \sim \mathcal{D}} \left[\sum_{i=i_0}^{|\tau|-1} \gamma_0^{i-i_0}r_i\right], 
%         \end{equation}
% \end{itemize}

% \begin{equation}
% \label{equation:final objective definition}
%     \mathbb E_{\Upsilon \sim \rho} \left[\sum_{n=n_0}^\infty \gamma_0^{t_n-t_{n_0}}V(p_n)\right], 
% \end{equation}
% where with $V(p)$ we refer to the value of a packet, defined as:
% \begin{equation}
%     V(p)=\mathbb{E}\left[\sum_{k=0}^{T(p)}\gamma_1^k r_k(p)\right].
% \end{equation}

% In such a formulation, $\Upsilon$ denotes a sequence of packets transmitted at random times, where $\rho$ is the distribution over packets and time. $\gamma_0$ and $\gamma_1$ are discount factors respectively affecting the sum of the values of successive packets and successive retransmissions for a single packet. $t_n$ is the time of transmission of packet $n$, with $t_{n_0}$ being the time of transmission of the first packet of the sequence. $T(p)$ is a random variable indicating the termination step for the transmission of packet $p$. Finally, $r_k(p)$ indicates the reward associated to the $k$-th transmission for packet $p$.

% The formulation is general enough that by setting $\gamma_0=0$ the objective converges to a packet basis, similar to the objective for the formulation described in \ref{MDP formulation}; by choosing $0 < \gamma_0 < 1$ the objective instead becomes a discounted sum of future rewards. We can imagine the first case as conditioning \ac{DT} on intermediate goals for each packet. 

% \textcolor{blue}{In the following sections we present results obtained by setting $\gamma_0 = 0$ or, alternatively, by simply computing average returns on a window with fixed size of $M$ transitions, discounting rewards at each transmission.}


% \subsubsection{Conditioning at inference}
% At inference time, we propose three different ways of conditioning the generation of actions. (1) \textbf{VANILLA} consists in fixing a target \ac{RTG} value $\omega$ for each packet, $\omega$ is fixed at the first transmission and adjusted in case of retransmissions; (2) \textbf{3GPP}, similarly to VANILLA, at each first packet transmission selects a target \ac{RTG} value according to the \ac{3GPP} \ac{CQI} Table 5.2.2.1-3 in \cite{3rd_generation_partnership_project_3gpp_technical_2024}, depending on the \ac{CQI} value reported by the \ac{UE} inside the state; (3) \textbf{AVG} conditions each step with the same value of average \ac{RTG} as a target. 

\subsection{Decision Transformers for LA}

In this section, we describe how we adapted the \ac{DT} architecture for the Link Adaptation (LA) problem. We introduce two changes: one to the attention layer, and one for the positional embedding mechanism.


% \begin{figure}
%     \centering
%     % Resize the combined TikZ images to fit within the column width
%     \resizebox{\linewidth}{!}{%
%     \input{tikz_imgs/img_sequence_builing}
%     }
%     \caption{Given a trajectory $\tau$ (relative to a single \ac{UE}), input sequence (a) is built by setting $K=4$ while sequence (b) is built with $n_p=2$. The first index in the notation $t_{i,j}$ identifies the transmission count while the second is a unique packet id. A same color also identifies transmissions for a same packet.}
%     \label{fig: sequence building}
% \end{figure}

\subsubsection{Attention masking for delayed feedback}

A significant challenge in training a DT architecture  for LA is preventing the leakage of future data during the training process. During inference, rewards are only received upon acknowledgment of a transmission (either positive or negative). Consequently, it is essential to ensure that the DT's outputs during training rely solely on information available in real-time, avoiding any use of future data that would not be accessible in an actual deployment.

To describe the modification we need to introduce some notation. First, for a trajectory \[\tau=(\underbrace{s_0}_{X_{0}},\underbrace{a_0}_{X_1},\underbrace{r_0}_{X_2},\dots, \underbrace{s_K}_{X_{3K}}, \underbrace{a_K}_{X_{3K+1}}, \underbrace{r_K}_{X_{3K+2}}),\]
let $(X_0, X_1,\dots, X_{3K+2})$ be the corresponding sequence of tokens fed as input to the DT. Secondly, define $t_a(p)$ and $t_r(p)$ to be the instants in time at which, respectively,  the action for packet $p$ is scheduled and  the associated reward signal is received by the BS. Lastly, indicate by $p(X)$ the mapping $X\mapsto p$ that maps a token to the corresponding packet. Then, the attention mask between any two tokens $X_i,X_j $ is given by
\[
\hbox{\texttt{attn\_mask}}(X_i,X_j) = \mathbf{1}\{ t_r(p(X_i)) \leq t_a(p(X_j))\}.
\]
 In other words, if we have not received yet any reward for packet $p(X_i)$, then the tokens of the packet $p(X_j)$ should not be affected by the tokens of packet $p(X_i)$. \cref{fig: attn mask} describes such a formulation visually.

% Formally, by referring to the instant in time at which the action for packet $i$ is scheduled with $t_{a,i}$ and the instant in time the associated reward signal is received with $t_{r,i}$, we apply:
% \begin{align}
%         \begin{array}{rcl}
%             \text{given a sequence of tokens }\left[T_0, T_1, ..., T_{3 \cdot \text{seq\_len}-1} \right], \\
%             \forall T_i,T_j, \text{ if } t_{r,i} > t_{a,j} \text{ then } attn(i,j) = -\infty,
%         \end{array}
%     \end{align}
% where $attn(i,j)$ represents the un-normalized attention score between token~$i$~and~$j$. 


\begin{figure}
    \centering
    % Resize the combined TikZ images to fit within the column width
    \resizebox{\linewidth}{!}{%
    \input{tikz_imgs/img_attention_mask}
    }
    \caption{\textbf{At training time}, the modified definition of the attention mask prevents the tokens associated to $p_2$ and $p_4$ from attending $p_1$, as its reward is not available at the time an MCS index is requested. Left matrix: original attention mask definition; right matrix: modified attention mask definition.}
    \label{fig: attn mask}
\end{figure}

\subsubsection{Temporal embeddings}
% \ac{LA} is a real-time process where states (sim. actions) are observed at points in time that are not equidistant between each other. The DT architecture was designed for processes with an equidistant sampling. We propose to capture the correlation in time between successive packet transmissions by modifying the \ac{DT} positional encoding. 
\ac{LA} is a real-time process with states (sim. actions) observed at irregular intervals, whereas the Decision Transformer (DT) architecture assumes equidistant sampling. To capture the temporal correlations between successive packet transmissions, we consider the following modifications of the DT's positional encoding:
\begin{enumerate}
    \item \textbf{Baseline encoding (BE)}: as a baseline, we implement a minor modification to the original encoder from \cite{chen_decision_2021}, where embeddings are learned based on each token's index within the sequence ($i \in [0, K-1]$).
    \item \textbf{\Ac{LT} encoding}: 
    embeddings are learned using a linear layer with $(\Delta {t}_i)_{i=0}^K$ as input, where $\Delta t_i= t_a(p(X_i)) - t_a(p(X_0))$. Hence, $\Delta {t}_i$ is a measure of the relative time  between the $i$-th token and the first one.
    Note that tokens within the same packet have identical relative timestamps, allowing the DT to associate the reward to the corresponding state and action.

    \item \textbf{\Ac{CT} encoding}: inspired by \cite{zuo_transformer_2020, zhang_continuous-time_2023},  the $k$-th element of the positional embedding vector for token $X_i$ is computed as:
\begin{equation}
    PE(\Delta t_i, k) = \begin{cases}
    \sin\left(\displaystyle \frac{\Delta t_i / 100}{{C}^{\frac k {d_\text{model}}}}\right) & \text{ for even } k, \\[4ex]
    \cos\left(\displaystyle \frac {\Delta t_i / 100} {C^{\frac {k-1} {d_\text{model}}}}\right) & \text{ for odd } k,
    \end{cases}
    \end{equation}
    where $d_{\text{model}}$ is a user-chosen constant (see also  \cite{zhang_continuous-time_2023}).
\end{enumerate}


==> tikz_imgs/img_sequence_builing.tex <==


\begin{tikzpicture}

% Define styles
\tikzstyle{block} = [draw, minimum width=1cm, minimum height=0.8cm, align=center]
\tikzstyle{arrow} = [thick,->,>=stealth]
\definecolor{darkgreen}{RGB}{0, 150, 0} % Define a custom dark green color


% Episode 1 blocks
\node[block, fill=blue!30] (1) {t$_{1,0}$};
\node[block, fill=magenta!30, right=0cm of 1] (2) {t$_{1,1}$};
\node[block, fill=yellow!30, right=0cm of 2] (3) {t$_{1,2}$};
\node[block, fill=magenta!30, right=0cm of 3] (4) {t$_{2,1}$};
\node[block, fill=green!30, right=0cm of 4] (5) {t$_{1,3}$};
\node[block, fill=green!30, right=0cm of 5] (6) {t$_{2,3}$};
\node[block, fill=magenta!30, right=0cm of 6] (7) {t$_{3,1}$};
\node[block, fill=yellow!30, right=0cm of 7] (8) {t$_{2,2}$};
\node[block, fill=cyan!30, right=0cm of 8] (9) {t$_{1,5}$};
% -------------------
\node[block, fill=lightgray!10, right=0cm of 9] (10) {};
\node[block, fill=lightgray!10, right=0cm of 10] (11) {};
\node[block, fill=lightgray!10, right=0cm of 11] (12) {};
\node[block, fill=lightgray!10, right=0cm of 12] (13) {};
\node[block, fill=lightgray!10, right=0cm of 13] (14) {};


\coordinate (B) at (9.east |- {0, -0.6}); % 0.5cm below the east point
\coordinate (C) at (9.east |- {0, +1}); % 0.5cm below the east point

\draw[dotted, red, line width=0.8mm] (B) -- (C);


\node[below=0.15cm of B] (t) {$t$};

\node[left=0.3cm of 1] (tau) {$\tau$:};

\node[below=1.5cm of 1] (approach_a) {Approach (a):};
\node[block, fill=green!30, right= 0.15cm of approach_a] (s11) {t$_{2,3}$};
\node[block, right=0cm of s11, fill=magenta!30] (s21) {t$_{3,1}$};
\node[block, right=0cm of s21, fill=yellow!30] (s31) {t$_{2,2}$};
\node[block, right=0cm of s31, fill=cyan!30] (s41) {t$_{1,5}$};



\node[right=0.8cm of s41] (approach_b) {Approach (b):};
\node[block, fill=lightgray!10, right= 0.15cm of approach_b] (s12) {[PAD]};
\node[block, right=0cm of s12, fill=yellow!30] (s22) {t$_{1,2}$};
\node[block, right=0cm of s22, fill=yellow!30] (s32) {t$_{2,2}$};
\node[block, right=0cm of s32, fill=cyan!30] (s42) {t$_{1,5}$};









\end{tikzpicture}
